A General Recipe for the Analysis of Randomized Multi-Armed Bandit Algorithms

In this paper we propose a general methodology to derive regret bounds for randomized multi-armed bandit algorithms. It consists in checking a set of sufficient conditions on the sampling probability of each arm and on the family of distributions to prove a logarithmic regret. As a direct application we revisit two famous bandit algorithms, Minimum Empirical Divergence (MED) and Thompson Sampling (TS), under various models for the distributions including single parameter exponential families, Gaussian distributions, bounded distributions, or distributions satisfying some conditions on their moments. In particular, we prove that MED is asymptotically optimal for all these models, but also provide a simple regret analysis of some TS algorithms for which the optimality is already known. We then further illustrate the interest of our approach, by analyzing a new Non-Parametric TS algorithm (h-NPTS), adapted to some families of unbounded reward distributions with a bounded h-moment. This model can for instance capture some non-parametric families of distributions whose variance is upper bounded by a known constant.

==> deviation_inequalities.tex <==
\section{Known results: Deviation inequalities for Dirichlet Sampling}

\subsection{Upper bounds}

For a set of observations $X=(X_1, \dots, X_n)$ drawn from $F \in \cF$ and for $\mu \in \R$, following Suzuki's work we can apply Chernoff trick to obtain upper bounds on the probability \[\bP\left(X^T w \geq \mu, w \in \cS^{-1}_X(\cF)\right)\;.\] Without detailing the computation, it appears clearly that if $\cF$ can be defined as a set of independent linear constraints on $w$, i.e for some $M\geq 1$ there exists some matrix $A \in \cR^{M \times n}$ and $b \in \R^M$ such that \[\bP\left(X^T w \geq \mu, w \in \cS^{-1}_X(\cF)\right) = \bP\left(A^T w \geq b\right) \;, \]

then we should have $\bP\left(X^T w \geq \mu, w \in \cS^{-1}_X(\cF)\right) \leq \exp\left(-n \kinf^\cF(F_n, \mu)\right)$, denoting by $F_n$ the empirical distribution of $X_1,\dots, X_n$.

\paragraph{Example} Consider that $\cF$ is defined by definition~\ref{def::uncentered_constraint}, i.e $\forall f \in \cF\;,\bE_f[h(|X|)]\leq B$ for some $B>0$. We use the notation $h_X = (h(|X_1|), \dots, h(|X_n|)$, consider $\alpha>0$, $\beta>0$ and write

\begin{align*}
\bP_{w \sim \cD_n}(w^T X \geq \mu, w \in \cS^{-1}_X(\cF)) & =\bP_{w \sim \cD_n}(w^T X \geq \mu, w^T h_X \leq B) \\
& = \bP_{R \sim \cE(1)^n}(R^T (X-\mu) \geq 0, R^T (B-h_X) \geq 0)\\
& = \bP_{R \sim \cE(1)^n}\left(e^{\alpha(R^T (X-\mu)} \geq 1, e^{\beta (R^T (B-h_X))} \geq 1\right) \\
& \leq \bP_{R \sim \cE(1)^n}\left(e^{\alpha(R^T (X-\mu) + \beta (R^T (B-h_X))} \geq 1\right) \\
& \leq \bE_{R \sim \cE(1)^n}\left[e^{\alpha(R^T (X-\mu) + \beta (R^T (B-h_X))}\right] \;.
\end{align*}

Now if $(\alpha, \beta) \in L_n = \left\{(\alpha, \beta): \forall i \in \{1, \dots, n\}:  \alpha (X_i-\mu) + \beta (B-h(|X_i|)) \leq 1 \right\}$, then we have that 

\begin{align*}
\bP_{w \sim \cD_n}(w^T X \geq \mu, w \in \cS^{-1}_X(\cF)) & \leq \prod_{i=1}^n \bE_{R_i \sim \cE(1)}\left[e^{\alpha(R_i (X_i-\mu) + \beta (R_i (B-h(|X_i|)))}\right] \\
& = \prod_{i=1}^n \frac{1}{1- \left(\alpha(X_i-\mu) + \beta(B-h(|X_i|))\right)} \\
& = \exp\left(-n \bE_{F_n} \left[\log\left(1-\left(\alpha(X-\mu) + \beta(B-h(|X|))\right)\right)\right]\right)\\
& \leq \exp\left(-n \max_{(\alpha, \beta) \in L_n} \bE_{F_n} \left[\log\left(1-\left(\alpha(X-\mu) + \beta(B-h(|X|))\right)\right)\right]\right)\\
& \leq \exp\left(-n \kinf^\cF(F_n, \mu)\right) \;.
\end{align*}

Building on this simple result we can make a few observations.

\begin{remark} It seems that the joint probability already has the right exploration rate if we want to build an asymptotically optimal strategy. Hence, it is not clear whether the "rejection" scheme is necessary or not. For instance, we could simply set the index of arm $k$ to $-\infty$ if the distribution obtained by drawing $w$ does not belong to $\cF$.
\end{remark}

To support this remark we can analyze $\bP(w \in \cS_X^{-1}(\cF))$ with similar Chernoff arguments. If $F_n \in \cF$, then \[\bP(w \in \cS_X^{-1}(\cF))\geq 1- \bP(w \notin \cS_X^{-1}(\cF)) \geq 1-\exp(-n H_\cF(F_n))\;,\] 
where $H_\cF$ is obtained as the $\kinf$ and should have similar continuity properties. In this case, the rejection scheme does not change much the exploration of the algorithm. On the other hand if $F_n \notin \cF$, then dividing by $\bP(w \in \cS_X^{-1}(\cF))$ should bring an exponentially increasing term in the balance. \textbf{The question is: is this boost necessary or not in the pre-convergence phase?}

\begin{remark}
	The computation remains the same with $h(|X-\mu|)$ instead of $h(|X|)$. So if the distributions satisfy definition~\ref{def::centered_constraint}, then it seems that checking that $w$ satisfies $\sum_{i=1}^n w_i h(|X_i-\mu|) \leq B$ instead of $\sum_{i=1}^n w_i h(|X_i-\bE_{F_n}[X_i]|) \leq B$ should be a good proxy that leads to the same level of exploration... maybe we can propose and analyze a "proxy" algorithm that would do that if we are not able to deal with the true constraint.
\end{remark}

\subsection{Lower bounds}

From now on we call \textit{Boundary Crossing Probability} (BCP) the expression \[\text{[BCP]} \coloneqq \bP_{w \sim \cD_{n+1}}\left(\sum_{i=1}^{n+1} w_i X_i \geq \mu, w \in \cS \right)\;,\]
for some fixed observations $(X_1,\dots, X_{n+1})\in \R^{n+1}$, a threshold $\mu \in \R$, and a subset of the simplex $\cS$ that will be specified in the context.

\subsubsection{Known results} The existing results are derived when $\cS$ is the $n+1$-dimensional probability simplex. First of all, if the observations satisfy $\forall i \neq j \;, X_i \neq X_j$ then the exact probability can be computed using a result from \cite{volume_simplex_clipped}, 

\[\bP_{w \sim \cD_{n+1}}\left(\sum_{i=1}^{n+1} w_i X_i \geq \mu\right) = \sum_{i=1}^{n+1} \frac{(X_i-\mu)_+^n}{\prod_{j=1, j \neq i}^{n+1} (X_i - X_j)} \;.\]

While useful for numerical analysis, so far we were unfortunately unable to use this result to obtain a sharp lower bound involving $\kinf$. However, a very simple lower bound can be derived by truncating all $X_i$ satisfying $X_i > \mu$ in $\mu$. Assuming without loss of generality that $X_{n+1}=\max_{i=1}^{n+1}$, we obtain

\begin{align*}
\bP_{w \sim \cD_{n+1}}\left(\sum_{i=1}^{n+1} w_i X_i \geq \mu\right) &\geq \bP_{w \sim \cD_{n+1}}\left(\sum_{i=1}^{n} w_i \min(X_i, \mu) + w_{n+1} X_{n+1} \geq \mu\right) \\
& = \frac{(X_{n+1}-\mu)^n}{\prod_{j=1}^n (X_{n+1}-X_j)} \;.
\end{align*}

A simple re-writing provides 

\begin{align*}
\bP_{w \sim \cD_{n+1}}\left(\sum_{i=1}^{n+1} w_i X_i \geq \mu\right) &\geq \exp\left(\sum_{j=1}^n \log\left(\frac{X_{n+1}-\min(X_j,\mu)}{X_{n+1}-\mu}\right)\right) \\
& \geq \exp\left(-\sum_{j=1}^n \log\left(1+\frac{\mu-\min(X_j, \mu)}{X_{n+1}- \mu}\right)\right) \\
& \geq \exp\left(-n\frac{\mu-\mu_{k, n}^+}{X_{n+1}-\mu}\right) \;,
\end{align*}

where $\mu_{k, n}^+ = \frac{1}{n} \sum_{j=1}^n \min(X_j, \mu)$. This formula is useful to understand that \textbf{when at least one observation $X_{n+1}$ tend to $+\infty$, $e^{-Cn}=o(\text{[BCP]})$ for any constant $C$.} Hence, as we know that this is not the case for families $\cF$ for which we can derive upper bounds as presented in the previous section it is necessary to understand that we will have \[\bP_{w \sim \cD_{n+1}}\left(\sum_{i=1}^{n+1} w_i X_i \geq \mu, w \in \cS \right) = o\left(\bP_{w \sim \cD_{n+1}}\left(\sum_{i=1}^{n+1} w_i X_i \geq \mu\right)\right)\;,\]

if $\cF$ is a family of unbounded distributions. This indicates us that studying the later is not sufficient for the families $\cS$ that we consider. 

For bounded distribution, a (not tight but) sufficient upper bound is provided in Lemma 14 of \cite{RiouHonda20}. Using a discretization argument, for $\epsilon>0$ there exist $M>0$ and a constant $C$ such that 
\[\bP_{w \sim \cD_{n+1}}\left(\sum_{i=1}^{n+1} w_i X_i \geq \mu\right) \geq \frac{C}{n^{\frac{M}{2}}} \exp\left(-n\left(\kinf(F_n, \mu)-\epsilon\right)\right)\;.\]

Unfortunately, the value of $M$ is inversely proportional to the discretization step, and applying the same technique without discretization would provide a factor $\frac{n!}{n^n} \sim \sqrt{2\pi n} e^{-n}$ (Stirling), which is too small to use this inequality in the proofs.

A question is: can we use this discretization trick for unbounded distributions? Well, it is trivially OK for semi-bounded distributions satisfying $\text{supp}(F) \in [a, +\infty]$ for some $a\in \R$ if they satisfy that for any $\epsilon>0$ there exist some $U \in \R$ such that $\bE_F[X \ind(X >U)] \leq \epsilon$. In the analysis we can lower bound the BCP by first truncating the observations larger than this (unknown) $U$ and then consider the discretization scheme as in the bounded case.

Hence, I think it is already interesting to consider the BCP in the bounded case, but adding the constraint $w \in \cS$, where $\cS = \{w \in \Delta^M: w^t h_{X, \mu} \leq B \}$. Without this constraint, we could provide a lower bound by consider the space $\cS_2 = \{w \in \Delta^M: w_i \in [0, w_i^\star] \; \forall i \in \{1,\dots, n\}\}$, where $w^\star \in \Delta^M$ is any weight satisfying the constraint $(w^\star)^T X \geq \mu$. With the new constraint we cannot do that, since for instance if $w = (0, \dots, 0, 1)$ is not allowed as $h(|X_{n+1}|)> B$. However, we can try to use the same trick if we assume that there exists a set $\cS_3 = \{w \in \Delta^M: w_i \in [w_i^-, w_i^+] \; \forall i \in \{1,\dots, n\}\}$ for some $w^- \in \Delta^M$ and $w^+ \in \Delta^M$ satisfying $\cS_3 \subset \cS$.

Then, denoting by $\beta_i$ the number of items in each bin a simple computations with multinomial distributions give

\[\bP(w^T X \geq \mu, w \in \cS) \geq \bP(w^T X \geq \mu, w \in \cS_3) = \frac{n!}{\prod_{i=1}^{M}\beta_i!} \prod_{j=1}^M \left(w_i^{+\beta_j}-w_i^{- \beta_j}\right) \]

Now, assume for example that $w^+$ is such that we can choose $w^-=(1-\epsilon)^\frac{1}{\beta}w^+$, then we would obtain a lower bound of the form 

\[\bP(w^T X \geq \mu, w \in \cS) \geq \frac{C}{n^{M/2}} \prod_{j=1}^M w_i^{+ \beta_j} \times \epsilon^M  \;.\]

Then, if we can jointly choose $w^+$ as the weight obtained with the $\kinf$ and $\epsilon$ as a constant independent of $n$ we would be good. However, it seems unlikely that it could be like that since it would require $w^+$ to not make the two constraints bind... and that should be the case. Maybe we should consider checking a $\cS_\eta$, allowing for instance $\sum_{i=1}^{n+1} w_i h_{X, \mu} \leq B+\eta$? 










==> draft_uncentered.tex <==
\section{Families with a centered condition $\bE_F[h(|X-\bE_F[X]|)]\leq B$}

\subsection{MED with the exact $\kinf^\cF$}

We provided an algorithm for distributions satisfying $\cF^{\text{uc}} =\{F \in \cP : \bE_F[h(|X|)] \leq B \}$ for some function $h$ and some constant $B$. Intuitively, this condition is "centered in $0$". For instance, if $h(x) = x^2$ we control the second moment of the distribution. It would be interested to study the "centered" version where we would control the variance instead. Hence, we can define the family \[\cF =\{F \in \cP : \bE_F[h(|X-\bE_F[X]|)] \leq B \}\;.\]

Studying the $\kinf^\cF$ associated with this family directly is intricate because the optimization problem is no more linear in the weights of the projection. We propose to resort on the following functions, 

\[\widetilde \cG^\cF : (F, \mu) \mapsto \inf_{G \in \cF} \KL(F, G) \quad \text{s.t } \begin{array}{ll} \bE_G[X] = \mu \\ \bE_G[h(|X-\mu|)] \leq B \end{array} \;.\]

Then, we remark that

 \[ \kinf^\cF(F, \mu_1) = \inf_{\mu \in [\mu_1, +\infty)} \widetilde \cG^\cF(F, \mu)\;.\]

The proof is direct: let $G_\star$ be a distribution satisfying $\kinf^\cF(F, \mu_1) = \KL(F, G_\star)$ and denote by $\mu_\star$ its mean. It holds that $\cG^\cF(F, \mu_\star) = \KL(F, G_\star)$, as otherwise another distribution $\widetilde G \subset \cF$ would satisfy $\KL(F, \widetilde G) < \KL(F, G_\star)$. On the other hand, with the same argument for all $\mu \in [\mu_1, +\infty)$ it holds that $\cG^\cF(F, \mu) \geq \KL(F, G_\star)= \cG^\cF(F, \mu_\star)$, hence the result.

The main interest of this transformation is that the constraint in $h$ becomes linear in the weights, as in the un-centered case. Furthermore, we can show that for a fixed distribution $F$ the minimum is achieved in a compact segment $[\mu_1, \mu_1+ \Delta_F^+]$: for $F\in \cF$, $\bP_{F}\left(|X-\mu_F| \geq h^{-1}(\frac{B}{\epsilon})\right) \leq \epsilon$. This means that if $F \in \cF$ and $\cG \in \cF$ and $G$ has mean $\mu_F + 2 h^{-1}\left(\frac{B}{\epsilon}\right)$, then a mass at least $1-\epsilon$ will be below $\mu_F + h^{-1}\left(\frac{B}{\epsilon}\right)$ for $F$, and above for $G$. Thanks to the data processing inequality it holds that \[\KL(F, G) \geq (1-2\epsilon)\log\left(\frac{1}{\epsilon}-1\right)\;.\]

This implies that $\widetilde \cG^\cF(F, \mu) \rightarrow +\infty$ when $\mu \rightarrow + \infty$, so the $\kinf^\cF$ is attained for a finite value of $\mu$. Re-formulating, we obtain that if $h(\Delta/2)/B \geq 2$, 

\begin{equation}~\label{eq::ginf_bound}\widetilde \cG^\cF\left(F, \mu_k+\Delta\right) \geq \left(1- 2\frac{B}{h\left(\frac{\Delta}{2}\right)}\right) \log \left(\frac{h\left(\frac{\Delta}{2}\right)}{B} - 1\right) \;. \end{equation}

Using that $\widetilde \cG^\cF(F, \mu_1)$ is finite, we conclude on the existence of a finite $\Delta_F^+$ for which the bound of Equation~\ref{eq::ginf_bound} is larger than $\widetilde \cG^\cF(F, \mu_1)$ for any $\Delta>\Delta_F^+$.

Then, using the same tools as for the un-centered case we can derive $\widetilde \cG^\cF$ as 

\[\widetilde \cG^\cF(F, \mu) = \max_{(\lambda_1,\lambda 2) \in \cS} \bE_F\left[\log(1-\lambda_1(X-\mu) -\lambda_2 (B-h(|X-\mu|)) \right]\;,\]

where $\cS = \{(\lambda_1, \lambda_2)\in \R \times \R^+: \inf_{y \in \R} 1-\lambda_1(y-\mu) -\lambda_2 (B-h(|y-\mu|))>0 \}$. Similarly to the un-centered case we can prove that $\lambda_1 \leq \frac{1}{h^{-1}(B)}$ and $\lambda_2 \leq \frac{1}{B-h(0)}$ \textcolor{blue}{if $\mu$ and $\mu+h^{-1}(B)$ are in the history}. However this time $\lambda_1$ can be negative, but we can show too that $\lambda_1 > -\frac{1+\frac{B}{B-h(0)}}{h^{-1}(B)}$. Hence, the optimal Lagrangian parameters belong to a compact set as in the un-centered case. The continuity of $\widetilde \cG^\cF$ wrt its two parameters can be proved similarly as in the un-centered case using Berge's theorem \cite{berge1997topological}. We can further prove the differentiability of this function in $\mu$ and compute its partial derivative as

%\[\frac{\partial \widetilde \cG^\cF(F, \mu)}{\partial \mu} = \lambda_1^\star + \lambda_2^\star \bE_{G^\star}\left[\frac{\partial h(|X-\mu|)}{\partial \mu}\right]- \frac{\partial \lambda_1^\star}{\partial \mu}\bE_{G^\star}[X-\mu] - \frac{\partial \lambda_2^\star}{\partial \mu}\bE_{G^\star}[B-h(|X-\mu|)] \;.\]
%
%We can make a few observations:
%\begin{enumerate}
%	\item With the equality constraint the third term is always $0$.
%	\item If $\lambda_1^\star\neq 0, \lambda_2^\star >0$ the constraints are binding and the derivative is $\lambda_1^\star + \lambda_2^\star \bE_{G^\star}\left[\frac{\partial h(|X-\mu|)}{\partial \mu}\right]$.
%	\item If the distribution is unbounded $\lambda_2^\star$ has to be strictly positive. If $\lambda_2^\star=0$, then $\lambda_1^\star>0$ since otherwise the mean would decrease.
%	\item With the equality $\lambda_1^\star$ can be negative.
%	\item The two partial derivatives are positive.   
%\end{enumerate}
%
%If $\frac{\partial \lambda_i^\star}{\partial \mu}$ is continuous (or $\widetilde \cG^\cF$ is doubly differentiable) then if $\lambda_i^\star=0$, $\frac{\partial \lambda_i^\star}{\partial \mu}=0$. In that case the two last product terms are always $0$ and the derivative is 
\[\frac{\partial \widetilde \cG^\cF(F, \mu)}{\partial \mu} = \lambda_1^\star + \lambda_2^\star \bE_{G^\star}\left[\frac{\partial h(|X-\mu|)}{\partial \mu}\right]\;.\]

Note that both optimal lagrangian parameters should be increasing with $\mu$ for a fixed distribution (as the problem becomes much and much harder). Hence, finding $\kinf^\cF(F, \mu_1)$ for a distribution $F$ consists in finding the minimum of a convex function over a bounded set.

%\textcolor{red}{Now I convinced myself that the products are always equal to $0$. It may not the case only in single points where we would have $\lambda_1^\star=0$ and $\frac{\partial \lambda_1^\star}{\partial \mu}>0$. Due to the continuity of the mapping $\mu \rightarrow G^\star(\mu)$ then the expectation is $0$.}

\subsection{MED with a $\kinf^\cF$ proxy} 

The main drawback with resorting to function $\widetilde \cG^\cF$ is that the location of the minimum is unclear. Furthermore, some of the properties we need such as the analysis of $\frac{\partial \kinf^\cF}{\partial \mu}$ seem complicated to obtain. We now propose to use the following functions, 

\[\cG^\cF : (F, \mu) \mapsto \inf_{G \in \cF} \KL(F, G) \quad \text{s.t } \begin{array}{ll} \bE_G[X] \geq \mu \\ \bE_G[h(|X-\mu|)] \leq B \end{array} \;,\]

to compute the $\kinf^\cF$ proxy $\cK^\cF(F, \mu) = \inf_{\mu \geq \mu_1} \cG^\cF(F, \mu)$. As the distribution minimizing $\kinf^\cF(F, \mu)$ is admissible for this new problem, it holds that $\cK^\cF(F, \mu_1) \leq \kinf^\cF(F, \mu_1)$, but the reverse is not necessarily true. Hence, a bandit algorithm can sample sub-optimal arms at a rate $\sum_k \log(T)/\cK^\cF(F_k, \mu_1)$.

We remark that the function $\cG^\cF(F,\mu)$ satisfies $\cG^\cF(F_n, \mu) \coloneqq \kinf^{\cF_{\text{uc}}}(F_{n, -\mu}, 0)$, where $F_{n, -\mu}$ is the distribution $F_n$ translated by $-\mu$ (alternatively, the empirical distribution of observations $Y_i = X_i - \mu$) and $\cF^\text{uc}$ denotes the family of distribution defined as in \ref{def::uncentered_constraint} for $h$ and $B$. Furthermore, we know that $\kinf^{\cF_{\text{uc}}}$ is continuous in both its argument, and we obtain the continuity of $\cG^\cF$ with respect to the second argument thanks to the continuity of this function in the first argument under the Wasserstein metric.

As for $\widetilde \cG^\cF$, we can show that the variations of $\cG$ wrt the second argument satisfy \[\frac{\partial \cG^\cF(F, \mu)}{\partial \mu} = \lambda_1^\star + \lambda_2^\star \bE_{G^\star}\left[\frac{\partial h(|X-\mu|)}{\partial \mu}\right]\;.\] 

However, here both Lagrangian parameters are positive since the two constraints are inequalities. Hence, if the expectation in $G^\star$ is positive, then $\cG^\cF(F, \mu)$ is increasing in $\mu$. This is the case if $\frac{\partial h(|X-\mu|)}{\partial \mu}$ is strictly convex and $h'(0)\geq 0$. Indeed, in that case we can use Jensen inequality and obtain that \[\bE_{G^\star}\left[\frac{\partial h(|X-\mu|)}{\partial \mu}\right] \geq \frac{\partial h(|\bE_{G^\star}[X]-\mu|)}{\partial \mu} = h'(\bE_{G^\star}[X]-\mu)\geq h'(0) \geq 0 \;.\]

Hence, we obtain that $\cG^\cF$ is increasing in $\mu$. We can even obtain that it is strictly increasing, as either $\lambda_1^\star >0$ and $\frac{\partial \cG^\cF(F, \mu)}{\partial \mu} \geq \lambda_1^\star > 0$ or $\lambda_1^\star=0$ and then  $\lambda_2^\star > 0$ and $\bE_{G^\star}[X]-\mu >0$. In both cases the derivative is strictly positive.

We can hence conclude that for any $F, \mu$, if $\frac{\partial h}{\partial \mu}$ is convex and satisfies $h'(0)\geq 0$ then $\cK^\cF(F, \mu_1)= \cG^\cF(F, \mu_1)$. This avoids searching the minimum over $\mu>\mu_1$. And will be convenient to prove (P1)-(P4)

\paragraph{(P1)} comes from the continuity of $\kinf^{\cF_{\text{uc}}}$, as explained above.

\paragraph{(P2)} As for the un-centered case, we consider the value of the objective function of the optimization problem in the optimal parameter, and obtain that 
\[\bP\left(\cG^\cF(F_{k, n}, \mu_1 ) \leq \cG^\cF(F_k, \mu_1 ) -\delta\right) \leq \bP\left(L(\lambda_\star, F_{k,n}, \mu_1) \leq L(\lambda_\star, F_k, \mu_1)- \delta\right) \;,  \]

where $L(\lambda_\star, F, \mu)= \bE_F\left[\log(1-\lambda_1^\star(X-\mu)-\lambda_2^\star(B-h(|X-\mu|)))\right]$. Thanks to this re-formulation we have that $L(\lambda_\star, F_{k,n}, \mu_1)$ is the average of $n$ \textit{light-tailed} i.i.d random variables of mean $L(\lambda_\star, F_k, \mu_1)$. Hence, $\bP\left(\cG^\cF(F_{k, n}, \mu_1 ) \leq \cG^\cF(F_k, \mu_1 ) -\delta\right)$ admits an exponentially decreasing upper bound of the form $e^{-nI(\delta)}$, for some rate function $I$ satisfying $I(\delta)>0$ if $\delta>0$. 

\paragraph{(P3)} The discussion on this property is the same as in the un-centered case.

\paragraph{(P4a)} In the centered case we had to assume that $F_{k, n} \notin \cF$ has a probability decaying fast enough. Here, we choose another compact set $\widetilde \cF_\alpha$ satisfying this property, allowing us to extend the functions $h$ for which our proof works. Let $\widetilde \cF_\alpha = \{F \in \cP: \; \bE_F\left[h(|X-\mu_F|)^\frac{1}{\alpha} \leq B^\frac{1}{\alpha}\right], \Delta_F \geq \Delta^- \;,\}$

for some $\alpha$ and $\mu^-$. If we assume that the means are lower bounded we can use this directly.
Otherwise, we have to do something in the case $\mu_{k, n} \leq \mu^-$. We can for instance use the lower bound on the $\kinf^\cF$ we derive (just as we could use $\Delta^2/2$ with normal distributions). Note that to concentrate the constraint in $\widetilde \cF_\alpha$ however we will need to concentrate the mean (robust estimator?). Note: we can prove that $\mu_\star(t)\geq \min_{k\in \K} \mu_k - \epsilon$ we high probability (due to one arm being linearly sampled), so this is quite similar to fixing a lower bound on the mean. Furthermore, I think it's better if we assume that the means concentrate fast enough to avoid using robust estimator (that may break the proof because it depends on $n$, or if we want to find an estimate that work independently of the sample size).
\paragraph{(P4b)} We directly use Theorem 11 of \cite{agrawal2020optimal}, thanks to the equality $\cG^\cF(F_{k,n}, \mu)  = \kinf^{\cF_{\text{uc}}}(F_{k,n, -\mu}, 0)$.

\paragraph{Summary} Combining all those results, under the only additional condition on $h$ (wrt to the un-centered case) that $\frac{\partial h(|x-\mu|)}{\partial \mu}$ is strictly convex and that $h'(0)\geq0$, then the MED algorithm that samples the arms until they belong to $\widetilde \cF_\alpha$ and use $\cK^\cF$ as a proxy for $\kinf^\cF$ has a regret of order \[\sum_{k>1} (1+c)\frac{\log(T)}{\cK^\cF(F_k,\mu_1)-\epsilon}\;,\]
for any $c>0$ if a lower bound $\mu^-$ on the means is known. 

We can try to analyze how far this is from optimality. For an arm $k$, we have that $\cK^\cF(F_k, \mu_1) < \kinf^\cF(F_k, \mu_1)$ only if $\cK^\cF(F_k, \mu_1)$ is achieved by a distribution $G_\star$ that satisfies $\bE_{G^\star}[X]>\mu_1$ and $\bE_{G^\star}[h(|X-\mu_1|)]\leq B$, i.e the mean constraint is not binding.

I really don't think this is possible, but this seems quite intricate to prove. Intuitively, saturating the convex constraint but not the mean can happen if the distributions is already shifted on the upper side of the mean. This does not seem possible if $\mu_F<\mu_1$ and $\bE_F[h(|X-\mu_F|)]\leq B$

\cite{agrawal2020optimal} claim (Theorem 12) that in any case the constraints are tight so the equality may hold directly. However, I'm not convinced by the proofs... we can build direct counter-examples with Dirac distributions (in $h^{-1}(B+C)$ for some $C$) for instance.


\subsection{Previous draft}

\paragraph{(P1)} To prove the continuity we could use Berge theorem but it may be a bit an overkill. Maybe more simple: we proved that $\cG^\cF(F, .)$ is continuous in $\mu$ for a given distribution $F$. For any $\epsilon >0$ we consider $\kinf^\cF(F, \mu+\epsilon)-\kinf^\cF(F, \mu)$. First, this quantity is strictly positive by definition. Then, we remark that for any $\epsilon'>0$, if $\epsilon$ is small enough by continuity of $\cG$ it holds that 

\begin{align*}
	\kinf^\cF(F, \mu) & = \inf_{\widetilde \mu> \mu} \cG^\cF(F, \widetilde \mu) \\  
	&\geq \inf\left\{\kinf^\cF(F, \mu+\epsilon), \inf_{\widetilde \mu \in [\mu, \mu+\epsilon]} \cG^\cF(F, \widetilde \mu) \right\} \\
	&\geq \inf \left\{\kinf^\cF(F, \mu+\epsilon), \cG^\cF(F, \widetilde \mu)-\epsilon' \right\} \\
	&\geq \inf \left\{\kinf^\cF(F, \mu+\epsilon), \kinf^\cF(F, \mu+\epsilon)-\epsilon' \right\} \\
	& \geq \kinf^\cF(F, \mu+\epsilon)-\epsilon' \;,
\end{align*}

which gives the continuity of $\kinf^\cF$ in its second argument.

\paragraph{(P2)} $\kinf^\cF(F_{k,n}, \mu_1)>0$ so for this side of the inequality there exists a good rate function? If we consider $\inf_{\mu \in \{\mu_1, \mu_1+\frac{b_n}{n}, \dots, b_n  \}} \cG^\cF(F, \mu)$ we can now use a union bound. Actually, we can even replace $b_n$ by the upper bound corresponding to the empirical distribution, using Equation~\eqref{eq::ginf_bound} below to compute the maximum value $\mu^+$ for which $\cG^\cF(F_n ,\mu^+)$ can be smaller than $\cG^\cF(F_n, \mu)$. Furthermore, for $j \in [1, n]$ and $\mu_{kj}$ being the mean of the distribution achieving the $\kinf^\cF$, \[\bP(\cG^\cF(F_{k, n}, \mu_j) \leq \cG^\cF(F_{k,n}, \mu_{1k}) - \delta) \leq \bP(\cG^\cF(F_{k, n}, \mu_j) \leq \cG^\cF(F_{k,n}, \mu_j)- \delta) \;.\]

We further need that at some point some $\mu_j$ is close enough to the true $\mu_{k,j}$.


We can provide upper bounds on $\cG^\cF(F, \mu)$ for a given $\mu$ too. We can add $\mu$ and $\mu+h^{-1}(B)$ to the support. A simple idea is to first make the new distribution meet the condition by adding mass to $\mu$ and then to make its mean grow to $\mu$ by adding mass to $\mu+h^{-1}(B)$. We use the notation $\Delta_F= \mu-\mu_F$ and $Z_F=\bE_F[h(|X-\mu|)]$. First, we consider $G = \frac{B}{Z_F} F + \left(1-\frac{B}{Z_F}\right) \delta(\{\mu\})$. Then, we take $\widetilde G = \frac{h^{-1}(B)}{h^{-1}(B)+\Delta_F} G + \frac{\Delta_F}{h^{-1}(B)+\Delta_F} \delta(\{\mu+h^{-1}(B) \})$.

Hence, we obtain 
\[\cG^\cF(F, \mu) \leq \log\left(\frac{Z_F}{B} \left(1+\frac{\Delta_F}{h^{-1}(B)}\right)\right) = \log\left(\frac{Z_F}{B} \right)+\log\left(1+\frac{\Delta_F}{h^{-1}(B)}\right)\;. \]

Note that if $Z_F \leq B$ this can be simplified to the second term only.

Get back to (P2), we detail the computation:

\begin{align*}
	\bP\left(\inf_{\mu \in \{\mu_1, \mu_1^2,\dots, \mu_1^n  \}} \cG^\cF(F, \mu) \leq \kinf^\cF(F_{k}, \mu_1) - \delta \right) & \leq  \sum_{j=1}^n \bP\left(\cG^\cF(F_{k, n}, \mu_1^j) \leq \kinf^\cF(F_{k}, \mu_1) - \delta \right) \\
	& \leq \sum_{j=1}^n \bP\left(\cG^\cF(F_{k, n}, \mu_1^j) \leq \cG^\cF(F_{k}, \mu_1^j) - \delta \right) \\
	& \leq \sum_{j=1}^n \bP\left(L(\lambda_\star^j, F_{k, n}, \mu_1^j) \leq L(\lambda_\star^j, F_{k}, \mu_1^j) - \delta \right) \;,
\end{align*}

where $L(\lambda, F_{k, n}, \mu) = \bE_{F_{k,n}}\left[\log(1-\lambda_1(X-\mu)-\lambda_2(B-h(|X-\mu|)))\right]$ is the function giving the dual form of $\kinf^\cF$, and $\lambda_\star^j$ the optimal lagrangian parameter corresponding to the mean $\mu_1^j$. The last steps can then be copied from the uncentered case: we obtain an exponential concentration by remarking that $L(\lambda, F_{k, n}, \mu)$ is a light-tailed random variable and that $L(\lambda, F_{k}, \mu)$ is its expectation.

\paragraph{(P3)} For the means no change compared with the un-centered case.

\paragraph{(P4b)} $\bP(\kinf^\cF(F_n, \mu_1) \geq x)\leq \bP(\cG^\cF(F_n, \mu_1) \geq x)$, which concentrates as in the un-centered case since the concentration inequality holds for arbitrary empirical distributions.

\paragraph{(P4a)} This seems very complicated BUT maybe we can prove it for $\cG^\cF(F_n, \mu_1)-\cG^\cF(F_n, \mu_1- \epsilon) $. In that case we can do just as in un-the centered case. It is not direct tough.


QUESTION: Is it possible that $F \in \cF$ but the $\kinf^\cF$ is not achieved by $\cG^\cF(F, \mu)$?

\paragraph{(P4a)} $\frac{\partial \cG^\cF(F, \mu)}{\partial \mu} = \lambda_1^\star + \lambda_2^\star \bE_{G^\star}\left[\frac{\partial h(|X-\mu|)}{\partial \mu}\right]$. By Jensen we can say that if $\mathrm{d}h: x \rightarrow \frac{\partial h(|X-\mu|)}{\partial \mu}$ is convex then $\bE_{G^\star}\left[\frac{\partial h(|X-\mu|)}{\partial \mu}\right] \geq \frac{\partial h(|\bE_{G^\star}[X]-\mu|)}{\partial \mu} = h'(0)\geq0$ since $h$ is increasing on $\R^+$. If $\mathrm{d}h$ is strictly convex then the inequality is strict. In that case, we can have that the difference $\cG^\cF(F, \mu)- \cG^\cF(F, \mu-\epsilon)$ is lower bounded by $\epsilon \times \inf_{x\in [\mu_1-\epsilon, \mu_1]} \lambda_1^\star(x)$. If we proceed to lower bound this quantity by restraining the optimization problem as before we're good.

But more than that, it shows that if $dh$ is convex then $\kinf^\cF(F, \mu) = \cG^\cF(F, \mu)$ ! 

Consider $\cG^\cF(F_k, \mu_1)$. As $\bE_{F_k}[X] <\mu_1$ then at either $\lambda_1^\star >0$ or $\lambda_2^\star >0$. This is already sufficient to apply our result for the un-centered case if $h'(0)>0$ and $dh$ is convex, and by applying the trick to sample arm $k$ if $\max\{\lambda_1^\star, \lambda_2^\star \} \leq 1/\sqrt{n}$.

In fact we can even say if $\lambda_1^\star + \lambda_2^\star h'\left(\bE_{G^\star}[X]-\mu\right) \leq 1/\sqrt{n}$ re-sample the arm. Then true parameters are either (1) $\lambda_1^\star>0$, in that case we apply the same proof as the un-centered case, (2) $\lambda_1^\star=0$, then $\lambda_2^\star>0$ and $h'\left(\bE_{G^\star}[X]-\mu\right) > h'(0) \geq 0$. Hence, by all the continuity arguments if the empirical distribution is in a Wasserstein ball after enough samples this should concentrate.


\paragraph{Remark} We worked with $\cG^\cF(F, \mu) = \inf \KL(F, G): \bE_G[X] \geq \mu, \bE_G[h(|X-\mu|)] \leq B$. Hence, our $\kinf^\cF(F, \mu)=\cG^\cF(F, \mu)$ is a lower bound of the true $\kinf$. MED is then not optimal if the two quantities are not identical. However, we believe it is a nice proxy.

\paragraph{How sub-optimal is this algorithm?} If a sub-optimal distribution $F$ satisfies $\bE_F[h(|X-\mu_1|)] \leq B$, then by Theorem XX of \cite{agrawal2020optimal} we known that the solution of the optimization problem has mean exactly $\mu_1$. Hence, the two versions match and the arm is sampled optimally. Actually, the two quantities don't match only if $\lambda_1^\star=0$. I wonder if it's possible. We can be even more precise: for the solution corresponding to $\cG^F(F, \mu_1)$ not to be matched by $\kinf^\cF$ it needs to be achieved by a distribution $G^\star$ satisfying $\bE_{G^\star}[X] = \mu_{G^\star}>\mu_1$, $\bE_{G^\star}[h(|X-\mu_1|)] \leq B$, and $\bE_{G^\star}[h(|X-\mu_{G^\star}|)] > B$. All of this knowing that $\bE_F[h(|X-\mu_1|)]>B$. The third condition holds because otherwise $G^\star$ would be achievable by $\widetilde \cG^\cF(F, \mu_{G^\star})$.

\textcolor{red}{Look at the question about the normalization term: if the best arm is not in $\cF$ we are in trouble.}





==> prelim_v0.tex <==
\section{Preliminaries: randomized bandit algorithms}\label{sec::prelim}

In this section we introduce some notation to describe randomized bandit algorithms. We then detail the MED and TS algorithms considered in this paper.

\paragraph{Notation} At each step $t$, a randomized bandit algorithm $\pi$ chooses an arm $A_t$ based on
%according to
past observations $\cH_{t-1}=(A_1,X_1, \dots, A_{t-1}, X_{t-1})$, where we denote by $X_t$ the reward collected at time $t$. We define the \emph{sampling probability} of each arm $k$ at time $t$ as 
\[p_k^\pi(t) \coloneqq \bP_\pi(A_t = k | \cH_{t-1}) \;.\]
This probability depends on the empirical distribution of each arm $k$, that we denote by $F_k(t)$. We also sometimes use this notation for the empirical cumulative distribution function (cdf) with a slight abuse of notation.
%refer to through their empirical 
% While in general $p_k^\pi(t)$ could depend on all the rewards collected so far, we restrict our analysis to algorithms for which the sampling probability of an arm $k$ can be bounded only by its
% empirical distribution represented by the 
%cumulative distribution function (cdf) $F_k(t): x\mapsto \frac{1}{n}\sum_{s=1}^{t-1} \ind(X_s\leq\allowbreak   x, A_s=k)$), with a slight abuse of notation.
%knowing its history, that we summarize by its empirical cumulative distribution function (cdf) $F_k(t): x\mapsto \frac{1}{n}\sum_{s=1}^{t-1} \ind\left(X_s \leq x, A_s=k\right)$. 
Throughout the paper, we denote by $\mu_k(t)$ the empirical mean of an arm $k$ at time $t$, and by $\mu^\star(t)=\max \mu_k(t)$ the best empirical mean. We also use for convenience the notation $F_{k, n}$ and $\mu_{k,n}$, denoting respectively the empirical distribution and mean corresponding to the $n$ first observations collected from an arm $k$. Finally, we denote by $\cP$ the set of probability distributions on $\R$.
% In the paper we also denote respectively by $F_{k,n}$ and $\mu_{k,n}$ the empirical cdf and mean of arm $k$ after collecting its $n$ first rewards.
Given these elements, our analysis is based on the following assumption.

\begin{assumption}[Upper and lower bound on $p_k^\pi(t)$] \label{ass::sampling_prob}
There exist some function $D_\pi: \cP \times \R \mapsto \R$ and some \textbf{positive} sequences $(c_n)_{n \in \N}, (C_n)_{n \in \N}$ and a \textbf{non-negative} sequence $(a_n)_{n \in \N}$ such that the bandit algorithm $\pi$ satisfies for any $k$ in $\K$ that
\begin{equation}\label{eq::sampling_prob} p_k^\pi(t) \exp\left(N_k(t) \frac{D_\pi(F_k(t),\mu^\star(t))}{1+a_{N_k(t)}}\right) \in [c_{N_k(t)}^{-1}, C_{N_k(t)}] \;.
\end{equation}
%The bandit algorithm $\pi$ admits a function $D_\pi: \cP \times \R \mapsto \R$ and some \textbf{positive} sequences $(a_n)_{n \in \N}, (c_n)_{n \in \N}, (C_n)_{n \in \N}$ such that for any $F_k(t), \mu_k(t)$ it holds that
%\begin{equation}\label{eq::sampling_prob} p_k^\pi(t) \exp\left(N_k(t) \frac{D_\pi(F_k(t),\mu^\star(t))}{1+a_{N_k(t)}}\right) \in [c_{N_k(t)}^{-1}, C_{N_k(t)}] \;,
%\end{equation}
%for some function $D_\pi$.
\end{assumption}

This assumption is the very core of our general recipe to analyze randomized policies, but it will be the only assumption directly made on a given policy. Intuitively, a good choice of $D_\pi$ would be as close as possible to $\kinf^\cF$ to obtain an optimal algorithm. The analysis will rely on the properties of $D_\pi$ on the family $\cF$, and we now introduce our first assumption.

\begin{assumption}[A1]\label{ass::A1} $D_\pi$ is \textbf{continuous in its second argument}, the mapping $x \mapsto D_\pi(F, x)$ is \textbf{non-decreasing} for any distribution $F\in \cP$ , and $D_\pi(F_k(t), \mu)=0$ for any $\mu\leq \mu_k(t)$.
\end{assumption}

In Section~\ref{sec::results} we provide an upper bound on the expected number of pulls of each sub-optimal arm under a policy $\pi$, assuming only that Assumptions~\ref{ass::sampling_prob} and \ref{ass::A1} hold. Before presenting this result, we motivate Assumption~\ref{ass::sampling_prob} by introducing the two policies that are the focus of this paper: Minimum Empirical Divergence (MED) and a slight variant of Thompson Sampling (TS). 

\paragraph{Minimum Empirical Divergence} The most intuitive way to design an algorithm $\pi$ satisfying Assumption~\ref{ass::sampling_prob} for a given function $D_\pi$ is to directly fix the sampling probability as \begin{equation}\label{eq::MED} p_k^\pi(t) \propto \exp\left(-N_k(t)\frac{D_\pi(F_k(t), \mu^\star(t))}{1+a_{N_k(t)}}\right) \;,\end{equation} for a given sequence $(a_n)_{n \in \N}$. If $a_n=0$ for all $n \in \N$, this is exactly the definition of the MED algorithm, proposed by \cite{honda11MED}, that defines exactly $D_\pi\coloneqq \kinf^\cF$. More recently, \cite{jun2022} proposed Maillard Sampling (MS) for sub-gaussian distributions, following the same principle but with $D_\pi(F_k(t), \mu_\star(t)) = \frac{(\mu^\star(t)-\mu_k(t))^2}{2}$.
In the present paper we consider general functions $D_\pi$, but will try to design them as close as possible to $\kinf^\cF$. We keep the name MED for simplicity, but will carefully specify $D_\pi$ in each context. Furthermore, the tuning of $(a_n)$ will be motivated by our analysis, and will be non-zero only for a few specific cases of unbounded distributions.

We can directly verify that Assumption~\ref{ass::sampling_prob} holds with $c_n^{-1} = \frac{1}{K}$ and $C_n=1$ for any $n\in \N$, as under (A1) we have that $D_\pi(F_k(t), \mu^\star)\geq 0$ with equality if $\mu_k(t)=\mu^\star(t)$.

% the normalization term to obtain probabilities from \eqref{eq::sampling_prob} is bounded between $1$
% (one arm has a far higher empirical mean than all the others)
% %(one empirically optimal arm)
% and $K$ (all arms have the same empirical mean), so

% \[p_k(t) \exp\left(N_k(t) \frac{D_\pi(F_k(t), \mu_\star(t))}{1+a_{N_k(t)}}\right) \in \left[\frac{1}{K}, 1\right] \;,\]
% and the MED algorithm using $D_\pi$ satisfies Assumption~\ref{ass::sampling_prob}. 

\paragraph{Thompson Sampling} Usual TS algorithms are \emph{index policies}: a sample $\widetilde \mu_k(t)$ is drawn from each arm $k$, and $A_t=\aargmax\;  \widetilde \mu_k(t)$ is pulled. Unfortunately, showing that Assumption~\ref{ass::sampling_prob} is satisfied by such algorithm is very intricate, as the performance of every arm has to be considered to bound each sampling probability. Furthermore, as discussed in Remark 3 of \citet{RiouHonda20} or in \citet{baudry21DS} such sampling for the best arm increases the computational cost in non-parametric cases and may be avoided by a slight change in the algorithm. We follow this direction since, as we will discuss in Section~\ref{sec::NPTS}, TS is particularly promising as a computationally efficient version of MED.  
% Unfortunately, Assumption~\ref{ass::sampling_prob} is not satisfied by such algorithm, as the performance of every arm has to be considered to bound the sampling probabilities. For this reason, we propose a slightly different algorithm scheme to avoid this issue. 
Assuming that the learner is provided a TS sampler that can return a sampled mean $\widetilde \mu_k(t)$ for each arm given $(F_k(t), \mu_k(t))_{k\in \K}$, the proposed variant performs the following steps:
\begin{enumerate} 
	\item Sample means $\widetilde \mu_k(t)$ according to the sampler for each arm satisfying $\mu_k(t) < \mu^\star(t)$.
	\item 
 Pull an arm at random from $\cA_t=\{k: \{\mu_k(t) =\mu^\star(t)\} \cup \{\widetilde \mu_k(t)\geq \mu^\star(t)\} \}$.
 %Set $\cA_t=\{k: \{\mu_k(t) =\mu^\star(t)\} \cup \{\widetilde \mu_k(t)\geq \mu^\star(t)\} \}$, pull an arm at random in $\cA_t$.
\end{enumerate}

%\begin{algorithm}[hbtp]
%	\SetKwInput{KwData}{Input}
%	\SetKwComment{Comment}{\color{purple} $\triangleright$\ }{}
%	\SetKwComment{Titleblock}{// }{}
%	\KwData{Sampling distributions $(\cP_n(F))_{n \in \N}$, number of arms $K$}
%	Draw each arm once, initialize the empirical distribution $\wh F_k$, empirical mean $\wh \mu_k$, and $N_k=1$ for each arm $k$  \\
%	\For{$t> 1$}{
%		Set $\cA=\aargmax_{k \in \K}\wh \mu_k$\Comment*[r]{\color{purple} \small Init. the set of candidate with current best arm(s)}
%		%Set $\ell = \aargmax_{k \in \K}\; \wh \mu_k$ \Comment*[r]{\color{purple} \small Define the leader}
%		%\vspace{2mm}
%		\For{$k \in \K$, if $\;\wh \mu_k < \max_{j} \wh \mu_{j}$}{
%			Sample $\widetilde \mu_k \sim \cP_{N_k}(\wh F_k)$ \Comment*[r]{\color{purple} \small Thompson Sampling}
%			\vspace{2mm}
%			If $\widetilde \mu_k \geq \max_{j} \wh \mu_{j}$, add $k$ to $\cA$. \\
%			%\If{$\widetilde \mu_k \geq \mu_\ell$}{Add $k$ to $\cA$}
%		}
%		Draw $k_t$ at random in $\cA$ \Comment*[r]{\color{purple} \small Choose an arm uniformly in $\cA$}
%		Draw an observation from $k_t$, update $\wh F_k$, $\wh \mu_k$, $N_k=N_k+1$}
%	\SetKwInput{KwResult}{Return}
%	\caption{Variant of Thompson Sampling}
%	\label{alg::TS_variant}
%\end{algorithm}

We detail the algorithm in Appendix~\ref{subsec::variant_TS} (Algorithm~\ref{alg::TS_variant}), along with the usual index policy (Algorithm~\ref{alg::TS}) written with the same notations for an easy comparison. %Note that in step 3 non-uniform probabilities could be chosen without changing the theoretical guarantees of the algorithm (e.g. different probabilities for
%empirically best arms and the others).
%best empirical arms and challengers).
Under this algorithm, we directly obtain that when an arm is empirically sub-optimal its sampling probability satisfies 
\[p_k^\pi(t) \in \left[\frac{\bP(\widetilde \mu_k(t) \geq \mu_\star(t))}{K}, \bP(\widetilde \mu_k(t) \geq \mu_\star(t))\right] \;,\]
and $p_k^\pi(t) \in [K^{-1}, 1]$ when the arm is empirically optimal. Hence, Assumption~\ref{ass::sampling_prob} holds
%for a function $D_\pi$ 
iff \eqref{eq::sampling_prob} holds for $\bP(\widetilde \mu_k(t) \geq \mu_\star(t))$ instead of $p_k^\pi(t)$. We call such quantity a \emph{Boundary Crossing Probability} (BCP). Bounds on the BCP are available in the literature for most existing TS policies, and so the analysis presented in this paper will allow us to revisit their proofs and simplify them under this slight algorithmic change. For example, the following algorithms are covered in our analysis: 
%TS with a conjugate prior and posterior for SPEF \citep{korda13TSexp, jin22expTS} under the assumption that the means belong to a finite range $[\mu_0^-, \mu_0^+]$, Gaussian TS with inverse-gamma priors \citep{honda14} for shape parameter satisfying $\alpha\leq 1/2$ and variances supported in a finite range $[0, V]$, and Non-Parametric TS \citep{RiouHonda20} for bounded distributions with a known range.
\begin{itemize}
	\item TS with a conjugate prior and posterior for SPEF \citep{korda13TSexp, jin22expTS} and under the assumption that the means belong to a finite range $[\mu_0^-, \mu_0^+]$.
	%Equation~\eqref{eq::sampling_prob} is satisfied by TS with conjugate prior/posterior for SPEF (e.g \citep{korda13TSexp})
	\item Gaussian TS with inverse-gamma priors \citep{honda14} for shape parameter satisfying $\alpha< 0$. % and variances supported in a finite range $[0, V]$.
	\item Non-Parametric TS \citep{RiouHonda20} for bounded distributions with a known range.
\end{itemize}
For completeness, we detail their implementation (following Alg.~\ref{alg::TS_variant}) in Appendix~\ref{subsec::old_ts} (Algs.~\ref{alg::TS_SPEF}--\ref{alg::NPTS}). % Besides the theoretical interest, this new approach can also have practical advantages in avoiding the sampling step for the best empirical arm. For example, it reduces the computational cost of a step of Non-Parametric TS (NPTS) \citep{RiouHonda20}, that is proportional to the number of observations of each arm. 
The fact that only an upper and lower bound on the BCP is needed to extend the analysis of a MED algorithm to a TS algorithm is the main ingredient of our simplified proofs for TS, and will be particularly helpful to analyze the novel $h$-NPTS algorithm introduced in Section~\ref{sec::NPTS}.


%\textcolor{blue}{I'm not that satisfied with the prop below. Maybe just state the Thompson Sampling of interest and their assumptions. Maybe give some results to justify the novelty in the results section? Find a nice way to put that we obtained interesting results in appendix.}
%
%\begin{proposition}[Some results for Thompson Sampling algorithms]\label{prop::bcp_ts}	
%Upper and lower bounds for the BCP can be derived for the following algorithms, with $D_\pi=\kinf^\cF$:
%\begin{itemize}
%		\item TS with a conjugate prior and posterior for SPEF, using results from \citep{kaufmann_bayesucb, korda13TSexp, jin22expTS} and under the assumption that the means belong to a finite range $[\mu_0^-, \mu_0^+]$.
%		%Equation~\eqref{eq::sampling_prob} is satisfied by TS with conjugate prior/posterior for SPEF (e.g \citep{korda13TSexp})
%		\item Gaussian TS with inverse-gamma priors \citep{honda14} for shape parameter satisfying $\alpha\leq 1/2$ and variances supported in a finite range $[0, V]$, $V<+\infty$.
%		\item Non-Parametric TS \citep{RiouHonda20} for bounded distributions with a known range.
%	\end{itemize}
%\end{proposition}
%In some cases the bounds do not fit exactly Assumption~\ref{ass::sampling_prob} but are ``close enough'' so that our upcoming results hold. The current formulation of the assumption aims at making the presentation of our results clearer, but we refer the interested reader to Appendix~\ref{sec::TS} for more precise discussions on this topic. In Appendix~\ref{sec::TS}, we also detail the bounds and prove all the results for completeness. We also explain how we could improve the existing bounds in some cases, with some results of independent interest that we do not introduce here due to space limitation.
 
%The relaxed version of Equation~\ref{eq::sampling_prob} is provided in Equation~\ref{eq::sampling_prob_relaxed}, and we explain how our upcoming results hold similarly under the two conditions. We chose to keep Equation~\ref{eq::sampling_prob} for a simpler presentation. All the proofs are issued or adapted from \cite{kaufmann_bayesucb} (SPEF), \cite{honda14} (Gaussian), and \cite{RiouHonda20} (Bounded). 


==> preliminaries.tex <==
\section{Miscellaneous}

\textcolor{red}{All of this will be removed when I am sure that we don't need any result from there.}

\subsection{Families of distributions} 

The starting point of this project is to extend NPTS to families of unbounded distributions, in particular the sub-gaussian distributions. The set of $\sigma$-subgaussian distributions is usually defined as \begin{equation}\label{def::subgauss} f \in \cF \Leftrightarrow \forall t \in \R,\; \bE_f\left[e^{tX}\right]\leq e^{t\bE_f[X]+ \sigma^2\frac{t^2}{2}}\;.\end{equation}
Note that in the same vein we could consider sub-exponential distributions, defined with the same condition, but only for $t \in [-b, b]$ for some parameter $b>0$.

A first remark we can make is that though these distributions are widely used, they are not very practical as they set up a continuum of constraints. To avoid that, we could maybe work instead with alternative definitions. For instance, for sub-gaussian distributions we could use an alternative definition \begin{equation}\label{def::orliz} f \in \cF \Leftrightarrow \bE_f\left[e^{\left(\frac{(X-\bE_f[X])^2}{8 \sigma^2}\right)} \right] \leq 2\;.\end{equation}

This is not strictly equivalent, but \ref{def::subgauss} $\Rightarrow$ \ref{def::orliz}, and it can be shown that distributions satisfying \ref{def::orliz} are sub-gaussian (for a parameter maybe a bit larger than $\sigma$). Hence, maybe it should be fine to work with definition \ref{def::orliz} since it may simplify the analysis?

Recently, \cite{agrawal2020optimal} propose to study families of distributions defined in the following way
\begin{equation}\label{def::uncentered_constraint}
f \in \cF \Leftrightarrow \bE_f\left[h(|X|)\right] \leq B \;,
\end{equation}
for some constant $B$ and some convex function $h$ that must be continuous, non-negative, and satisfy $h(y)/y \xrightarrow[]{y \rightarrow + \infty} +\infty$. 

Building on this work, the authors then proposed in \cite{agrawal2021regret} an interesting extension of the empirical KL-UCB for heavy-tailed distributions by considering $h(x)= x^{1+\epsilon}$ for some known $\epsilon$. The main drawback of these two works is that this condition is un-centered, and preferably we would like to work with conditions involving $X-\bE[X]$, giving families defined as
\begin{equation}\label{def::centered_constraint}
f \in \cF \Leftrightarrow \bE_f\left[h(|X-\bE_f[X]|)\right] \leq B \;.
\end{equation}

In my opinion the method we propose is not restrictive to a certain family of distribution, as we only require the ability to \textit{check} that an empirical distribution belongs to this family. This can be done with any of the definition proposed above, so I suggest that we study the problem for either definition \ref{def::uncentered_constraint} or \ref{def::centered_constraint} to start with. Furthermore, for the analysis we can first consider families satisfying \ref{def::uncentered_constraint} for several reasons: 
\begin{itemize}
	\item we could compare our algorithm to the KL-UCB of \cite{agrawal2021regret}.
	\item we could use the complete study of the $\kinf^\cF$ function provided in Theorem 12 of \cite{agrawal2020optimal} (dual formulation, continuity and nice side results).
	\item the constraint is linear, which may be a great help in our quest for lower and upper bounds for the deviation probabilities we will study.  
\end{itemize}

A first step could be to check that this algorithm works well empirically in that very general setting.

\subsection{Properties of the $\kinf^\cF$ for families $\cF$ defined as in \ref{def::uncentered_constraint}}

In this section we summarize some results provided in \cite{agrawal2020optimal}. Considered a family of distributions $\cF$ defined as in \ref{def::uncentered_constraint}. We denote by $\kinf^\cF$ the function satisfying for any distribution $F \in \cF$ and any $\mu \in \R$, \[\kinf^\cF(F, \mu) = \inf_{G \in \cF: \bE_G[X]>\mu} \KL(F, G)\;, \]

where $F$ and $G$ are used to denote both the distribution and their cdf, with a slight abuse of notations. Let $\cP(\R)$ denote the set of distributions with values in $\R$, the following result restate Theorem 12 of \cite{agrawal2020optimal}, providing properties of the dual formulation of $\kinf^\cF$.

\begin{theorem}[Theorem 12 from \cite{agrawal2020optimal}]\label{th::theorem_12_agrawal}
For any $F \in \cP(\R)$ and $\mu$ such that $\bE_F[X] \leq \mu$ and $h(|\mu|)\leq B$, it holds that 
\[\kinf^\cF(F, \mu) = \max_{(\lambda_1, \lambda_2) \in \cR_2} \bE_{F}\left[\log\left(1-(X-\mu)\lambda_1 - (B-h(|\mu|))\lambda_2\right)\right]\;, \]
where $\cR_2= \left\{(\lambda_1, \lambda_2) \in (\R^2)^+: \forall y \in \R, 1-(y-\mu) \lambda_1 - (B-h(|y|))\lambda_2 \geq 0 \right\}$. Then, the following properties hold,
\begin{itemize}
	\item The maximum is attained at a unique $(\lambda_1^\star, \lambda_2^\star)\in \cR_2$.
	\item For $\mu \geq \bE_F[X]$ and $F \notin \cF$ any distribution $G^\star$ achieving infimum in the primal problem satisfies $\bE_{G^\star}[X]=\mu$ and $\bE_{G^\star}[h(|x|)]=B$. Furthermore, \[\frac{dF}{dG^\star}=\frac{1}{1-(X-\mu)\lambda_1^\star - (B-h(|\mu|))\lambda_2^\star}\;. \]
	\item If $\int_{y \in \text{Supp}(F)} dG^\star <1$, then $\text{Supp}(G^\star)= \text{Supp}(F) \cup \{y_0\}$, where \[1-(y_0-\mu) \lambda_1^\star - (B-h(|y_0|))\lambda_2^\star = 0
	\;.\]
	\item (not in Theorem 12 but in other parts of the paper) $\kinf^\cF$ is continuous with respect to each argument, under the topology induced by $(\cP(\R), W)$ for the first one where $W$ is the Wasserstein metric.
\end{itemize}
\end{theorem}

\subsubsection{Details for empirical distributions}

Consider $F=\sum_{i=1}^n \frac{1}{n} \delta_{X_i}$, for some observations $X_1, \dots, X_n$. Using Suzuki's proof to show that a distribution at most one item is added to the support achieves the minimum (the Jensen argument holds with $h$ convex), the optimization problem is 
\[ \min_{g_1, \dots, g_n, g_{n+1}, X_{n+1}} \frac{1}{n} \sum_{i=1}^n \log\left(\frac{1}{n g_i}\right) \quad \text{s.t} \quad \left\{\begin{array}{llll} \sum_{i=1}^{n+1} g_i=1 \vspace{2mm}\\ \sum_{i=1}^{n+1} g_i X_i \geq \mu \vspace{2mm}\\\sum_{i=1}^{n+1} g_i h(|X_i|) \leq B \vspace{2mm}\\ g_{n+1}\geq 0 \end{array} \right.\]
 
Note that technically we should also have written $g_i \geq 0 \forall i \in \{1, \dots, n \}$ but this constraint cannot bind as it would set the KL to $+\infty$. We write the Lagrangian function $L$ as 

\begin{align*} L(g_1, \dots, g_n, g_{n+1}, X_{n+1}, \lambda_1, \lambda_2, \lambda_3, \lambda_4) =& \sum_{i=1}^n \log\left(\frac{1}{n g_i}\right) + \lambda_1 \left(1-\sum_{i=1}^{n+1} g_i\right)+ \lambda_2 \left(\mu- \sum_{i=1}^{n+1} X_i g_i\right) \\ &+ \lambda_3 \left(\sum_{i=1}^{n+1} g_i h(|X_i|)-B\right)- \lambda_4 g_{n+1} \;. \end{align*}

We write KKT conditions, and obtain 

\begin{align}
&\frac{\partial L}{\partial g_i} = -\frac{1}{n g_i} - \lambda_1 - \lambda_2 X_i + \lambda_3 h(|X_i|) = 0 \;, \quad \forall i \in \{1, \dots, n\} \label{cond1}\\
&\frac{\partial L}{\partial g_{n+1}} = -\lambda_1 - \lambda_2 X_{n+1} + \lambda_3 h(X_{n+1}) - \lambda_4 = 0 \label{cond2}\\
&\frac{\partial L}{\partial X_{n+1}} = g_{n+1}(\lambda_3 h'(X_{n+1})- \lambda_2) = 0 \label{cond3}\\
& \sum_{i=1}^{n+1} g_i = 1 \;, \; \lambda_1 \in \R \label{cond4}\\
& \left\{\sum_{i=1}^{n+1} g_i X_i = \mu \;, \; \lambda_2 \geq 0 \right\} \quad \text{or} \quad \left\{\lambda_2 = 0 \;, \; \sum_{i=1}^{n+1} g_i X_i > \mu\right\} \label{cond5}\\
& \left\{\sum_{i=1}^{n+1} g_i h(|X_i|) = B \;, \; \lambda_3 \geq 0\right\}  \quad \text{or} \quad \left\{ \lambda_3 = 0 \;, \; \sum_{i=1}^{n+1} g_i h(|X_i|) > B\right\} \label{cond6}\\
& \left\{g_{n+1} = 0 \;, \; \lambda_4 > 0\right\} \quad \text{or}\quad \left\{ g_{n+1}>0 \;,\; \lambda_4=0\right\} \label{cond7}\;.
\end{align}

We first consider the case where $g_{n+1}=0$. Then, $X_{n+1}$ can take any arbitrary value and we only need to consider the problem without these two variables. In this case with usual techniques we obtain a result similar to Theorem~\ref{th::theorem_12_agrawal}, \[\max_{(\lambda_2, \lambda_3) \in \cR} \bE_F\left[\log \left(1- (X-\mu)\lambda_2 - (B-f(|X|)) \lambda_3\right)\right]\;,\]
with $\cR = \{(\lambda_2, \lambda_3) \in (\R^{+})^2: \min_{i \in \{1, \dots, n\}} 1 - (X_i-\mu) \lambda_2 - (B-f(|X_i|)) \lambda_3 > 0\}$. Note that the definition of $\cR$ is a bit different than the one of $\cR_2$ (less restrictive).

Now we consider the case where $g_{n+1} > 0$, which means that $\lambda_4=0$. From \ref{cond3} we remark that $\lambda_2=0 \Leftrightarrow \lambda_3 = 0$. This is impossible since (6) would give $\lambda_1=0$, and ultimately $1/g_i=0$ for all $i$. Hence, if $g_{n+1}>0$ then all other constraints are saturated. Then we obtain that $\lambda_2 = \lambda_3 h'(X_{n+1})$, and so $\lambda_1 = \lambda_3 \left(h(X_{n+1})- X_{n+1} h'(X_{n+1})\right)$. Considering that $\lambda >0$ and $\lambda_3>0$ we can now obtain 
\[g_i = \frac{1}{n} \times \frac{1}{-\lambda_1 - \lambda_2 X_i + \lambda_3 h(|X_i|)} = \frac{1}{n} \times \frac{1}{\lambda_3} \times \frac{1}{h'(X_{n+1})(X_{n+1}-X_i) - (h(X_{n+1})-h(X_i)))} \;.\]

By convexity of $h$ the denominator is always positive. 

We now use the notations $Z_i = \frac{1}{h'(X_{n+1})(X_{n+1}-X_i) - (h(X_{n+1})-h(X_i)))}$, and $\bar Z = \frac{1}{n}\sum_{i=1}^n Z_i$. Using \ref{cond4} we first obtain that 
\[\lambda_3 (1-g_{n+1}) =  \bar Z \Rightarrow g_i = (1-g_{n+1}) \frac{Z_i}{n \bar Z} \;. \]

Then, we use \ref{cond5} to obtain that 

\begin{align*} \sum_{i=1}^{n+1} g_{i} X_i = \mu & \Rightarrow \sum_{i=1}^n (1-g_{n+1}) \frac{Z_i X_i}{n\bar Z} + g_{n+1} X_{n+1} = \mu \\
\end{align*}

For simplicity of notations we now define $\bar Y = \frac{1}{n} \sum_{i=1}^n \frac{Z_i X_i}{\bar Z}$, and obtain that \[g_{n+1} = \frac{\mu- \bar Y}{X_{n+1}- \bar Y} \;, \quad \text{and so } \forall i \in \{1, \dots, n \}: \; g_i = \frac{1}{n}\times \frac{Z_i}{\bar Z} \left(\frac{X_{n+1}-\mu}{X_{n+1}- \bar Y}\right) \;.\]

Finally, using \ref{cond6} we obtain that $X_{n+1}$ is the real number satisfying 
\[\sum_{i=1}^{n+1} g_i X_i = B \Rightarrow \frac{1}{n} \left(\frac{X_{n+1}-\mu}{X_{n+1}- \bar Y}\right) \sum_{i=1}^{n} \frac{Z_i h(|X_i|)}{\bar Z} + \frac{\mu - \bar Y}{X_{n+1}-\bar Y} h(X_{n+1}) = B \;. \]

By further denoting $\bar W = \frac{1}{n} \sum_{i=1}^{n} \frac{Z_i h(|X_i|)}{\bar Z}$, and by substracting by $B$ on both sides and multiplying by $X_{n+1}-\widehat Y$ we can further obtain  

\begin{equation}\label{eq::x_to_add}
(X_{n+1}-\mu)(\bar W - B) - (\bar Y - \mu) (h(X_{n+1})-B) = 0\;.
\end{equation}

Hence, if $g_{n+1}>0$ then the value $X_{n+1}$ that is added to the support of $F$ satisfies Equation~\ref{eq::x_to_add}. We can also rewrite the expression as 
\[\sum_{i=1}^n Z_i \left((X_{n+1}-\mu)(h(|X_i|-B)) -(X_i-\mu)(h(|X_{n+1}|)-B)\right) = 0 \;. \]

\paragraph{Why is it interesting?} Equation~\ref{eq::x_to_add} can be solved with a simple search algorithm (need to find the conditions for which it holds though), so we can easily compute it and even more easily find an upper bound on $X_{n+1}$ (remark: we should study the regularity of the function in terms of $X_{n+1}$). In our NPTS algorithm, by adding something strictly larger than this value we ensure that the $\kinf^\cF$ of the modified empirical distribution will have a solution as given by Theorem~\ref{th::theorem_12_agrawal}. This makes it easier to link our BCP with $\kinf^\cF$. Now, the remaining question is: is adding this value enough to ensure sufficient exploration with our algorithm? 

\paragraph{Sanity check} Consider the case that $F$ is a Dirac in $\mu_F<\mu$. It is clear that it is necessary to add an element to its support to obtain an expectation larger than $\mu$. As all the constraints will be saturated we can simply write the $\kinf$ problem as solving the system 

\[\left\{\begin{array}{lll} p_1 + p_2 = 1 \vspace{2mm}\\ p_1 \mu_F + p_2 x = \mu \vspace{2mm}\\ p_1 h(|\mu_F|)+p_2 h(x) = B\end{array}\right. \]

We can then simply obtain that \[p_1 = \frac{x-\mu}{x-\mu_F} = \frac{h(x)-B}{h(x)-h(|\mu_F|)} \Rightarrow (x-\mu)(h(x)-h(|\mu_F|))=(x-\mu_F)(h(x)-B)\;. \]

We then remark that $(x-\mu_F)(h(x)-B)= (x-\mu)(h(x)-B) + (\mu - \mu_F)(h(x)-B)$, so a little re-factorization provides

\[(x-\mu)(B-h(\mu_F)) = (\mu - \mu_F)(h(x)-B) \;. \]

Now, this is exactly Equation~\ref{eq::x_to_add} providing that $\bar W = h(\mu_F)$ and $\bar Y=\mu_F$ as all $Z_i$ are constant. The question is to know whether the value of $x$ provided by this simpler equation is larger than the one satisfying Equation~\ref{eq::x_to_add} for a general distribution $F$. I tend to think that yes as it seems to me that the Dirac corresponds to the worst case in terms of difficulty to change a distribution to another of larger mean, but not sure if this is easy to show.


\paragraph{Check of $\cF$} In our previous attempts we wanted to show that $\bP(w^T X \geq \mu, w^T(h(|X-w^T X|)) \leq B) \approx \bP(w^T X \geq \mu, w^Th(|X-\mu|) \leq B)$, why not checking this second condition directly ? If we're right this would not change the magnitude of the probability, but we can discuss this and this is typically something for which experiments could be helpful.

\textcolor{red}{Question: is Sanov theorem enough to conclude about (P3) and/or (P4b)?}

Indeed, if we use Sanov Theorem we get that for any set of distributions $\Gamma$ 
\[\limsup \frac{1}{n} \log \bP(F_n \in \Gamma) \leq - \inf_{P \in \bar \Gamma} \KL(P, F_1)\;, \]

so if $\Gamma=\{P \in \cP: \kinf^\cF(P, \mu_1) \geq x \}$, then $\forall P \in \Gamma$: $\KL(P, F_1) \geq \kinf^\cF(P,\mu_1)\geq x$. Using these results we obtain that 
\[\limsup \frac{1}{n} \log\bP(\kinf^\cF(F_n, \mu_1)\geq x) \leq -x \;.\] 

Actually, we could do the same for (P3), we would define the set $\Gamma_\delta = \{P\in \cP: \kinf^\cF(P, \mu_1) \leq \kinf^\cF(F_k, \mu_1)-\delta \}$, and write that 
\[\limsup \frac{1}{n} \log \bP(F_{k, n} \in \Gamma_\delta) \leq - \inf_{P \in \bar \Gamma} \KL(P, F_k)\;. \]

Now, we remark that if $\kinf^\cF$ is continuous in its first argument with respect to some topology, then $\Gamma_\delta$ is compact under that topology. This means that the infimum is achieved by some distribution in $\Gamma_\delta$, that we call $F_\delta$. Furthermore, $\KL(F_\delta, F_k)>0$ unless $F_\delta=F_k$, which is impossible when $\delta>0$. Hence, there exists some function $I$ such that 

\[\limsup_{n\rightarrow +\infty} \frac{1}{n} \log(\bP\left(\kinf^\cF(F_{k,n}, \mu_1) \leq \kinf^\cF(F_k, \mu_1)-\delta\right)) \leq -I_k(\delta);, \]

where $I_k(\delta)>0$ if $\delta>0$ \textbf{if $\kinf^\cF$ is continuous in the first argument} under some topology. We can use this statement to claim that there exists some sequence $(a_n)_{n \geq 0}$ such that $\lim_{n \rightarrow + \infty} a_n = 0$, and so
\[\bP\left(\kinf^\cF(F_{k,n}, \mu_1) \leq \kinf^\cF(F_k, \mu_1)-\delta\right) \leq e^{-n (I_k(\delta)-a_n)} \leq e^{-n \frac{I_k(\delta)}{2}} \;, \]
for $n$ large enough. If the above use of Sanov Theorem is correct then (P2) is guaranteed.

For (P4b) we can do the same with a sequence $b_n$, and replace $\delta_{\epsilon}$ by $\delta_{\epsilon}/2$ for instance for $n$ large enough by in taking account $b_n$.

\textcolor{red}{Discussion with Odalric: Sanov holds for finite time (with $\leq$) if the level set is convex. This is true in dimension $1$, but not for larger dimensions (this is even the complementary of a convex set). However, we may built a finite or countable union of convex sets and then apply Sanov. This is written in his thesis.}


\textcolor{red}{draft}

Using the same arguments as in e.g \citep{agrawal2020optimal} we can show that a set of distributions $\widetilde \cF$ satisfying a constraint of the type $\forall F \in \widetilde F: \; \bE[g(|X|)]$ for any strictly increasing function $g$ (not necessarily convex here) is compact (as it is closed and tight, using Prohorov's theorem). Furthermore, using Jensen inequality for concave functions, we know that for any r.v $Z$ and $\alpha \geq 1$, $\bE[Z^{1/\alpha}] \leq \bE[Z]^{1/\alpha}$. Hence, if $\cF$ satisfies Definition~\ref{def::uncentered_constraint} for some function $h$ and constant $B$ then 

\[\forall F \in \cF\;,\; \bE_F\left[h(|X|)^\frac{1}{\alpha}\right] \leq \bE_F\left[h(|X|)\right]^\frac{1}{\alpha}\leq B^\frac{1}{\alpha} \;. \]  

We now define the family $\widetilde \cF_\alpha = \{F \in \cP: \; \bE_F\left[h(|X|)^\frac{1}{\alpha}\right]\leq B^\frac{1}{\alpha} \}$, and to implement the following rule in the MED algorithm: for each arm $k$, if $F_{k,n}\notin \widetilde \cF$ sample arm $k$. The choice of the value of $\alpha$ depends on the decay rate of $\bP(F_{k,n} \in \cF)$. We need it to be at least in $o(1/n)$. Using results from \citep{fournier_wasserstein}, we know that this is true at least for $\alpha > 2$. On the other hand we would like to enforce a condition as tight as possible, so we suggest the user (depending on the nature of the function $h$) to choose the smallest $\alpha$ for which the condition holds.


We start with $\kinf^\cF$: we consider the objective function of its dual form $L(\lambda_\star, X)$: $\bP(1/n \sum L(\lambda^\star, X_i) \geq \bE[L(\lambda^\star, X)] - \delta)$, then remark that the variable $Z=L(\lambda^\star, X)$ is light-tailed by remarking that $\bE[e^{Z}] \leq 1+\lambda_1 \Delta$ and $\bE[e^{-Z}]<+\infty$ as $Z$ is lower bounded. Hence, using the Cramér's theorem we know that $Z$ admits a good rate function and so the probability is exponentially decreasing.

\paragraph{Details for (P2)} We denote by $L(\lambda, X, \mu) = \log\left(1-\lambda_1(X-\mu)-\lambda_2(B-h(|X|))\right)$ the function giving the dual form of $\kinf^\cF$, that is $\kinf^\cF(F, \mu)=\max_{\lambda \in \cS}\bE_F[L(\lambda,X, \mu)]$.

Then, we denote by $\lambda^\star= (\lambda_1^\star, \lambda_2^\star)$ the optimal parameters giving $\kinf^\cF(F_k, \mu)$ for some arm $k$ and some $\mu$. We use that 
\[\bP\left(\kinf^\cF(F_{k, n}, \mu) \leq \kinf^\cF(F_k, \mu)-\delta\right) \leq \bP\left(\frac{1}{n}\sum_{i=1}^n L(\lambda^\star, X_i, \mu) \leq \bE[L(\lambda^\star, X_1, \mu)]-\delta\right) \;. \]

Then, we notice that the variable $L(\lambda^*, X, \mu)$ is light-tailed when $X\sim F$ since $\bE[e^{|L(\lambda^*, X, \mu)|}] \leq \bE[e^{-L(\lambda^*, X, \mu)}] + \bE[e^{L(\lambda^*, X, \mu)}]<+\infty$. Hence, by Cramér's theorem (see \citep{large_deviation_book})there exists a rate function $I_k^\cF$ such that \[\bP\left(\frac{1}{n}\sum_{i=1}^n L(\lambda^\star, X_i, \mu) \leq \bE[L(\lambda^\star, X_1, \mu)]-\delta\right) \leq e^{-nI_k^\cF(\delta)} \;,\] 

where $I_k^\cF(x) \geq 0$, and $I_k^\cF(x)=0$ only if $x=0$.

\paragraph{Details} At the beginning of each round, for all $k \in \K$ check if $F_k(t) \in \cF$. Then, pull an arm at random in the set $\{k: F_k(t) \notin \cF\}$, if this set is not empty. We can then decompose the number of pulls of arm $k$ as

\begin{align*}
	\bE[N_k(T)] &\leq 1 + \bE\left[\sum_{t=K+1}^{T-1} \ind(A_{t+1}=k)\right] \\ 
	&\leq 1+ \bE\left[\sum_{t=K+1}^{T-1} \ind(A_{t+1}=k, \cap_{k'=1}^K \{F_{k'}(t) \in \widetilde \cF_\alpha\})\right]+ \bE\left[\sum_{t=K+1}^{T-1} \ind(A_{t+1}=k, F_{k}(t) \notin \widetilde \cF_\alpha)\right] \;. \end{align*}

The second term is classically upper bounded by $\sum_{n=1}^{T} \bP(F_{k,n} \notin \widetilde \cF_\alpha)$, that converges if the probability decays in $o(1/n^\gamma)$ for some $\gamma>1$. When we detail the union bound on the value of $N_1(t)$ to upper bound (F3) it is clear that the event $\ind(F_{1,n} \in \widetilde \cF_\alpha)$ can be propagated in the proof just as $\ind(\mu_{1,n} \leq \mu_1-\epsilon)$. Hence, we obtain 

\[\text{(F3)} \leq \sum_{n=1}^T \bE\left[(c_n e^{n \kinf^\cF(F_n, \mu_1-\epsilon)}-1) \ind(F_{1,n} \in \widetilde \cF_\alpha, \mu_{1, n}< \mu_1-\epsilon) \right] \;. \]

After carefully splitting and handling the term in $\ind(\mu_{1,n}< \mu_1-\epsilon)$ we now have to upper bound 
\begin{equation}\label{eq::F3_uncentered}\sum_{n=1}^T \bE\left[(e^{n \kinf^\cF(F_n, \mu_1-\epsilon)}-1) \ind(F_{1,n} \in \widetilde \cF_\alpha) \right] \;. \end{equation}

We then use that \[F_n \in \widetilde \cF_\alpha \subset \left\{\kinf^\cF(F_n, \mu_1)-\kinf^\cF(F_n, \mu_1-\epsilon) \geq \delta_{\epsilon}\right\} \cap \left\{\kinf^\cF(F_n,\mu_1) \leq C_{B,\mu} \right\}\;,\]

where $C_{B,\mu} < +\infty$ is an unknown but finite constant and $\delta_{\epsilon}>0$ is also unknown but strictly positive \textcolor{red}{(Theorem 12 of \cite{agrawal2020optimal}, tightness of the constraints)}, both thanks to the compactness of $\widetilde \cF_\alpha$. We can then use these results as follow,

\begin{align*}
	&\bE\left[(e^{n \kinf^\cF(F_n, \mu_1-\epsilon)}-1) \ind(F_{1,n} \in \cF) \right]  \\
	& \leq \int_0^{+\infty} \bP\left(\ind(\kinf^\cF(F_n, \mu_1)-\kinf^\cF(F_n, \mu_1-\epsilon) \geq \delta_{\epsilon},\kinf^\cF(F_n,\mu_1) \leq C_{B,\mu})\left(e^{n \kinf^\cF(F_n, \mu_1-\epsilon)}-1)\right)>x \right) dx \\
	& \leq \int_0^{e^{n C_{B,\mu-\epsilon}}-1} \bP\left(e^{n (\kinf^\cF(F_n, \mu_1)-\delta_{\epsilon})}-1>x\right) dx \;, \\
\end{align*}

and we are back to an upper bound that is sufficient to conclude if (P4b) hold.

\paragraph{Clarification on the tightness of constraints} It seems to me that \cite{agrawal2020optimal} prove only that $\lambda_1^\star>0$ if the distribution needs an additional support. Even this does not seem true to me (are we sure the function is convex?). I only agree that if the additional support is not $0$ we can take some mass from it and spread it without any other item and $0$, strictly decreasing the $\KL$. Hence, in that case $\lambda_1^\star=0$ is possible only if the additional support is $0$, which can happen only if $\bE_F\left[\frac{B}{h(|x|)}\right]\leq 1$

We can elaborate for more general case: consider $g$ and $g'$ two densities of distributions $G$ and $G'$, $g=g'$ except on two sets $\cA$ and $\cB$, for which $g'=g+\delta_0$ and $g-\delta_1$ respectively. Then, for any $F$
\begin{align*}
	\KL(F, G) - \KL(F, G') &= \int f \log\left(\frac{g'}{g}\right) \\
	& = \int_\cA f(x) \log\left(1+\frac{\delta_0}{g(x)}\right) \mathrm{d}x + \int_\cB f(x) \log\left(1-\frac{\delta_1}{g(x)}\right) \mathrm{d}x \\
	& \approx \delta_0 \int_\cA \frac{f(x)}{g(x)} \mathrm{d}x - \delta_1 \int_\cB \frac{f(x)}{g(x)} \mathrm{d}x\;.
\end{align*}

If we apply this we $g$ as the density satisfying the $\kinf$ we have that $\frac{f(x)}{g(x)}=1-\lambda_2^\star (B-h(|x|))$, so we have 

\[\KL(F, G) - \KL(F, G') \approx (\delta_0 \bP_F(\cA)-\delta_1 \bP_F(\cB))(1-\lambda_2^\star B) + \lambda_2^\star \left(\delta_0 \int_\cA h(|x|) \mathrm{d}x-\delta_1 \int_\cB h(|x|) \mathrm{d}x\right) \;. \]

If $\lambda_1^\star = 0$ then we have necessarily:

\begin{itemize}
	\item $\bE_F\left[\frac{1}{1-\lambda_2(B-h(|x|))}\right] +p_0 = 1$, with equality if no additional point (hence possible only if this point is $0$). Assume that $x_0$ is added, with mass $p_0$: $x_0$ must be $0$ (remark that the $\kinf$ is same as for bounded distrib).
	\item $\bE_F\left[\frac{\mu-X}{1-\lambda_2(B-h(|x|))}\right] + p_0 x_0 >0$.
	\item $\bE_F\left[\frac{B-h(|X|)}{1-\lambda_2(B-h(|x|))}\right]+ p_0 (B-h(x_0))= 0 \Rightarrow \bE_F\left[\frac{1}{1-\lambda_2(B-h(|x|))}\right] = 1$ (multiplying by $-\lambda_2$ and adding/removing the same amount to get the $1$). 
	\item $\lambda_2 = \frac{1}{B-h(x_0)}$ if $p_0>0$ (comes from above), which implies $\bE_F\left[\frac{B-h(x_0)}{h(x)-h(x_0)}\right] < 1$.
\end{itemize}


\textcolor{blue}{My (possibly) final take: we assume that $\alpha=1$ is sufficient. If $F_{k, n} \in \cF$ then $\kinf^\cF(F_{k, n}, \mu_{F_{k,n}})=0$, and also for $\mu > \mu_{F_{k,n}}$ we have $\kinf^\cF(F_{k, n}, \mu)>0$. Hence, $\lambda_1^\star(\mu)>0$ for $\mu>\mu_{F_{k, n}}$. The family $\cF$ is compact, hence we have the result.}

\textcolor{red}{The result below is still interesting.}

\paragraph{On (A5) for heavy-tailed distributions} If $\bE[X^2]=+\infty$ then we can use an unbiased robust estimate of the mean instead (see below). We can adapt the proof of \cite{bubeck_heavy} for the truncation-based estimator. Consider a sequence $(u_n)_{n \geq 0}$ et further assume that $h(|x|) > x^{1+\delta}$ for some $\delta>0$. Then we consider the estimator $\frac{1}{n} \sum_{i=1}^n X_i \ind(|X_i|\leq u_n)$. Then,

\begin{align*}
	\bP\left(\frac{1}{n} \sum_{i=1}^n X_i \ind(|X_i|\leq u_n) \leq \mu_1-\epsilon\right)  & = 	\bP\left(\frac{1}{n} \sum_{i=1}^n (X_i \ind(|X_i|\leq u_n)-\widetilde \mu_1) \leq (\mu_1-\widetilde \mu_1)-\epsilon \right) \;,
\end{align*}

where $\widetilde \mu_1 = \bE[X \ind(|X|\leq u_n)]$. We first handle the difference between the mean of the truncated and un-truncated variable.

\begin{align*}
	\mu_1 - \widetilde \mu_1 &= \bE\left[X \ind(|X|\geq u_n)\right] \\
	& \leq \bE\left[|X| \ind(|X|\geq u_n) \right] \\
	& \leq \bE\left[\frac{|X|}{h(|X|)} h(|X|)  \ind(|X|\geq u_n) \right] \\
	& \leq \frac{B}{u_n^{\epsilon}} \;. \\
\end{align*}

If $u_n \rightarrow+\infty$ then this quantity tends to $0$, and so for $n \geq n_0$ large enough it holds that 

\[\bP\left(\frac{1}{n} \sum_{i=1}^n X_i \ind(|X_i|\leq u_n) \leq \mu_1-\epsilon)\right)  \leq  	\bP\left(\frac{1}{n} \sum_{i=1}^n (X_i \ind(|X_i|\leq u_n)-\widetilde \mu_1) \leq -\frac{\epsilon}{2} \right)\;. \]

We can then use Bernstein inequality, after remarking that $\bE\left[X^2 \ind(|X|\leq u_n)\right] = \bE\left[\frac{|X|}{h(|X|)} |X| h(|X|)\ind(|X|\leq u_n)\right] \leq \bE\left[|X|^{1-\epsilon} h(|X|)\ind(|X|\leq u_n)\right] \leq B u_n^{1-\epsilon}$.

Then, Bernstein inequality gives us that 

\begin{align*}
	\bP\left(\frac{1}{n} \sum_{i=1}^n (X_i \ind(|X_i|\leq u_n)-\widetilde \mu_1) \leq (\mu_1-\widetilde \mu_1)-\epsilon \right) \leq \exp\left(- \frac{n^2 \frac{\epsilon^2}{8}}{n B u_n^{1-\epsilon} + \frac{1}{3}u_n \epsilon}\right) \;,
\end{align*}

and so the sum of these probabilities converges for instance by taking $u_n = \cO(n)$.

\paragraph{We aim at providing the corresponding NPTS} \textcolor{red}{If too difficult take a semi-bounded support (e.g $[0, +\infty]$).}
\textcolor{red}{Remark: if the empirical distribution belongs to $\cF$ then its support is bounded in $[-h^{-1}(nB), h^{-1}(nB)]$.}

\section{Draft lower bound $h$-NPTS}

\textcolor{blue}{To finish: if additional support is not needed we choose $x=\mu^\star$. then we re-normalize by $1/(1-w_{n+1})$ et obtain the BCP as below without additional support. If $x=x_F^\star$ is needed, then we simply choose to not tilt it's distribution and get the supplementary term corresponding to its expectation in the upper bound of each proba. The impact of the bonus is in $n\leq n_\cF$.}

\textcolor{blue}{Story: (1) we either need $X_{n+1}$ or not. If not, take $X_{n+1}=\mu$. If needed, take the $X_{n+1}$ maximizing the $\kinf$. We now that kinf associated with optimal allocation giving weights blabla to each. The idea is to compute the prob under a change of measure for which this optimal allocation is the expectation. Thanks to the (potential) additional point, the "expectation" lies in the set of allocations that ensure the conditions, which ensures that the event as large prob under this new event.}

We want to lower bound the following:
$$ \text{[BCP]} = \bP\left(\sum_{i=1}^n R_i(X_i-\mu) \geq 0, \sum_{i=1}^n R_i(B-h(|X_i-\mu|)) \geq 0 \right) \;,$$

where $(R_i)_{i\geq 1}$ are i.i.d and follow an exponential distribution $\cE(1)$. We consider an exponential tilting for each of these variables, with the distributions

\[ \frac{\mathrm{d}\bP_{\alpha, \beta}^i}{\mathrm{d}\bP}(R_i) = e^{R_i (\alpha (X_i-\mu) + \beta (B-h(|X_i-\mu|))) + \ell(\alpha, \beta, X_i)} \;, \]

where $\ell(\alpha, \beta, X_i) = \log(1-\alpha(X_i-\mu)-\beta(B-h(|X_i-\mu|)))$. Furthermore, it holds that $\bP_{\alpha, \beta}^i$ is an exponential distribution $\cE(1-\alpha(X_i-\mu)- \beta (B-h(|X_i-\mu|)))$.

We then write the BCP using those exponentially tilted distribution. For simplicity, we use the notations $\sum_{i=1}^n R_i(X_i-\mu)=R^T U$ and $\sum_{i=1}^n R_i(B-h(|X_i-\mu|)) = R^T V$, and $\bP_{\alpha, \beta}= \prod_{i=1}^n\bP_{\alpha, \beta}^i$, and $\bar \cL(\alpha, \beta) = \frac{1}{n}\sum_{i=1}^n \ell(\alpha, \beta, X_i)$.

\begin{align*}
	\text{[BCP]} =& \bE_{\bP}\left[\ind\left(R^T U \geq 0, R^T V \geq 0\right)\right] \\
	= & \bE_{\bP_{\alpha, \beta}}\left[\ind\left(R^T U \geq 0, R^T V \geq 0\right) \prod_{i=1}^n \frac{\mathrm{d}\bP}{\mathrm{d}\bP_{\alpha, \beta}^i}(R_i)\right] \\
	= & \bE_{\bP_{\alpha, \beta}}\left[\ind\left(R^T U \geq 0, R^T V \geq 0\right) e^{- \sum_{i=1}^n \ell(\alpha, \beta, X_i) - \sum_{i=1}^n R_i (\alpha (X_i-\mu)+ \beta (B-h(|X_i-\mu|)))}\right] \\
	\geq &  e^{-n \bar \cL(\alpha, \beta) - \alpha y - \beta z} \times  \bE_{\bP_{\alpha, \beta}}\left[\ind\left(y \geq R^T U \geq 0, z \geq R^T V \geq 0\right)\right] \\
	\geq &   e^{-n \bar \cL(\alpha, \beta) - \alpha y - \beta z} \times \left(1- \underbrace{\bP_{\alpha, \beta}(R^T U \leq 0)}_{p_1} - \underbrace{\bP_{\alpha, \beta}(R^T V \leq 0)}_{p_2} - \underbrace{\bP_{\alpha, \beta}(R^T U \geq y)}_{p_3}- \underbrace{\bP_{\alpha, \beta}(R^T V \geq z)}_{p_4}\right) \;.
\end{align*}


We can already obtain the exponential term of the bound from this expression. First, we use from \citep{agrawal2019optimal} that for the un-centered condition it must hold that $\alpha \leq \alpha_M \coloneqq \frac{1}{h^{-1}(B)-\mu}$ and $\beta \leq \beta_M \coloneqq \frac{1}{B-h(\mu)}$ (resp. $\frac{1}{h^{-1}(B)}$ and $\frac{1}{B}$ for the centered case). Hence, to obtain the right dependency in $\delta$ we simply choose $y=\frac{\delta}{2\alpha_M}n$ and $z = \frac{\delta}{2\beta_M}n$. Then, using the notation $(\alpha_F^\star, \beta_F^\star)=\aargmax \bar \cL(\alpha, \beta)$, we use that for any choice of $(\alpha, \beta)$ it holds that $\bar \cL(\alpha, \beta)\leq \bar \cL(\alpha_F^\star, \beta_F^\star)$. Hence, we can write that 

\[\text{[BCP]}  \geq \exp\left(-n (\bar \cL(\alpha_F^\star, \beta_F^\star)+\delta)\right) \times \left(1-p_1-p_2-p_3-p_4\right)\;. \]

We directly remark that the bound becomes meaningful when the sum of probabilities is smaller than $1$, and to complete the proof we only need to show that there exists a universal constant $n_\cF$ such that for $n \geq n_\cF$ it is smaller than $1/2$. We now use the Chernoff method and properties of the exponential distribution to upper bound each of the probabilities $(p_i)_{i \in [4]}$. Starting with $p_1$, for any $\lambda>0$ it holds that

\begin{align*}
	p_1 & = \bP_{\alpha, \beta}\left(\sum_{i=1}^n R_i (X_i -\mu) \leq 0 \right) \\
	& = \bP_{\alpha, \beta}\left(e^{-\lambda \sum_{i=1}^n R_i (X_i -\mu) }\geq 1\right) \\
	& \leq \prod_{i=1}^n \bE_{\bP^i_{\alpha, \beta}} \left[e^{-\lambda R_i (X_i -\mu)} \right] \\
	& \leq \prod_{i=1}^n \left( 1-\alpha(X_i-\mu)-\beta(B-h(|X_i-\mu|))\right) \prod_{i=1}^n \frac{1}{1-(\alpha-\lambda)(X_i-\mu)-\beta(B-h(|X_i-\mu|))} \\
	& = \exp\left(-n \left(\bar \cL(\alpha-\lambda, \beta) - \bar \cL(\alpha, \beta)\right) \right) \;.
\end{align*}

We can then perform the exact same steps for $p_2$, $p_3$ and $p_4$. We could consider different variables $(\lambda_i)_{i\in[4]}$, but for simplicity we write all the bounds with $\lambda$:

\begin{align*}
	p_2 & \leq \exp\left(-n \left(\bar \cL(\alpha, \beta-\lambda) - \bar \cL(\alpha, \beta)\right) \right) \;, \\
	p_3 & \leq \exp\left(-n \left(\lambda \frac{\delta}{2\alpha_M} - \left(\bar \cL(\alpha, \beta) - \bar \cL(\alpha+\lambda, \beta)\right) \right)\right) \;, \\
	p_4 & \leq \exp\left(- n \left( \lambda \frac{\delta}{2\beta_M} -\left(\bar \cL(\alpha, \beta) - \bar \cL(\alpha, \beta+ \lambda)\right) \right) \right) \;. \\
\end{align*}

We see that $(\alpha, \beta)= (\alpha_F^\star, \beta_F^\star)$ then the bounds for $p_1$ and $p_2$ are vacuous. We need to choose $\alpha>\alpha_F^\star$ and $\beta>\beta_F^\star$ so that $p_1$ and $p_2$ can be smaller than $1$. Then, in order to make $p_3$ and $p_4$ small too we need to choose $(\alpha, \beta)$ close enough to the optimal parameters so that the gradient of $\bar \cL$ is small. Indeed, using the concavity and differentiability of $\bar \cL$, and that $\alpha > \alpha_F^\star$ and $\beta > \beta_F^\star$ we obtain

\[ \bar \cL(\alpha, \beta) - \bar \cL(\alpha+\lambda, \beta) \leq \lambda \left| \frac{\partial \bar \cL}{\partial \alpha} (\alpha+\lambda, \beta)\right| \;, \quad \bar \cL(\alpha, \beta) - \bar \cL(\alpha, \beta+\lambda) \leq \lambda \left| \frac{\partial \bar \cL}{\partial \beta} (\alpha, \beta+\lambda)\right| \;. \]

Plugging this result in the upper bound, we obtain that

\begin{align*}
	p_3 & \leq \exp\left(- n\lambda  \left(\frac{\delta}{2\alpha_M} - \left| \frac{\partial \bar \cL}{\partial \alpha} (\alpha+\lambda, \beta)\right| \right) \right) \;, \\
	p_4 & \leq \exp\left(- n\lambda \left(\frac{\delta}{2\beta_M} - \left| \frac{\partial \bar \cL}{\partial \beta} (\alpha, \beta+\lambda)\right| \right) \right) \;. \\
\end{align*}
We now choose $(\alpha, \beta, \lambda)$ in order to get exponentially decreasing upper bounds. Considering a parameter $\lambda\coloneqq \lambda_F$, we simply define $\alpha = \alpha_F^\star+\lambda_F$ and $\beta=\beta_F^\star+\lambda_F$. We then use the continuity of the partial derivatives of $\bar \cL$ and that $\frac{\partial \bar \cL}{\partial \alpha} (\alpha^\star, \beta^\star)=0$ and $\frac{\partial \bar \cL}{\partial \beta} (\alpha^\star, \beta^\star)=0$, to tune the parameter $\lambda_F$ as follow: 

\[\lambda_F = \max \left\{\lambda\geq 0 : \max\left\{\left|\frac{\partial \bar \cL}{\partial \alpha} (\alpha_F^\star+2\lambda, \beta_F^\star+\lambda)\right|, \left|\frac{\partial \bar \cL}{\partial \beta} (\alpha_F^\star+\lambda, \beta_F^\star+2\lambda)\right| \right\} \leq \frac{\delta}{4\min\{\alpha_M, \beta_M\}}\right\}\;. \]

The continuity of the derivatives ensure that $\lambda_F>0$. Thanks to this choice, both $p_3$ and $p_4$ can be upper bounded by $\exp\left(-n c_F^{(3)}\right)$, with $c_F^{(3)} = \frac{\delta}{4 \min\{\alpha_M, \beta_M\}}$. Then, we simply obtain that $p_1 \leq \exp\left(-n c_F^{(1)}\right)$ and $p_2 \leq \exp\left(-n c_F^{(2)}\right)$ with 

\begin{align*} 
	c_F^{(1)} &= \bar \cL(\alpha_F^\star, \beta_F^\star+\lambda_F) - \bar \cL(\alpha_F^\star+\lambda_F, \beta_F^\star+\lambda_F)> 0  \;,\\
	c_F^{(2)}&=\bar \cL(\alpha_F^\star+\lambda_F, \beta_F^\star) - \bar \cL(\alpha_F^\star+\lambda_F, \beta_F^\star+\lambda_F)> 0 \;.
\end{align*}

From this step, we obtain the desired bound $p_1+p_2+p_3+p_4\leq 1/2$ for instance if  
\[n \geq n_F \coloneqq \frac{\log(8)}{\min_{i \in [4]} c_F^{(i)}}  \;. \]

To conclude, we need to remove the dependency of this result in the empirical distribution: as a consequence of Berge maximum theorem \citep{berge1997topological}, the mappings $F\in \cF \mapsto c_F^{(1)}$ and $F\in \cF \mapsto c_F^{(2)}$ are continuous, and as a consequence the mapping $F\in \cF \mapsto n_F$ is also continuous. Using the compactness of the set $\cF$, we obtain the existence of a constant $n_\cF = \max_{F \in \cF} n_F \in \N$ satisfying 

\[\forall n \geq n_\cF \;, \; \text{[BCP]} \geq \frac{1}{2} \exp\left(-n (\bar \cL(\alpha_F^\star, \beta_F^\star)+\delta)\right) \;. \] 

This gives the first part of our result, with a lower bound valid for large enough sample sizes.



\textcolor{blue}{BEFORE CHANGING MY MIND}

\textcolor{blue}{I am still sure about if the tilting for $n+1$ should try to reach $\Lambda_{\alpha, \beta}(\widetilde F_n, \mu)$, where $(\alpha, \beta)$ are taken close to what gives the optimal value for $\widetilde F_n$, and $\widetilde F_n$ is the cdf including the additional support. \\
	If we allow $X_{n+1}$ then in $(\alpha_\star, \beta_\star)$ our definition of $g_{\alpha, \beta}^i$ gives $+\infty$. \\
	I think we should indeed take $\widetilde \alpha, \widetilde \beta$}

\paragraph{First step: existence of weights satisfying the constraints} We first prove that, thanks to the extra point added to the support, conditions inside the BCP can be reached by some allocation of the weights. To formalize this, considering two parameters $(\alpha, \beta)$ we use the notation \[\forall i \in \{1,\dots, n\}: \; g_{\alpha, \beta}^i = \frac{1}{n}\frac{1}{1-\alpha(X_i-\mu)-\beta(B-h(|X_i-\mu|))}\;,\]
and $g_{(\alpha, \beta)}^{n+1} = \max \{1/n, 1-\sum_{i=1}^n g_{\alpha, \beta}^i\}$. We now define the set $\cS_2$ of parameters $(\alpha, \beta)$ such that
\[\left\{ \begin{array}{ll}
&\Lambda_{(\alpha, \beta)}(F_n, \mu) = \frac{1}{n} \sum_{i=1}^n -\log(ng_{\alpha, \beta}^i)\geq 0 \;,\\
&\sum_{i=1}^{n+1} g_{\alpha, \beta}^i X_i \geq \mu  \\
&\sum_{i=1}^{n+1} g_{\alpha, \beta}^i h(|X_i-\mu|) \leq B  \\
\end{array} \right.
\]

The key argument here is that adding the potential extra point in the support makes the set $\cS_2$ non-empty, since at least $(\alpha_{F_n}^\star, \beta_{F_n}^\star) \in \cS_2$, but furthermore by continuity of each function there exists some $\epsilon_{F_n}>0$ such that $\cS_2$ contains the set $\cB(\alpha_{F_n}^\star, \beta_{F_n}^\star, \epsilon_{F_n})\coloneqq \{\alpha \in [\alpha_{F_n}^\star, \alpha_{F_n}^\star+\epsilon_{F_n}], \beta \in [\beta_{F_n}^\star, \beta_{F_n}^\star+\epsilon_{F_n}] \}$. 

\paragraph{Second step: Exponential tilting} Let us consider any $(\alpha, \beta) \in \cS_2$. We consider a change of measure, known as exponential tilting. We choose a measure $\bP_{\alpha, \beta}=\prod_{i=1}^{n+1}\bP_{\alpha, \beta}^i$, such that for any $i \in \{1, \dots, n+1\}$, under $\bP_{\alpha, \beta}^i$ it holds that 
\[\forall i \in \{1,\dots, n\}\;, \; \bE_{\bP_{\alpha, \beta}}[R_i] = n g_{\alpha, \beta}^i \Rightarrow \left\{\begin{array}{ll} 
\bE_{\bP_{\alpha, \beta}}\left[\sum_{i=1}^{n+1} R_i (X_i-\mu)\right] \geq 0 \\
\bE_{\bP_{\alpha, \beta}}\left[\sum_{i=1}^{n+1} R_i (B-h(|X_i-\mu|))\right] \leq 0 \\	
\end{array} \right. \]

This can be done by defining $\bP_{\alpha, \beta}^i$ as follows,

\[ \frac{\mathrm{d}\bP_{\alpha, \beta}^i}{\mathrm{d}\bP}(R_i) = e^{R_i (\alpha (X_i-\mu) + \beta (B-h(|X_i-\mu|))) + \ell(\alpha, \beta, X_i)} \;,\; \text{with} \quad \ell(\alpha, \beta, X_i) = \log(1/(n g_{\alpha, \beta}^i)) \;. \]

Furthermore, we remark that $\bP_{\alpha, \beta}^i$ is still an exponential distribution, with parameter $1/(ng_{\alpha, \beta}^i)$. We now re-write the BCP in terms of this new measure. For the simplicity of notation, we define 
\[\left\{\begin{array}{ll} 
& \sum_{i=1}^n R_i(X_i-\mu)=R^T U \;, \\
\text{and } & \sum_{i=1}^n R_i(B-h(|X_i-\mu|)) = R^T V \;. 	
\end{array} \right. \] 

We now defined all the elements that allow to obtain our first result, re-writing the BCP in terms of the tilting distribution. For any $(\alpha,\beta) \in \cS_2$, we obtain

\begin{align*}
	\text{[BCP]} =& \bE_{\bP}\left[\ind\left(R^T U \geq 0, R^T V \geq 0\right)\right] \\
	= & \bE_{\bP_{\alpha, \beta}}\left[\ind\left(R^T U \geq 0, R^T V \geq 0\right) \prod_{i=1}^n \frac{\mathrm{d}\bP}{\mathrm{d}\bP_{\alpha, \beta}^i}(R_i)\right] \\
	= & \bE_{\bP_{\alpha, \beta}}\left[\ind\left(R^T U \geq 0, R^T V \geq 0\right) e^{- \sum_{i=1}^n \ell(\alpha, \beta, X_i) - \sum_{i=1}^n R_i (\alpha (X_i-\mu)+ \beta (B-h(|X_i-\mu|)))}\right] \\
	= & (n g_{\alpha, \beta}^{n+1}) \times e^{-n \Lambda_{\alpha, \beta}(F_n, \mu)} \times \bE_{\bP_{\alpha, \beta}}\left[\ind\left(R^T U \geq 0, R^T V \geq 0\right) e^{- \alpha R^T U - \beta R^T V}\right] \;. \\
\end{align*}

Interestingly, this simple transform already exhibit the main exponential term that we want to obtain, remarking that for any choice of $(\alpha, \beta)$ it holds that $e^{-n \Lambda_{\alpha, \beta}(F_n, \mu)} \geq e^{-n \Lambda_{\alpha_{F_n}^\star, \beta_{F_n}^\star}(F_n, \mu)}$. Furthermore, the truncation of $g_{n+1}$ to $1/n$ ensures that $ng_{\alpha, \beta}^{n+1}$. We could make this truncation without additional difficulty in the proof since we do not formally require $\sum_{i=1}^{n+1} g_{\alpha, \beta}^{i}=1$, and we are only interested in the can adjust $X_{n+1}$ to keep the same expectation for $R^T U$ and $R^T V$ (we recall that $X_{n+1}$ can be arbitrary). For instance, when $\sum_{i=1}^{n+1} g_{\alpha, \beta}^{i}=1$ (i.e. the additional support is not needed) then $X_{n+1}=\mu+h^{-1}(B)$ can help to meet the two constraints, and we do not change .

We now handle the exponential term inside the expectation by first using from \citep{agrawal2019optimal} (slightly adapting their proof to get the centered condition instead of un-centered) that it must hold that $\alpha \leq \alpha_M \coloneqq \frac{1}{h^{-1}(B)}$ and $\beta \leq \beta_M \coloneqq \frac{1}{B}$ (resp. $\frac{1}{h^{-1}(B)-\mu}$ and $\frac{1}{B-h(\mu)}$ for the centered case). Then, for any $\delta >0$ we consider the event $\{R^T U \leq  \frac{\delta}{2 \alpha_M}n , R^T V \leq \frac{\delta}{2\beta_M} n \}$, and write that

\begin{equation}\label{eq::lower_bcp_npts_intermediate}
\text{[BCP]} \geq  e^{-n (\Lambda_{\alpha, \beta}(F_n, \mu)+\delta)} \times  \bP_{\alpha, \beta}\left(0 \leq R^T U\leq n\frac{\delta}{2\alpha_M}, 0 \leq R^T V \leq n\frac{\delta}{2\beta_M}\right)
\end{equation}
Interestingly, \eqref{eq::lower_bcp_npts_intermediate} holds for any choice of $(\alpha, \beta) \in \cS_2$. We now introduce the notation 

\[P_{\alpha, \beta} = \bP_{\alpha, \beta}\left(0 \leq R^T U\leq n\frac{\delta}{2\alpha_M}, 0 \leq R^T V \leq n\frac{\delta}{2\beta_M}\right) \;, \]

and simply write that 
\begin{align*}
	P_{\alpha, \beta} \geq 1- \underbrace{\bP_{\alpha, \beta}(R^T U \leq 0)}_{p_1} - \underbrace{\bP_{\alpha, \beta}(R^T V \leq 0)}_{p_2} - \underbrace{\bP_{\alpha, \beta}(R^T U \geq y)}_{p_3}- \underbrace{\bP_{\alpha, \beta}(R^T V \geq z)}_{p_4} \;.
\end{align*}

The rest of the proof consists in showing that for $n$ large enough, $P_{\alpha, \beta}\geq 1/2$. We now use the Chernoff method and properties of the exponential distribution to upper bound each of the probabilities $(p_i)_{i \in [4]}$. Starting with $p_1$, for any $\lambda>0$ it holds that


==> previous_version_lb.tex <==
\subsection{Lower bound: $h$-moment condition \textcolor{red}{PREVIOUS VERSION}}

In this section we prove the lower bounds on the BCP in Lemma~\ref{lem::bounds_bcp}. We recall that for observations $X_1,\dots, X_n$ the BCP is expressed as 

\[\text{[BCP]} \geq \bP_{w \sim \cD_{n+1}}\left(\exists X_{n+1} \geq \mu^\star: \; \sum_{i=1}^{n+1} w_i X_i\geq \mu^\star, \sum_{i=1}^{n+1} w_i h(|X_i-\mu|)\leq B \right) \;.\]

To provide a lower bound on this quantity we can consider a carefully chosen single value for $X_{n+1}$, that will be motivated later by the following quantity: given some parameters $\alpha, \beta, \mu, B$ and a cdf $F_n$, we define 

\[\Lambda_{\alpha, \beta}(F_n, \mu, B) = \bE_{F_n}\left[\log\left(1-\alpha(X-\mu)-\beta(B-h(|X-\mu|))\right)\right] \;. \]

After rewriting the BCP in terms of exponential random variables (instead of Dirichlet variables), we now want to lower bound the following:
$$ \text{[BCP]} = \bP_{R_1\sim \epsilon(1),\dots, R_n \sim \epsilon(1)}\left(\sum_{i=1}^{n+1} R_i(X_i-\mu) \geq 0, \sum_{i=1}^{n+1} R_i(B-h(|X_i-\mu|)) \geq 0 \right) \;,$$

where $(R_i)_{i\geq 1}$ are i.i.d and follow an exponential distribution $\cE(1)$. To lower bound this quantity, we will perform a change of measure for each variable $R_i$. In particular, we propose to consider a variable that has expectation $G_i$, for some $(G_i)_{i=1,\dots, n+1}$. We can do that by choosing exponential random variables $\epsilon\left(\frac{1}{G_i}\right)$. This technique is known as exponential tilting. If $\widetilde f_i$ denotes the density of this random variable and $f$ denotes the density of the distribution $\epsilon(1)$, it holds that 

\[\forall x \geq 0 : \; \frac{f_i(x)}{\widetilde f_i(x)} = G_i e^{- \left(1-\frac{1}{G_i} \right) x}
\]

We further denote by and $\bP $and $\widetilde \bP$ their respective product. Using the notation $R^T U = \sum_{i=1}^{n+1} R_i (X_i-\mu)$ and $R^T V = \sum_{i=1}^{n+1}R_i(B-h(|X_i-\mu|))$, we now re-write the BCP using the distributions of densities $\widetilde f_i$, 

\begin{align*}
	\text{[BCP]} =& \bE_{\bP}\left[\ind\left(R^T U \geq 0, R^T V \geq 0\right)\right] \\
	= & \bE_{\widetilde \bP}\left[\ind\left(R^T U \geq 0, R^T V \geq 0\right) \prod_{i=1}^{n+1} \frac{f_i(R_i)}{\widetilde f_i(R_i)}\right] \\
	= & \prod_{i=1}^{n+1} G_i \times \bE_{\widetilde \bP}\left[\ind\left(R^T U \geq 0, R^T V \geq 0\right) e^{-\sum_{i=1}^{n+1} \left(1-\frac{1}{G_i}\right)R_i}\right] \\
	= & G_{n+1} e^{- \sum_{i=1}^{n} \log\left(\frac{1}{G_i}\right)} \bE_{\widetilde \bP}\left[\ind\left(R^T U \geq 0, R^T V \geq 0\right) e^{-\sum_{i=1}^{n+1} \left(1-\frac{1}{G_i}\right)R_i}\right] \;.\\
\end{align*}
Interestingly, we recognize before the expectation a quantity of the form $e^{-n\KL(F_n, g)}$, if $\frac{1}{n}\sum_{i=1}^n G_i \leq 1$ so $(G_i/n)_{i \in [n]}$ can define a probability distribution supported on $(X_1,\dots, X_n)$ and at most one extra point. Our objective is to get the term $\max_{(\alpha, \beta)}\Lambda_{\alpha, \beta}(F_n, \mu, B)+\delta$ from this exponential term before the expectation, and to show that the expectation can be lower bounded by a constant. To do that, we consider stronger constraints by defining two arbitrary constants $\eta_1>0, \eta_2>0$, and consider for $i\leq n+1$

\[ G_i =  \frac{1}{1-\alpha(X_i-\mu-\eta_1)- \beta (B-\eta_2 - h(|X_i-\mu|))} \;, \] 
for some constants $(\alpha, \beta)$. We still center the $h$-moment in $\mu$, as we want the objective inside the expectation to be strictly easier to reach with our change of distribution. However, we keep the notation $\Lambda_{\alpha, \beta}$ with a slight abuse for simplicity. If $(\alpha, \beta)= (\alpha^\star, \beta^\star) \coloneqq \aargmax  \Lambda_{\alpha, \beta}(F_n, \mu+\eta_1, B-\eta_2)$, then $(G_i/n)_{i\in [n]}$ defines a distribution supported on $(X_1, \dots, X_n)$ and at most one extra point, with expectation $\mu+\eta_1$ and $h$-moment (centered in $\mu$) $B-\eta_2$. Furthermore, if this extra-point $X_{n+1}$ is needed, we know from \citep{agrawal2020optimal} that it satisfies 

\[1-\alpha(X_{n+1}-\mu-\eta_1)-\beta(B-\eta_2-h-(|X_{n+1}-\mu|)) = 0 \]

As $x \mapsto 1-\alpha(x-\mu-\eta_1)-\beta(B-\eta_2-h-(|x-\mu|))$ is strictly positive otherwise, this motivates the choice of $X_{n+1}$ in the BCP as follows,

\begin{equation}\label{eq::X_n+1} X_{n+1} = \inf_{x\in \R} \{1-\alpha_{F_n}^\star(x-\mu-\eta_1)- \beta_{F_n}^\star (B-\eta_2 - h(|x-\mu|))\} \;. \end{equation}

Interestingly, this value of $X_{n+1}$ ensures that $\alpha_{F_n}^\star = \beta_{F_n}^\star \times  \text{sgn}(X_{n+1}-\mu) h'(X_{n+1}-\mu)$. Furthermore, thanks to the convexity of $h$ and that $h'(0)=0$, we are sure that if $X_{n+1}>\mu$ (which is the case due to $F_n \in \cF$ and $\bE_{F_n}[X] \leq \mu < \mu+\eta_1$) then either $\alpha_{F_n}^\star = \beta_{F_n}^\star = 0$ (impossible since $F_n$ does not meet the constraints), or they are linearly dependent (and hence simultaneously large or small). In addition, this choice ensures in any case it will hold that $G_{n+1}\geq 1$, or in words $X_{n+1}$ is necessarily ``helping" to reach the objectives so its weight will be increased by the change of measure if $(\alpha, \beta)$ is not far from $(\alpha_{F_n}^\star, \beta_{F_n}^\star)$. Thanks to this observation, we now write that 

\[ \text{[BCP]} \geq   e^{-n \Lambda_{\alpha, \beta}(F_n, \mu+\eta_1, B-\eta_2)} \times \bE_{\widetilde \bP}\left[\ind\left(R^T U \geq 0, R^T V \geq 0\right) e^{- \alpha R^T \widetilde U - \beta R^T \widetilde V}\right] \;,
\]

with $\widetilde U = (X_1-\mu-\eta_1, \dots, X_{n+1}-\mu-\eta_1)$ and $\widetilde V = (B-\eta_2-h(|X_1-\mu|), \dots, B-\eta_2-h(|X_{n+1}-\mu|)$, and after remarking that for all $i$,
\[1- \frac{1}{G_i}= \alpha (X_i-\mu-\eta_1) + \beta (B-\eta_2-h(|X_i - \mu|)).\]

We now handle the exponential term inside the expectation by first using from \citep{agrawal2019optimal} (their proof can be simply adapted to get the centered condition instead of un-centered) that $\alpha$ and $\beta$ ar both upper bounded respectively by some constants $\alpha_M $ and $\beta_M$ depending only on $\mu+\eta_1$ and $B-\eta_2$. Then, for any $\delta >0$ we write that 
\[	\text{[BCP]} \geq  e^{-n \left(\Lambda_{\alpha, \beta}(F_n, \mu+\eta_1, B-\eta_2)+\frac{\delta}{2}\right)} \times P_{\alpha, \beta} \;,
\]

where we defined 
\[P_{\alpha, \beta} = \widetilde \bP\left(R^T U \geq 0, R^T V \geq 0, R^T \widetilde U \leq n\frac{\delta}{4\alpha_M}, R^T \widetilde V \leq n\frac{\delta}{4\beta_M}\right) \;.
\]

We now re-write $P_{\alpha, \beta}$ as

\begin{align*}
	P_{\alpha, \beta} \geq 1- \underbrace{\bP_{\alpha, \beta}(R^T U \leq 0)}_{p_1} - \underbrace{\bP_{\alpha, \beta}(R^T V \leq 0)}_{p_2} - \underbrace{\bP_{\alpha, \beta}(R^T \widetilde U \geq n\frac{\delta}{4\alpha_M})}_{p_3}- \underbrace{\bP_{\alpha, \beta}(R^T \widetilde V \geq n\frac{\delta}{4\beta_M})}_{p_4} \;.
\end{align*}

The rest of the proof consists in showing that for $n$ large enough, $P_{\alpha, \beta}\geq 1/2$. We will use the Chernoff method and properties of the exponential distribution to upper bound each of the probabilities $(p_i)_{i \in [4]}$. Before that, we explain the interest of considering $\mu+\eta_1$ and $B-\eta_2$: under this choice these probabilities represent a deviation of each vector from their mean. Indeed, if we chose $(\alpha, \beta)=(\alpha_{\widetilde F_n}^\star, \beta_{\widetilde F_n}^\star)$ (where $\widetilde F_n$ is the empirical distribution including $X_{n+1}$) we would have 
\[\bE_{\alpha, \beta}[R^T U] = (n+1) \eta_1 \;, \quad \bE_{\alpha, \beta}[R^T V] = (n+1) \eta_2 \; \quad \bE_{\alpha, \beta}[R^T \widetilde U] = 0 \;,\; \text{and} \quad \bE_{\alpha, \beta}[R^T \widetilde V] = 0  \;,
\]
and hence even for $(\alpha, \beta)$ close enough to these values we would obtain expectations that are relatively far from respectively $0$ and $n \frac{\delta}{2\max\{\alpha_M, \beta_M\}}$. However, if we set $\eta_1=\eta_2=0$, even with $(\alpha, \beta)=(\alpha_{\widetilde F_n}^\star, \beta_{\widetilde F_n}^\star)$ the first two expectations would be $0$. In that case, upper bounding $p_1$ and $p_2$ would have required more sophisticated tools, and our intuition is that it may not be possible to reach a constant upper bound for $\sum p_i$ in that case.

From now on, we will use the function $\widetilde \Lambda: (\alpha, \beta) \mapsto \Lambda_{\alpha, \beta}(\widetilde F_n, \mu+\eta_1, B-\eta_2)$, omitting other dependencies in the parameters in the notation for simplicity. Starting with $p_1$, for any $\lambda_1>0$ it holds that

\begin{align*}
	p_1 & = \bP_{\alpha, \beta}\left(\sum_{i=1}^{n+1} R_i (X_i -\mu) \leq 0 \right) = \bP_{\alpha, \beta}\left(e^{-\lambda_1 \sum_{i=1}^{n+1} R_i (X_i -\mu) }\geq 1\right) \\
	& \leq \prod_{i=1}^{n+1} \bE_{\alpha, \beta} \left[e^{-\lambda_1 R_i (X_i -\mu)} \right] \\
\end{align*}

We then use that for all $i \in [n+1]$, $R_i \sim \epsilon(1/G_i)$, so
\begin{align*}
p_1	& \leq \prod_{i=1}^{n+1} \left( 1-\alpha(X_i-\mu-\eta_1)-\beta(B-\eta_2-h(|X_i-\mu|))\right) \\
	& \quad \times  \prod_{i=1}^{n+1} \frac{1}{1-\alpha(X_i-\mu-\eta)-\beta(B-\eta_2-h(|X_i-\mu|)) + \lambda_1(X_i-\mu)} \\
	&  =e^{(n+1)\widetilde \Lambda(\alpha, \beta)} \times  \prod_{i=1}^{n+1} \frac{1}{1-(\alpha-\lambda_1)(X_i-\mu-\eta)-\beta(B-\eta_2-h(|X_i-\mu|)) + \lambda_1 \eta_1} \;, \\
\end{align*}

that we can re-write by factorizing by $1+\lambda_1\eta_1$ the denominators as 
\begin{equation*}
	p_1 \leq e^{-(n+1) \log(1+\lambda_1 \eta_1)}e^{(n+1) \left(\widetilde \Lambda(\alpha, \beta) - \widetilde \Lambda\left(\frac{\alpha-\lambda_1}{1+\lambda_1 \eta_1},\frac{\beta}{1+\lambda_1 \eta_1}\right)\right)} \;.
\end{equation*}

We then use that for  $x <1$, $\log(1+x) \geq x - x^2/2 \geq x/2 $. Hence, the left-hand exponential terms can be directly replaced respectively by $e^{-(n+1)\frac{\lambda_1 \eta_1}{2}}$. We can then perform the exact same steps for $p_2$, considering a parameter $\lambda_2>0$ and hence obtain that 

\begin{align}
	p_1 \leq e^{-(n+1) \frac{\lambda_1 \eta_1}{2}}e^{(n+1) \left(\widetilde \Lambda(\alpha, \beta) - \widetilde \Lambda\left(\frac{\alpha-\lambda_1}{1+\lambda_1 \eta_1},\frac{\beta}{1+\lambda_1 \eta_1}\right)\right)} \;.\label{eq::ub_p1} \\
	p_2 \leq e^{-(n+1) \frac{\lambda_2 \eta_2}{2}} e^{(n+1) \left(\widetilde \Lambda(\alpha, \beta) - \widetilde \Lambda\left(\frac{\alpha}{1+\lambda_2 \eta_2},\frac{\beta-\lambda_2}{1+\lambda_2 \eta_2}\right)\right)} \;. \label{eq::ub_p2}
\end{align}

Then, applying the same Chernoff method to $p_3$ and $p_4$ gives for some $\lambda_3>0, \lambda_4>0$ that

\begin{align}
	p_3 & \leq e^{-(n+1)\lambda_3 \frac{\delta}{4\alpha_M}} \times e^{(n+1) \left(\widetilde \Lambda(\alpha, \beta) - \widetilde \Lambda(\alpha+\lambda_3, \beta)\right)} \;,\label{eq::ub_p3} \\
	p_4 & \leq e^{-(n+1)\lambda_4 \frac{\delta}{4\beta_M}} \times e^{(n+1) \left(\widetilde \Lambda(\alpha, \beta) - \widetilde \Lambda(\alpha, \beta+\lambda_4)\right)}\label{eq::ub_p4}\;.
\end{align}

The intuition for the rest of the proof is the following: we can choose $(\alpha, \beta)$ close to $(\alpha_{\widetilde F_n}^\star, \beta_{\widetilde F_n}^\star) \coloneqq \aargmax \widetilde \Lambda(\alpha, \beta)$, so that all the gradients of $\widetilde \Lambda$ in a large enough neighborhood of $(\alpha, \beta)$ are arbitrarily close to $0$. In that case, the exponentially decreasing (left-hand) term will be dominating all the inequalities. 

First, motivated by Eq~\eqref{eq::X_n+1}, we now choose to link all the parameters as follow
\[\lambda_1 = \lambda_2 h'(X_{n+1}-\mu) \;, \quad \lambda_3 =\lambda_4 h'(X_{n+1}-\mu) \text{ , and} \quad \eta_2=h'(X_{n+1}-\mu)\eta_1 \;,\]

Then, we use that $\bE_{F_n}[X]<\mu$ and that the change of measure was targeting a mean $\mu+\eta_1$ and a moment condition holding with $B-\eta_2$, to obtain that for any distribution $F_n \in \cF$ it holds that $\beta^\star>0$ and $\alpha^\star>0$. Thanks to the compactness of $\cF$ and the continuity of the mapping $F \rightarrow (\alpha_F^\star, \beta_F^\star)$ (as a consequence of Berge's theorem \citep{berge1997topological}) we deduce the existence of minimum parameters $(\alpha_m, \beta_m)$ (omitting the dependency in $\mu, B, \eta_1, \eta_2$ in the notation for simplicity) such that \[\forall F \in \cF \;, \quad \alpha_F^\star \geq \alpha_m \quad \text{and} \quad \beta_F^\star \geq \beta_m\;.\] On the other hand, in some difficult cases $(\alpha_{\widetilde F_n}^\star, \beta_{\widetilde F_n}^\star)$ may be arbitrarily close to their upper boundary (this corresponds to the ``worst cases" for $F_n$, e.g. if all observations are below $\mu-\eta_1-h^{-1}(B)$). Motivated by these observations, we choose \[(\alpha_{\widetilde F_n}^\star, \beta_{\widetilde F_n}^\star)=(\alpha + \lambda_3, \beta+\lambda_4).\] 
 
Thanks to this choice, we are sure to obtain a range of acceptable values for all our parameters that is at least $[\alpha_{\widetilde F_n}^\star -\alpha_m, \alpha_{\widetilde F_n}^\star]\times [\beta_{\widetilde F_n}^\star-\beta_m, \beta_{\widetilde F_n}^\star]$. Our choice for $(\alpha, \beta)$ directly ensures that \[p_3 \leq e^{-(n+1)\lambda_4 h'(X_{n+1}-\mu)\frac{\delta}{4\alpha_M}} \leq e^{-(n+1)\lambda_4 h'(\eta_1)\frac{\delta}{4\alpha_M}} \quad \text{and} \quad p_4 \leq e^{-(n+1)\lambda_4 \frac{\delta}{4\beta_M}}.\] We now consider $p_1$ and $p_2$. The concavity of $\widetilde \Lambda$ ensures that for any $(\alpha, \beta), (\alpha', \beta')$ it holds that

\begin{equation}\label{eq::concavity} \widetilde \Lambda(\alpha, \beta) - \widetilde \Lambda(\alpha', \beta') \leq \begin{pmatrix} \alpha -\alpha' \\ \beta-\beta' \end{pmatrix}^T \begin{pmatrix} \frac{\partial \widetilde \Lambda}{\partial \alpha}(\alpha', \beta') \vspace{2mm} \\  \frac{\partial \widetilde \Lambda}{\partial \beta}(\alpha', \beta') \end{pmatrix}\;. \end{equation}
 
Then, using the notation $(\alpha^\star, \beta_\star)=(\alpha_{\widetilde F_n}^\star, \beta{\widetilde F_n}^\star)$ (to save some space) and the dependencies introduced between the parameters $(\lambda_i)_{i\in [4]}, \eta_1, \eta_2$ we use that both $p_1$ and $p_2$ can both be upper bounded by studying

\begin{align*} &\widetilde \Lambda(\alpha, \beta) -\min \left\{\widetilde \Lambda\left(\frac{\alpha-\lambda_2 h'(X_{n+1}-\mu)}{1+\lambda_2 \eta_2},\frac{\beta}{1+\lambda_2 \eta_2}\right),\widetilde \Lambda\left(\frac{\alpha}{1+\lambda_2 \eta_2},\frac{\beta-\lambda_2}{1+\lambda_2 \eta_2}\right) \right\} \\ 
 &\leq  \widetilde \Lambda(\alpha^\star, \beta^\star) - \widetilde \Lambda\left(\frac{\alpha^\star-(\lambda_4 + \lambda_2)h'(X_{n+1}-\mu)}{1+\lambda_2\eta_2}, \frac{\beta^\star-(\lambda_4 + \lambda_2)}{1+\lambda_2\eta_2}\right) \;.
\end{align*}

We now choose $\lambda_2 = \lambda_4 = \lambda/2$, and use the notation $\alpha(\lambda)= \frac{\alpha^\star-\lambda h'(X_{n+1}-\mu)}{1+\lambda\eta_2/2}$ and $\beta(\lambda) = \frac{\beta^\star-\lambda}{1+\lambda\eta_2/2}$. We then use Equation~\eqref{eq::concavity} to further upper bound this term by \[\left(|\alpha^\star - \alpha(\lambda)|+|\beta^\star - \beta(\lambda)|\right) \left( \left|\frac{\partial \widetilde \Lambda}{\partial \alpha}(\alpha(\lambda), \beta(\lambda))\right| + \left|\frac{\partial \widetilde \Lambda}{\partial \beta}(\alpha(\lambda), \beta(\lambda))\right|\right) \;.\] 

Finally, we simply use the compactness of the set $\cF$ (thanks to the enforcement of the condition $F_n \in \cF$), so that all $(\alpha^\star, \beta^\star, h'(X_{n+1}-\mu))$ admit universal bounds: there exists $k_\cF\geq 0$ such that $|\alpha^\star - \alpha(\lambda)| \leq k_\cF \lambda$. Then, we choose $\lambda$ as follows: 

\[\lambda = \max \left\{\lambda >0: \quad \left|\frac{\partial \widetilde \Lambda}{\partial \alpha}(\alpha(\lambda), \beta(\lambda))\right| + \left|\frac{\partial \widetilde \Lambda}{\partial \beta}(\alpha(\lambda), \beta(\lambda))\right| \leq \max\left\{\frac{\eta_1}{4 k_\cF h'(X_{n+1}-\mu)}, \frac{\eta_2}{4 k_\cF} \right\}  \right\} \;, \]

that is strictly positive since for $\lambda=0$ the gradients is $0$. For this choice of $\lambda$ we obtain that 

\[\left\{\begin{array}{llll}
p_1 \leq e^{-(n+1)\lambda \frac{\eta_1}{4}} \\
p_2 \leq e^{- (n+1)\lambda \frac{\eta_2}{4}} \\
p_3 \leq e^{-(n+1) \lambda \frac{\delta}{4\alpha_M}} \\
p_4 \leq e^{-(n+1) \lambda \frac{\delta}{4\beta_M}} \;,\\	
\end{array} \right. \]

so all these quantities are exponentially decreasing with $n$. Hence, there exists some rank $n_{F_n}\geq 0$ such that for all $n\geq n_{F_n}$,

\[p_1+p_2+p_3+p_4 \leq 1/2 \;. \]

For the final step of this part of the proof, we would like this equation to be valid for a universal rank. To prove that, we use that the mapping $F \in \cF \mapsto n_{F}$ is continuous, so using again the compactness of $\cF$ we can deduce the existence of an upper bound \[n_\cF^{\eta_1, \eta_2} = \max_{F\in \cF} n_F\;,\] 
such that the above inequality is valid for $n\geq n_\cF^{\eta_1, \eta_2}$ for all instances of $F \in \cF$, where $n_\cF^{\eta_1, \eta_2}$ decreases with $\eta_1, \eta_2$, and is infinite when one of them is equal to $0$. We hence obtain that for $n\geq n_\cF^{\eta_1, \eta_2}$, the BCP satisfies 

\[	\text{[BCP]} \geq  \frac{1}{2} e^{-n \left(\Lambda_{\alpha, \beta}(F_n, \mu+\eta_1, B-\eta_2)+\frac{\delta}{2}\right)}\;,
\]
  
for the choice of $(\alpha, \beta)$ explained above. We now consider the tuning of $\eta_1, \eta_2$, and recall that we choose $\eta_1 h'(X_{n+1}-\mu)=\eta_2$ (and $h'(X_{n+1}-\mu) \in [h'(\eta_1), H^+]$ for some value $H^+$ depending on the maximum value taken by $X_{n+1}$ on $\cF$). Hence, we simply consider them as being the largest parameters such that 

\[\forall F\in \cF: \quad \Lambda_{\alpha, \beta}(F, \mu+\eta_1, B-\eta_2) \leq \Lambda_{\alpha_{F_n}^\star, \beta_{F_n}^\star}(F, \mu, B) + \frac{\delta}{2} \;,\]

that provides again strictly positive values due to the compactness of $\cF$. This is sufficient to conclude our proof, using the notation $n_\cF$ for the value $n_{\cF}^{\eta_1,\eta_2}$ corresponding to this specific choice:
\[\forall n\geq n_\cF\;,\quad  \text{[BCP]} \geq \frac{1}{2} e^{-n \left(\Lambda_{\alpha_{F_n}^\star, \beta_{F_n}^\star}(F, \mu, B) + \delta \right)} \;.\]

==> proof_duel_algo.tex <==
\section{Regret decomposition (following Theorem~3.1 of \cite{baudry21DS})}\label{app::general_proof}

In this section we study the regret of our proposed modification of the DS algorithm to tackle a given family on distributions $\cF$. 

Before starting the analysis we introduce some notations and assumptions.

\subsection{Notations and Assumptions}

\begin{itemize}
	\item We denote by $T$ the total number of rounds played by the bandit algorithm. 
	\item $\cA_r \subset \{1,\dots, K\}$: Set of arms to pull at the end of round $r$.
	\item $N_k(r)=1 + \sum_{s=1}^{r-1} \ind(k \in \cA_s)$: Number of pulls of arm $k$ up to round $r$.
	\item $\ell^r \in \{1,\dots, K\}$: Leader at round $r$, we recall that 
	\[\ell^r \in \aargmax_{k \in \{1, \dots, K\}} N_k(r)\;. \]
	\item For an arm $k$, we assume that an infinite stream of data $X_1^k, \dots, X_T^k, \dots$ is available, and for any $n \in \N$ $X_n^k$ is the $n$-th observation collected by the algorithm for arm $k$.
	\item $\mu_k(r) = \frac{1}{N_k(r)} \sum_{i=1}^{N_k(r)} X_i^k$ denotes the empirical average of arm $k$ at round $r$.
	\item $\mu_{k, n} = \frac{1}{n} \sum_{i=1}^{n} X_i^k$ denotes the empirical average of arm $k$ after collecting exactly $n$ observations.
	\item $\widetilde \mu_k(r) = \sum_{i=1}^n w_i X_i^k + w_{n+1} Y_k(r)$ denotes the re-weighted mean potentially used for arm $k$ at round $r$ if it is challenger. $w \sim \cD_{n+1}$ are weights drawn from the Dirichlet distribution $\cD_{n+1}$ with parameter $1_{n+1} = (1, \dots, 1)$ and $1_{n+1}^T 1_n = n+1$. $Y(r)$ denotes the bonus added to the observations of arm $k$ at round $r$ and depend on the current leader. When considering this function for a fixed arm $k$ with with sample size $n$ and bonus that depends only on $X_1, \dots, X_n,y$ for some $y \in \R$ we also write $\widetilde \mu_k(n, y)$.
\end{itemize}


The first condition that we assume on the arms distributions ensures the concentration of the means.

\paragraph{Condition 1 (C1): concentration of the means} For all $k$, there exists a good rate function $I_k$ satisfying for all $x \geq \mu_k$, $y \leq \mu_k$, and any i.i.d sequence $X_1, \dots, X_n$ drawn from $\nu_k$ 
\begin{equation*}\bP\left( \frac{1}{n} \sum_{i=1}^n X_i \geq x \right) \leq e^{-n I_k(x)} \;, \; \text{and } \bP\left(\frac{1}{n} \sum_{i=1}^n X_i \leq y\right) \leq e^{-n I_k(y)} \;.\end{equation*}


\textcolor{red}{Maybe we can be more general and replace the exponentials by something like $\frac{C_x}{n^\alpha}$, where $\alpha > 3$ is needed for the sums to converge in the following proof. Decide later if we want to cover this or not.}

\paragraph{Condition 1b (C1b): concentration of the means} For all $k$, there exists a function $C_k$ satisfying for all $x \geq \mu_k$, $y \leq \mu_k$, and any i.i.d sequence $X_1, \dots, X_n$ drawn from $\nu_k$ 
\begin{equation*}\bP\left( \frac{1}{n} \sum_{i=1}^n X_i \geq x \right) \leq \frac{C_k(x)}{n^3} \;, \; \text{and } \bP\left(\frac{1}{n} \sum_{i=1}^n X_i \leq y\right) \leq \frac{C_k(y)}{n^3} \;.\end{equation*}

\subsection{Regret decomposition}

Classically with the round-based algorithms, we start by decomposing the regret depending on whether the optimal arm is the leader or not. Without loss of generality, we assume arm $1$ to be the leader and we assume that all other arms are sub-optimal (see \cite{chan2020multi} for a similar proof handling the case of several optimal arm).

\begin{align*}
	\bE[N_k(T)] &= 1 + \bE\left[\sum_{r=1}^{T-1} \ind(k \in \cA_{r+1})\right] \\
	&= 1 + \sum_{r=1}^{T-1} \bE\left[\ind(k \in \cA_{r+1}, \ell^r=1) + \ind(k \in \cA_{r+1}, \ell^r \neq 1) \right] \\
	&\leq 1 + \underbrace{\bE\left[\sum_{r=1}^{T-1}\ind( k \in \cA_{r+1}, \ell^r=1)\right]}_{n_k(T)} + \underbrace{\bE\left[\sum_{r=1}^{T-1}\ind(\ell^r\neq 1) \right]}_{A_T} \;. 
\end{align*}

We can now upper bound separately the terms $n_k(T)$, corresponding to the post-convergence term in \cite{RiouHonda20}, and the term $A_T$ that corresponds to their pre-convergence term. We start by providing the generic proof scheme to upper bound $A_T$ inspired by the proof of \cite{baudry21DS} before introducing novel elements.

\subsection{Upper bound on $A_T$}

We simply decompose $\ind(\ell^r \neq 1)$ into two alternatives, namely 1) arm $1$ has already been leader and has lost the leadership at some point (leadership takeover), or 2) arm $1$ has never been leader. We define the sequence $a_r = \lceil r/4 \rceil$ and the event
\[\cD_r = \{\exists u \in [a_r, r]: \ell^u=1\} \;.\]

\subsubsection{$\cD_r$ is true: arm $1$ has already been leader after round $a_r$}

We propose an adaptation of the proof of \cite{baudry21DS}, leading to a smaller upper bound for the terms we consider in this section. The idea is to analyze the event $\cup_{r=1}^{T-1}\{\ell^r=1 \cap \cD^r \}$ by noticing that (1) an arm can take the leadership only if its sample size is equal to the one of the leader and its empirical mean is larger and (2) a single sample can only lead to \textbf{one} leadership takeover. Hence, we can directly write that 
\[\{\{\ell^r \neq 1\} \cap \cD^r \} \subset \left\{\cup_{n=b_r}^r \left\{\mu_{1,n} \leq \max_{k=2,\dots, K} \mu_{k, n}\right\}\right\} \;, \]

where $b_r=\lceil a_r/K \rceil$ grows linearly in $r$ thanks to the choice of $a_r$. 
Using that simple result, for any $r_0\geq 8K$ and for any $x \in \left(\max_{k=2, \dots, K} \mu_k, \mu_1 \right)$ we can directly obtain that

\begin{align*}
\bE\left[\sum_{r=r_0}^{T-1}\ind(\ell^r\neq 1, \cD^r)\right] 
& \leq  \sum_{r=r_0}^{T-1}\sum_{n=b_r}^{r} \bP\left(\mu_{1,n} \leq \max_{k=2, \dots, K} \mu_{k, n}\right) \\
& \leq  \sum_{r=r_0}^{T-1}\sum_{n=b_r}^{r} \bP\left(\mu_{1,n} \leq x\right) + \sum_{k=2}^K \sum_{r=r_0}^{T-1}\sum_{n=b_r}^{r}\bP\left(\mu_{k, n} \geq x\right)\\
& \leq  \sum_{r=r_0}^{T-1}r \bP\left(\mu_{1,b_r} \leq x\right) + \sum_{k=2}^K \sum_{r=r_0}^{T-1}r\bP\left(\mu_{k, b_r} \geq x\right) \;.
\end{align*}

We can conclude that if both $\bP(\mu_{1,n} \leq x) = o(n^{-2})$ and for all $k\geq 2$ $\bP(\mu_{k,n} \geq x) = o(n^{-2})$ then \[\bE\left[\sum_{r=1}^{T-1}\ind(\ell^r\neq 1, \cD^r)\right] = \cO(1) \;.\]

In this case, leadership takeovers from sub-optimal arms are too unlikely to cause a large regret. 
%Under $\cD_r$ we study the probability of a leadership takeover by a sub-optimal arm between $a_r$ and $r$. Such takeover can happen only if 1) a sub-optimal arm obtain the same number of samples as arm $1$, and 2) its sample average is larger than the one of arm $1$ at the round when it happens. We denote $\cX_n^k$ the history available for arm $k$ after it has been sampled $n$ times, and drop the exponent for arm $1$. We formalize the leadership takeover with the following events, 
%
%\begin{align*}
%	\{\ell^r&\neq 1\} \cap \cD^r \subset \cup_{u=a_r}^{r-1}\{\ell^u=1, \ell^{u+1}\neq 1 \} \\ 
%	& \subset \cup_{u=a_r}^{r-1} \cup_{k=2}^K \{\ell^u=1, k \in \mathcal{A}_{u+1}, N_k(u+1)=N_1(u+1),\mu_{k, N_k(u+1)} \geq  \mu_{1, N_1(u+1)}\} \\
%	& \subset \cup_{u=a_r}^{r-1} \cup_{k=2}^K \{N_k(u+1)=N_1(u+1),\mu_{k, N_k(u+1)} \geq  \mu_{1, N_1(u+1)}\} \\
%	& = \subset \cup_{u=a_r+1}^{r} \cup_{k=2}^K \{N_k(u)=N_1(u),\mu_{k, N_k(u)} \geq  \mu_{1, N_1(u)}\} \\
%	& \coloneqq \cup_{u=a_r+1}^{r} \cup_{k=2}^K \cB_k^u \;.
%\end{align*}
%
%Starting the sum on the rounds at some round $r_0$, we first develop and express the sum of these terms as
%
%\begin{align*}
%	\bE\left[\sum_{r=r_0}^{T-1} \sum_{u=a_r+1}^r \ind(\cB_{k}^u) \right]  &=
%	\bE\left[\sum_{r=r_0}^{T-1} \sum_{u=a_r+1}^r \ind(N_k(u)=N_1(u),\mu_{k, N_k(u)} \geq  \mu_{1, N_1(u)}) \right] \\
%	&\leq \bE\left[\sum_{r=r_0}^{T-1} \sum_{u=a_r+1}^{r} \sum_{n=\lceil u/K \rceil}^u \ind(N_k(u)=N_1(u)=n, \mu_{k, n} \geq  \mu_{1, n})\right] \\
%	&\leq  \bE\left[\sum_{r=r_0}^{T-1} \sum_{u=a_r+1}^{r} \sum_{n=\lceil u/K \rceil}^u \ind(\mu_{k, n} \geq  \mu_{1, n})\right]\,.
%\end{align*}
%
%We now define $x_k= \frac{\mu_1+\mu_k}{2}$. If $\mu_{k, n} \geq  \mu_{1, n}$, then either the arm $1$ had "under-performed" or arm $k$ has "over-performed", which means that $\mu_{k, n} \geq  x_k $ or $\mu_{1, n} \leq x_k$, which gives 
%
%\begin{align*}
%\bE\left[\sum_{r=r_0}^{T-1} \sum_{u=a_r+1}^t \ind(\cB_{k}^u) \right]	&\leq  \bE\left[\sum_{r=r_0}^{T-1} \sum_{u=a_r+1}^{r} \sum_{n=\lceil u/K \rceil}^u \ind(\mu_{k, n} \geq x_k \cup \mu_{1, n} \leq x_k)\right] \\
%	&\leq \sum_{r=r_0}^{T-1} \sum_{u=a_r+1}^{r} \sum_{n=\lceil u/K \rceil}^u \left[ \bP(\mu_{k, n} \geq x_k) + \bP(\mu_{1, n} \leq x_k) \right] \\
%	& \leq \sum_{r=r_0}^{T-1} r^2 \left[ \bP(\mu_{k, b_r}\geq x_k) + \bP(\mu_{1, b_r} \leq x_k) \right] \\
%	& \leq \sum_{r=r_0}^{T-1} r^2 \left(e^{-b_r I_1(x_k)} + e^{-b_r I_k(x_k)}\right)\\
%	& = O(1) \;,
%\end{align*}
%
%
%\textcolor{red}{Remove the exponential by the appropriate concentration we choose to consider, or remove the last line to be general. \\
%It seems that if we change the empirical means by Median-of-Means or something else we do not have to change anything. Again, adapt notations later depending on the level of generality we seek.}
%
%Thanks to the structure of the algorithm this condition is enough to upper bound the cost of leadership takeover by sub-optimal arms by a constant term in the regret. We now consider the case when arm $1$ has never been leader.

\subsubsection{$\cD_r$ is not true: arm $1$ has never been leader after round $a_r$}

Using the proof in \cite{baudry21DS}, we can directly write that
\[\sum_{r=r_0}^{T-1} \ind(\ell^r \neq 1, \bar \cD^r) \leq \sum_{r=r_0}^{T-1}\ind(\bar\cD^r) \leq 32 \sum_{r=\lceil r_0/4 \rceil}^{T-1} \ind(\cC^r) \;, \]

where $\cC^r=\left\{\exists k \neq 1,\ell^r=k, 1 \notin \cA_{r+1}\right\}$ denotes the simple fact that arm $1$ lost its duel at round $r$ against a sub-optimal leader. We can consider all possible sub-optimal leader, 

\[ \cC^r = \cup_{k=2}^K \{\ell^r =k, 1 \notin \cA_{r+1} \}\coloneqq \cup_{k=2}^K \widetilde \cC_{k}^r \;.\]

We now fix a sub-optimal leader $k \in \{2, \dots, K \}$. Again, two cases are possible: (1) the leader could be "over-performing", or (2) arm $1$ could be under-performing. The first case is easy to handle thanks again to the linear number of observations from the leader. For any $\eta>0$ we write \[\widetilde \cC_{k}^r = \underbrace{\{\widetilde \cC_{k}^r \cap |\mu_k(r)-\mu_k|\leq \eta\}}_{\cC_{k, 0}^r} \cup\underbrace{\{\widetilde \cC_{k}^r \cap |\mu_k(r)-\mu_k|\geq \eta\}}_{\cC_{k}^r} \;. \]

The first term can then by upper bounded by 
\begin{align*}
	\cC_{k, 0}^r &\leq \sum_{r=r_0}^{T-1} \sum_{n=\lceil r/K \rceil}^r \bP\left(\left|\mu_{k, n}-\mu_k\right|\geq \eta, N_k(r)=n\right)\\
	&\leq \sum_{r=r_0}^{T-1} r \bP\left(\left|\mu_{k, \lceil r/K\rceil}-\mu_j\right|\geq \eta\right)\\
	&= \cO(1), \\
\end{align*} 

under the same assumptions that ensured the convergence in the previous section. We now obtain the intermediate result 

\[\bE\left[\sum_{r=r_0}^{T-1} \ind(\ell^r \neq 1, \bar \cD^r)\right] \leq 32 \sum_{k=2}^K \bP(\cC_k^r) + \cO(1) \;. \]

Reformulating $\cC_k^r$ provides 
\begin{align*}\cC_k^r \subset & \{|\mu_k(r) - \mu_k| \leq \eta, \widetilde \mu_k(r) \leq \mu_k(r)\} \\ 
&  \subset \{|\mu_k(r) - \mu_k| \leq \eta, \widetilde \mu_k(r) \leq \mu_k+\eta \} \\
& \subset \{\widetilde \mu_k(N_k(r), \mu_k-\eta) \leq \mu_k+\eta \}
\end{align*}

\textcolor{red}{Maybe stop here for a general result: \[\sum_{r=1}^{T-1} \bP(\ell^r=1) \leq \bE\left[\sum_{r=1}^{T-1} \ind(1 \notin \cA_{r+1}, \ell^r=k, |\mu_k(r)-\mu(k)|\leq \eta)\right] + \cO(1)\] This is very general and true for any sampling distribution.}

Then, by carefully following the steps of the analysis of \cite{RiouHonda20} for the pre-convergence term we obtain that for any $k \in \{2, \dots, K\}$, 

\[\sum_{r=1}^{T-1} \bP(\cC_k^r) \leq \sum_{n=1}^{T-1} \bE\left[\frac{1}{\bP_w\left(\sum_{i=1}^n w_i X_i + w_{n+1} \cB_{\cX_n}(\mu_k-\epsilon) \geq \mu_j+\epsilon, w \in \cS_{\widetilde \cX_n}^{-1}(\cF)\right)}-1\right]\;, \] 

where $\cB_{\cX}(y)$ is the function that returns a solution of Equation~\ref{eq::x_to_add} provided a history $\cX$ and a mean $\mu$, and $\widetilde \cX_n = \cX_n \cup \cB_{\cX_n}(\mu_j-\epsilon)$. The work is then to lower bound the probability inside this expectation.

\subsection{Some work on $\bE\left[\frac{1}{\bP_w(w^T X \geq \mu, w \in \cS_\cX^{-1}(\cF))}-1\right]$}

Our idea is to simply remark that the quantity inside the expectation is a positive random variable. Using a known result, we can write that 

\[\bE\left[\frac{1}{\bP_w(w^T X \geq \mu, w \in \cS_\cX^{-1}(\cF))}-1\right] = \int_0^{+\infty} \bP\left(\frac{1}{\bP_w(w^T X \geq \mu, w \in \cS_\cX^{-1}(\cF))}-1 > x\right) dx \;.\]

I our precise case we do not have precise lower bounds on this probability yet, but I think this simple result may simplify the proof in \cite{RiouHonda20}. Assume that we can prove a lower bound of the form \[\bP_w(w^T X \geq \mu, w \in \cS_\cX^{-1}(\cF)) \geq  \frac{C}{n^\alpha}\exp(-n \kinf^\cF(\widehat F_n, \mu)) \;.\] 

Then, we can upper bound the expectation as

\begin{align*}
\bE\left[\frac{1}{\bP_w(w^T X \geq \mu, w \in \cS_\cX^{-1}(\cF))}-1\right] &= \int_0^{+\infty} \bP\left(\frac{1}{\bP_w(w^T X \geq \mu, w \in \cS_\cX^{-1}(\cF))}-1 > x\right) dx \\
& \leq \int_0^{+\infty} \bP\left(\frac{n_\alpha}{C} e^{n \kinf^\cF(\widehat F_n, \mu)} > 1 + x\right) dx \\
& = \int_0^{+\infty} \bP\left(\kinf^\cF(\widehat F_n, \mu) > \frac{1}{n}\log\left(\frac{C}{n^\alpha}(1 + x)\right)\right) dx \\
\end{align*}

\textcolor{red}{PROBLEM: for $x$ close to $0$ the probability is equal to $1$ if $C/n^\alpha >1$, leading to linear regret (alternatively, the lof term in above result is negative). }

\textcolor{red}{Potential Fix, re-write later}
I omitted in the proof the "side event" $\ind(\mu_{1,n}<\mu_1-\epsilon)$. Actually, this event can save us when $n^\alpha/C \neq 1$. Let simply consider that 

\begin{align*}
&\bE\left[\ind(\mu_{1,n}< \mu) \left(\frac{n^\alpha}{C} e^{n \kinf(F_n, \mu)}-1\right)\right]  \\
\leq & bE\left[\ind(\mu_{1,n}< \mu) \left(\frac{n^\alpha}{C} (e^{n \kinf(F_n, \mu)}-1) + \frac{n^\alpha}{C}-1\right)\right] \\
\leq & \left(\frac{n^\alpha}{C}-1\right)\bP(\mu_{1, n} < \mu) + \frac{n^\alpha}{C}\bE\left[e^{n \kinf(F_n, \mu)}-1\right]\;, \\
\end{align*}

and now we're back at considering $\bE\left[e^{n \kinf(F_n, \mu)}-1\right]$, which is nice. We require that $\sum_n \bP(\mu_{1, n} < \mu)= \cO(1)$.

\textcolor{red}{End of potential fix}

We recall that $\mu \approx \mu_k$ for a sub-optimal arm $k$. In \cite{agrawal2020optimal} Lemma 11 proposes a concentration inequality for $\kinf^\cF(\widehat F_n, \mu_1)$. We now simply transform our expression to use this inequality. 
\textcolor{red}{Assumption: We assume that $\inf_{\widehat F_n} \left\{\kinf^\cF(\widehat F_n, \mu_1) - \kinf^\cF(\widehat F_n, \mu_k) = \delta > 0\right\}$.}

In the case of def~\ref{def::uncentered_constraint} we can use a result from \cite{agrawal2020optimal}: using the convexity of $\kinf^\cF$, that
	\begin{align*}
	\inf_{\widehat F_n} \left\{\kinf^\cF(\widehat F_n, \mu_1) - \kinf^\cF(\widehat F_n, \mu_k)\right\} & \geq (\mu_1-\mu_k) \times \frac{\partial \kinf^\cF}{\partial \mu}(F_n, \mu_k) \\
	& =  (\mu_1-\mu_k) \alpha^\star(F_n, \mu_k) \\
	& \geq \frac{\mu_1-\mu_k}{f^{-1}(B)-\mu_k}
	\end{align*}

\textcolor{red}{Wrong, wrong side of the inequality... Or maybe yes at it corresponds to the derivative in the dirac in $-h^{-1}(B)$.}
\textcolor{red}{Note that at least $\delta$ exists if $\kinf^\cF$ is strongly convex in the second argument.}

We then have 

\begin{align*}
&\bE\left[\frac{1}{\bP_w(w^T X \geq \mu, w \in \cS_\cX^{-1}(\cF))}-1\right] \\
& \leq \int_0^{+\infty} \bP\left(\kinf^\cF(\widehat F_n, \mu_1) - (\kinf^\cF(\widehat F_n, \mu_1)-\kinf^\cF(\widehat F_n, \mu)) > \frac{1}{n}\log\left(\frac{C}{n^\alpha}(1 + x)\right)\right) dx \\
& \leq \int_0^{+\infty} \bP\left(\kinf^\cF(\widehat F_n, \mu_1) > \delta + \frac{1}{n}\log\left(\frac{C}{n^\alpha}(1 + x)\right)\right) dx \;.\\
\end{align*}

\textcolor{red}{2nd assumption: the kinf cannot be arbitrarily large (our bound can be integrated): typically true for bounded distributions as $\kinf^\cF(\widehat F_n, \mu_1)< \kinf^\cF(0, \mu_1)= -\log(\mu)$. Hence, the integral can be computed up to some constant $U_{\mu, \cF, n}$. For bounded, it would be $\exp\left(n(-\log(\mu)-\delta)\right)\times \frac{n^\alpha}{C}$.}

We now obtain using Lemma 11 of \cite{agrawal2020optimal}

\begin{align*}
\bE\left[\frac{1}{\bP_w(w^T X \geq \mu, w \in \cS_\cX^{-1}(\cF))}-1\right] 
& \leq (n+1)^2 e^{\bar B} e^{-n \delta} \times \frac{n^\alpha}{C} \int_0^{U_{\mu, \cF, n}} \frac{1}{1+x} dx \\
& = (n+1)^2 e^{\bar B} e^{-n \delta} \times \frac{n^\alpha}{C} \log(1+U_{\mu, \cF, n}) \\
\end{align*}

For bounded distributions the bound is $\approx (n+1)^{\alpha+3} e^{-n\delta}$, so the sum converges. This result is actually similar to what we need in the proof of \cite{RiouHonda20}, that also involves this $\delta$.

\textcolor{red}{It seems to me that everthing holds for bounded distributions. Hence, for convenience of the proof we may show everything by assuming that the distributions actually have a discrete support, letting it be potentially very large and completely unknown. But of course the main difficulty remains to find a lower bound.}

\subsection{Upper bound on $n_k(T)$}

\textcolor{red}{I let this part like that for the moment but we may remove $F_{k, r} \in \cF$, and maybe $W$ by another distance if it can be more suitable.}


We recall that for any $k \in \{2, \dots, K\}$, 
\[n_k(T) = \bE\left[\sum_{r=1}^{T-1} \ind(k \in \cA_{r+1}, \ell^r=1) \right] \]

We define a good event, that is \[\cG_k^r = \{\mu_1(r) \in [\mu_1-\epsilon_1, \mu_1+\epsilon_1], W(F_{k, r}, F_k) \leq \epsilon_2, F_{k, r}\in \cF \} \;.\] 

For any $y \in (\mu_k, \mu_1)$ we write that

\begin{align*}
n_k(T) & \leq \underbrace{\bE\left[\sum_{r=1}^{T-1} \ind(k \in \cA_{r+1}, \ell^r=1, \cG_k^r)\right]}_{B_1}+ \underbrace{\bE\left[\sum_{r=1}^{T-1}\ind(k \in \cA_{r+1},\ell^r =1,  \bar \cG_k^r) \right]}_{B2}\;.\\
\end{align*}

We now consider the first term,

\begin{align*}
B_1 & \leq \bE\left[\sum_{r=1}^{T-1} \ind(k \in \cA_{r+1}, \mu_{N_1(r)} \leq \widetilde \mu_{k, N_k(r)}(\mu_{N_1(r)}), \ell^r=1, \cG_k^r) \right] \\
& \leq \bE\left[\sum_{r=1}^{T-1} \ind(k \in \cA_{r+1}, \widetilde  \mu_{k, N_k(r)}(\mu_{N_1(r)}) \geq \mu_1 - \epsilon_1 , \cG_k^r) \right] \\
& \leq \bE\left[\sum_{r=1}^{T-1}\sum_{n=1}^T \ind(k \in \cA_{r+1}, N_k(r)=n, \widetilde \mu_{k, n}(\mu_1+\epsilon_1) \geq \mu_1 - \epsilon_1, W(F_{k,n}, F)\leq \epsilon_2, F_{k, n} \in \cF) \right] \\
& \leq \bE\left[\sum_{n=1}^T \ind(\widetilde \mu_{k, n}(\mu_1+\epsilon_1) \geq \mu_1 - \epsilon_1, W(F_{k,n}, F)\leq \epsilon_2, F_{k, n} \in \cF) \right] \\
& \leq m_k(T) + \bE\left[\sum_{n=m_k(T)}^{T-1} Cn e^{-n\kinf^\cF(F_{k, n}, \mu_1-\epsilon_1)} \ind(W(F_{k,n}, F)\leq \epsilon_2, F_{k, n} \in \cF)\right] \\
& \leq m_k(T) + T m_k(T) e^{-m_k(T) (\kinf^\cF(F_k, \mu_1)-\epsilon)} \;.
\end{align*}

\textcolor{red}{I assume we can prove the upper bound on the joint probability, and with a similar Chernoff argument when $F_{k, n} \in \cF$ we should be able to bound the denominator by a constant for $n$ large enough. I then use the continuity of $\kinf^\cF$ in both arguments.}

We then choose $m_k(T)= \frac{\log(T) + \log \left(\frac{\log(T)}{\kinf^\cF(F_k, \mu_1)-\epsilon}\right)}{\kinf^\cF(F_k, \mu_1)-\epsilon}$ to obtain that \[B_1 \leq \frac{\log(T)}{\kinf^\cF(F_k, \mu_1)-\epsilon} + o(\log(T)) \;. \]

Then we proceed with $B_2$, for which we will consider the three events that can make $\bar \cG_k^r$ hold.

\begin{align*}
B_{21} &\coloneqq \bE\left[\sum_{r=1}^{T-1}\ind(k \in \cA_{r+1},\ell^r =1,|\mu_1(r)-\mu_1| \geq \epsilon_1) \right] \\
& \leq \sum_{r=1}^{T-1} \sum_{n=\lceil r/K \rceil}^{r} \bP(|\mu_{1, n}-\mu_1| \geq \epsilon_1) \\
& \leq \sum_{r=1}^{T-1} r \times \bP(| \mu_{1, \lceil r/K\rceil}-\mu_1| \geq \epsilon_1) \\
& = \cO(1) \;,
\end{align*}

\textcolor{red}{under the right assumptions.}

Then we consider the events related to arm $k$, starting with
\begin{align*}
B_{22} & \coloneqq \bE\left[\sum_{r=1}^{T-1}\ind(k \in \cA_{r+1},\ell^r =1,W(F_k(r), F_k) \geq \epsilon_2) \right] \\
& \leq \sum_{n_k = 1}^{T-1} \bP(W(F_{k, n}, F_k)\geq \epsilon_2) \\
& = \cO(1) \;,
\end{align*}

\textcolor{red}{also under the right assumptions}

Finally, we obtain similarly 

\begin{align*}
B_{23} & \coloneqq \bE\left[\sum_{r=1}^{T-1}\ind(k \in \cA_{r+1},\ell^r =1, F_k(r) \notin \cF) \right] \\
& \leq \sum_{n_k = 1}^{T-1} \bP(F_{k, n} \notin \cF) \\
& = \cO(1) \;, 
\end{align*}
\textcolor{red}{under the right assumptions.}

Finally, we obtain that \[B_2 \leq B_{21} + B_{22} + B_{23} = \cO(1) \;. \]

\paragraph{What are these right assumptions?} For the Wasserstein distance finite exponential moment or simply finite moment $2+\eta$ for $\eta>0$ is fine \citep{fournier_wasserstein}. For the average of arm $1$ it is the same as in previous section. For the last one it is more mysterious. Obviously, $(h(X_i))$ is a collection of random variables and having $\bE[h(X)^{2+\eta}]< +\infty$ for some $\eta>0$ is enough to have a weak concentration inequality. However, for instance with sub-gaussian distributions it is clear that $\bE\left[e^{CX^4}\right]$ may not exist (e.g Gaussian), so finding a concentration inequality in that case may not be easy (not possible?). The trivial case where everything work is the case where distributions in $\cF$ are bounded (possibly by arbitrary large and unknown bounds, but still). 


\paragraph{Maybe simpler alternative proof}

\begin{align*}
B_1 & \leq \bE\left[\sum_{r=1}^{T-1} \ind(k \in \cA_{r+1}, \ell^r=1, \cG_k^r) \right] \\
& \leq m_T + \bE\left[\sum_{r=1}^{T-1} \ind(k \in \cA_{r+1}, \ell^r=1, \cG_k^r, N_k(r) \geq m_T) \right] \;.\\
\end{align*}

We recall that the probability to sample arm $k$ when arm $1$ is leader is upper bounded by $p_n(r) = e^{-N_k(r) \kinf^\cF(F_k(r), \mu_1(r))}$. Under the events provided in the expectation and using the continuity of $\kinf$ in both arguments it holds that \[e^{-N_k(r) \kinf^\cF(F_k(r), \mu_1(r))} \leq e^{-N_k(r) (\kinf^\cF(F_k, \mu_1)-\epsilon)} \leq e^{-m_T (\kinf^\cF(F_k, \mu_1)-\epsilon)}\;, \]

for some $\epsilon>0$ that depends on $\epsilon_1$ and $\epsilon_2$. Hence, we obtain 

\begin{align*}
B_1 & \leq m_T + T e^{-m_T \left(\kinf^\cF(F_k, \mu_1)-\epsilon\right)}  \;.\\
\end{align*}

Then, choosing $m_T=\frac{\log(T)}{\kinf^\cF(F_k, \mu_1)-\epsilon}$ provides $B_1=m_T+1$. Then, we obtain $B_2=\cO(1)$ under good assumptions. 

\textcolor{blue}{
To obtain that we require:
\begin{enumerate}
	\item $\kinf^\cF$ is continuous with respect to its first and second argument according to some metric $d$ (e.g Levy, Wasserstein).
	\item The optimal arm must satisfy $\sum_{r=1}^{T-1}r \bP\left(\mu_{1, \lceil r/K \rceil - \mu_1} \geq \epsilon_1 \right) = \cO(1)$ for any $\epsilon_1>0$ small enough.
	\item $(\cF, d)$ must satisfty $\sum_{n=1}^{+\infty}\bP(d(F_{k, n}, F_k) \geq \epsilon_2) = \cO(1)$ for any $\epsilon_2>0$ small enough.
\end{enumerate}
So far, we have 
\begin{itemize}
	\item everything is $\cF$ is a single-parameter exponential family (SPEF), bounded distributions with a known upper bound $B$, or if $\cF$ is defined as in def~\ref{def::uncentered_constraint} (\cite{agrawal2020optimal} for continuity) and is either light-tailed or at least have a finite 3rd moment (moment $3+\epsilon$ for some $\epsilon$). 
\end{itemize}
}

==> results_v0.tex <==
\section{General recipe for the regret analysis of randomized algorithms}\label{sec::results}

In the previous section we introduced some examples of algorithms covered by the scope of our analysis, we now introduce our main theoretical results.

\subsection{Common properties of existing families of distributions}

We first answer the first question that we introduced at the beginning of the paper, by exhibiting the salient features shared by many usual families of distributions for which there are asymptotically optimal bandit algorithms. We group these features in the generic Assumption~\ref{ass::sufficient_prop}, and will prove in the next section that they are sufficient to design a bandit algorithm that achieves logarithmic regret for a given family of distributions.

\begin{assumption}[Sufficient properties on a family of distributions $\cF$]\label{ass::sufficient_prop}
Let $F$ be any distribution of mean $\mu_F$. Let us denote by $F_n$ the empirical distribution\footnote{If $\cF$ is parametric we take the distribution of $\cF$ corresponding to the MLE of the parameters.} of $n$ i.i.d. samples drawn from $F$, and by $\mu_n$ their expectation. 

We assume that there exists a function $D: \cP \times \R \mapsto \R^+$ satisfying the following properties:
\begin{itemize}
\item \textbf{Continuity and monotonicity of $D$ (A1):} $D$ is continuous in its second argument, the mapping $x \mapsto D(F, x)$ is non-decreasing, and $D(F, \mu)=0$ for any $\mu\leq \mu_F$.
\item \textbf{Concentration of $D$ (A2):} for any $\mu > \mu_F$, and $\delta>0$, % small enough, 
\[\sum_{n=1}^{+\infty} \bP\left(D(F_{n}, \mu) \leq D(F, \mu)-\delta\right) = \cO(1)\;.\]
\item \textbf{Identifiability (A3):} For any $\epsilon>0$, there exists $\delta_{\epsilon, \mu_F}>0$ such that if $F_n \in \cF$, and $\mu_n \leq \mu_F-\epsilon$ it holds that
		\[D(F_n, \mu_F)-D(F_n, \mu_F-\epsilon)\geq \delta_{\epsilon, \mu_F}\;.\] 
\item \textbf{Concentration of $D(F_n, \mu_F)$ (A4):} For any $x>0$ it holds that \[\bP(D(F_{n}, \mu_F)> x) \leq \alpha_{n, x}\times e^{-nx}, \] where $\alpha_{n, x}$ is decreasing in $x$ for a fixed $n$, and polynomial in $n$ for a fixed $x$.
\item \textbf{Concentration of the mean estimator (A5):} For $\epsilon>0$, $\bP(\mu_n\leq \mu_F-\epsilon)$ admits an exponentially of polynomially decreasing upper bound.
	\end{itemize}
\end{assumption}

While these assumptions might look a bit heavy, they are necessary to reach a sufficient level of generality to tackle all the settings covered in this paper and have simple interpretations. In some cases they are easy to verify: let us consider for instance the family of bounded distributions (with range $[0,1]$) and $D(F_n, \mu)=2(\mu-\mu_n)^2\ind(\mu\geq \mu_n)$. (A1) is direct, and (A3) follows from a simple computation ($\delta_{\epsilon, \mu_F}=2\epsilon^2$). Then, all the remaining properties can be obtained without effort by using Hoeffding's inequality. In some sense, the assumptions (A1)--(A5) generalize the properties that are usually derived from concentration inequalities (Hoeffding's in our example) on the empirical means for simple models/choices of $D$ (bounded, sub-gaussian, SPEF). We now provide further high-level insights on their interpretation.

Intuitively, the metrics $D$ of interest are those for which $D(F, \mu)$ measures how ``far'' a distribution $F$ is to the sub-space of distributions from $\cF$ with expectation larger than $\mu$. We will typically consider metrics $D$ close to $\kinf$ for the families considered, but other choices are possible (e.g. squared gap or Bernoulli KL divergence for bounded distributions). \textbf{(A2)} is slightly weaker than assuming that $D$ is continuous in the first argument w.r.t. some metric and that $F_{n}$ converges ``fast enough" to some neighborhood of $F_k$. It ensures that the expected number of sample sizes for which the empirical distribution is ``over-performing'' is finite. Then, \textbf{(A3)} ensures that the metric $D$ properly separates the different mean levels, so that it can be used to identify an arm of mean $\mu$ from an arm of mean $\mu-\epsilon$. Finally, \textbf{(A4)} is another concentration property for $D$. This time, it relates an empirical distribution to the mean of the true distribution of its observation, requiring an exponentially decreasing bound. It ensures that, even if an empirical distribution is performing poorly, it has a low probability of being very far from the true distribution.
% \paragraph{(A3)--(A4) } \hspace*{-\baselineskip}
% might be
% %are
% the trickiest assumptions to prove for a given family $\cF$, and allow to upper bound the second term of $B(T,c,\epsilon)$. Their combination ensures that arm $1$ is regularly sampled even if it is performing poorly, so that such scenario does not harm the regret.

We can finally comment on \textbf{(A5)}, that is more usual in bandit analysis. Again, the statement is made general to cover all of our settings. If the distributions are \emph{light-tailed}, that is $\bE_F[\exp(\lambda |X|)]<+\infty$ for some $\lambda>0$, then an exponentially decreasing upper bound can be achieved (e.g. with Chernoff method), and a polynomial bound can be obtained if the distributions are \emph{heavy-tailed} but admit a finite moment-generating function. We refer to Theorem 2 of \citet{fournier_wasserstein} for such bounds (covering the two cases). Furthermore, in Appendix~\ref{app::A5_heavy} we also discuss the possible replacement of the empirical mean by a robust estimator for heavy-tailed distributions, to obtain exponentially decreasing bounds in that case.

We now show the level of generality of these assumptions by providing various examples of families $\cF$ for which Assumption~\ref{ass::sufficient_prop} is satisfied. 
In each case, we choose a function $D$ as close as possible to the $\kinf$ function corresponding to the family of distribution $\cF$. Due to space limitation, we detail the computation of these functions in Appendix~\ref{app::notation}. % Furthermore, when $(a_n)_{n\in \N}$ is un-specified the guarantees hold by setting $a_n=0$.

\begin{lemma}[Some families of distributions satisfying Assumption~\ref{ass::sufficient_prop}]\label{lem::P15}
Let $F$ be a distribution of mean $\mu_F$ and standard deviation $\sigma_F$, and $\mu\in\R$ be a threshold. Then, Assumption~\ref{ass::sufficient_prop} is satisfied if $\cF$ is one of the following families:  
\begin{itemize}
	\item \textbf{Single Parameter Exponential Family} with $D(F, \mu) = \kinf^\cF(F, \mu)$.%, if $(a_n)_{n\in \N}$ satisfies $\forall n \in \N,\; a_n > 0$ and $1/a_n = \cO(n^\alpha)$ for some $\alpha>0$.
	\item \textbf{Bounded distributions} with a known upper bound $B$, with $D(F, \mu) = \kinf^\cF(F, \mu)$.
	\item \textbf{Gaussian distributions}\footnote{For the Gaussian case we prove slightly relaxed version of (A3) and (A4) that are sufficient to obtain the same results, and justify a tuning of $a_n >\frac{1}{n-1}$ in our following results, see Section~\ref{app::gauss_P15} for more details.} with unknown means and variances, if% if $a_n > \frac{2}{n-2}$ and 
 \[D(F, \mu) = \kinf^\cF(F, \mu)\times \ind( (\mu-\mu_F)^2\leq \sqrt{n_F}, \sigma_F^2 \leq \sqrt{n_F})\;,\] 
 where $n_F$ is the size of the support of $F$ ($+\infty$ if $F$ is continuous).
	\item \textbf{$h$-moment conditions:} Let $h$ be a known positive convex function satisfying $\frac{h(|x|)}{|x|^{1+\eta}} \to + \infty$ for some $\eta>0$, and $\cF$ be defined as \begin{equation}\label{eq::uncentered_main}\cF = \left\{F \in \cP:\; \bE\left[h(|X|)\right] \leq B \;, \; \bE[h(|X|)^{2+\epsilon_F}]<+\infty \text{ for some } \epsilon_F>0 \right\} \;,\end{equation} 
 then (A1)--(A5) hold with $D(F, \mu) = \kinf^\cF(F, \mu) \ind(F \in \cF)$. This is also the case if the condition is \textbf{centered}, i.e. $h(|X|)$ is replaced by $h(|X-\mu_F|)$ in \eqref{eq::uncentered_main}, under the additional assumption that the means are lower bounded by a known constant $\mu^-$.
\end{itemize}
\end{lemma}

Lemma~\ref{lem::P15} answers the first question raised in Section~\ref{sec::introduction}: there is indeed a set of fundamental properties shared by all the main families of distributions that have been studied in the bandit literature, that may explain why the same algorithm principles work for all of them. Furthermore, we proved that these assumptions are valid for $\kinf^\cF$ or a function that matches $\kinf^\cF$ once the empirical distribution of an arm is ``close" to its true distribution. %As far as we know, this paper is the first to provide theoretical guarantees for settings with centered $h$-moment condition, that we believe to be an interesting result.

We postpone the proof in Appendix~\ref{app::proofs_A1_A5}, where we provide all the technical details and motivate the modifications made to $\kinf^\cF$ in some cases. We use several results from the literature, but also prove novel results of independent interest. For instance, Lemma~\ref{lem::conc_gaussian} is (as far as we know) a novel concentration inequality for the $\kinf$ of gaussian distributions with unknown variances. We now show the application of these results for the MED and TS algorithms introduced in Section~\ref{sec::prelim}.


\subsection{Regret bounds for MED and TS}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newpage
\section{\textcolor{blue}{Previous version of the section}}

We now present our first result, which is a generic upper bound of the expected number of pulls of each sub-optimal arm $k$ for any randomized policy satisfying Assumptions~\ref{ass::sampling_prob} and \ref{ass::A1}.

\begin{theorem}\label{th::first_bound}
Let $\pi$ be a policy satisfying Assumption~\ref{ass::sampling_prob} for a function $D_\pi$ satisfying (A1), and with $\log(C_n)= o(n^\alpha)$ for some $\alpha<1$. We assume w.l.o.g. that $\mu^\star=\mu_1$. Then, for any $c>0$ satisfying $c > \displaystyle \lim_{n\to \infty} a_n$ and for any $\epsilon>0$, it holds for any sub-optimal arm $k$ that 
\begin{equation}\label{eq::th_2}\bE[N_k(T)] \leq  (1+c) \frac{\log(T)}{D_\pi(F_k, \mu_1)} + B(T,c, \epsilon) + o(\log(T))\;,\end{equation}
%with \begin{align*}
%B(T,c, \epsilon) = &\sum_{n=u}^{+\infty} \bP\left(D_\pi(F_{k,n}, \mu_1-\epsilon)\frac{1+c}{1+a_n} \leq D_\pi(F_k, \mu_1)\right) \\ 
%+ &\sum_{n=1}^T c_n \int_{0}^{+\infty} \bP\left(D_\pi(F_{1,n}, \mu_1-\epsilon)> \frac{1+a_n}{n}\log(1+x)\right) \mathrm{d}x \\
%+ &  \sum_{n=1}^{T} (c_n-1) \bP\left(\mu_{1,n} \leq \mu_1-\epsilon \right) \;. 
%\end{align*}
%\end{theorem}
with \begin{align*}
	B(c, \epsilon) = &\sum_{n=1}^{+\infty} \bP\left(D_\pi(F_{k,n}, \mu_1-\epsilon)\frac{1+c}{1+a_n} \leq D_\pi(F_k, \mu_1)\right) \\ 
	+ &\sum_{n=1}^{+\infty} c_n \bE\left[e^{n \frac{D_\pi(F_{1,n}, \mu_1-\epsilon)}{1+a_n}}-1\right] +   \sum_{n=1}^{+\infty} (c_n-1) \bP\left(\mu_{1,n} \leq \mu_1-\epsilon \right) \;. 
\end{align*}
\end{theorem}
We detail the proof, which is inspired by the analysis of Maillard Sampling \citep{jun2022}, in Appendix~\ref{app::proof_th1}. We prove the result under the more general Assumption~\ref{ass::relaxed_sp} (presented in the Appendix) on the sampling probabilities, but we chose to present Assumption~\ref{ass::sampling_prob} in the main paper for the clarity of the presentation. The quantity $B(T, c, \epsilon)$ encapsulates the terms in the upper bound that require to carefully analyze the properties of $D_\pi$ on the family of distributions $\cF$. Furthermore, the additional $o(\log(T))$ term in \eqref{eq::th_2} is explicitly upper bounded in the proof: its scaling in $T$ only depends on $(C_n)$, and is for instance in $\cO\left(\log(\log(T))\right)$ if $(C_n)$ is polynomial, and constant if it is bounded.

Inspired by this result, we now propose a set of sufficient conditions that allow to upper bound $B(c, \epsilon)$ by a constant, hence proving a logarithmic regret with Theorem~\ref{th::first_bound}.

\begin{assumption}[Sufficient conditions for logarithmic regret]\label{ass::sufficient_prop}
\begin{itemize}
		\item \textbf{Concentration of $D_\pi$ for sub-optimal arms (A2):} for any $\mu > \mu_k$, and $\delta>0$ small enough, \[\sum_{n=1}^{+\infty} \bP\left(D_\pi(F_{k,n}, \mu) \leq D_\pi(F_k, \mu)-\delta\right) = \cO(1)\;.\]
		% \item \textbf{Identifiability of the best arm (A3)} For any empirical distribution\footnote{In parametric cases we replace $F_{1, n}$ by the parametric distribution corresponding to its observations.} $F_{1, n}\in \cF$ with expectation smaller than $\mu_1-\epsilon$, it holds that 
		% \[D_\pi(F_{1, n}, \mu_1)-D_\pi(F_{1, n}, \mu_1-\epsilon)\geq \delta_{\epsilon}\;,\] 
		% for some constant universal constant 
  % $\delta_{\epsilon}>0$ satisfying
  % $c_n = o(e^{n \frac{\delta_{\epsilon}}{2}})$.
\item \textbf{Identifiability of the best arm (A3):} For any $\epsilon>0$, there exists $\delta_{\epsilon}>0$ (depending only on $\mu_1$) such that $c_n = o(e^{n \frac{\delta_{\epsilon}}{2}})$ and 
for any empirical distribution\footnote{In parametric cases we replace $F_{1, n}$ by the parametric distribution corresponding to its observations.} $F_{1, n}\in \cF$ satisfying $\mu_{1,n} \leq \mu_1-\epsilon$ 
		\[D_\pi(F_{1, n}, \mu_1)-D_\pi(F_{1, n}, \mu_1-\epsilon)\geq \delta_{\epsilon}\;.\] 
\item \textbf{Concentration of $D_\pi(F_{1, n}, \mu_1)$ for the optimal arm (A4):} $D_\pi$ admits an exponential concentration inequality of the form \[\bP(D_\pi(F_{1, n}, \mu_1)> x) \leq D_n e^{-nx}, \] for any $x\geq x_0$, where $x_0>0$ can be arbitrary, and where $(D_n)$ is polynomial in $n$.
		\item \textbf{Concentration of the mean estimator (A5):} For $\epsilon>0$ small enough, \[\sum_{n=1}^{T} c_n \bP(\mu_{1, n} \leq \mu_1-\epsilon) = \cO(1)\;.\]
	\end{itemize}
\end{assumption}

We now motivate these assumptions and provide some high-level insights.

\paragraph{(A2) }  \hspace*{-\baselineskip} allows to upper bound the first term of $B(c, \epsilon)$ by a constant. It is slightly weaker than assuming that $D_\pi$ is continuous in the first argument w.r.t. some metric and that $F_{k,n}$ converges ``fast enough" to some neighborhood of $F_k$. %However, this decomposition will be convenient to prove (A2) for several families of distributions.
Intuitively, (A2) ensures the good convergence of the sampling probability of sub-optimal arms in a regime in which the best arm is well estimated.

\paragraph{(A3)--(A4) } \hspace*{-\baselineskip}
might be
%are
the trickiest assumptions to prove for a given family $\cF$, and allow to upper bound the second term of $B(T,c,\epsilon)$. Their combination ensures that arm $1$ is regularly sampled even if it is performing poorly, so that such scenario does not harm the regret.

\paragraph{(A5) } \hspace*{-\baselineskip} directly upper bounds the last term of $B(T,c,\epsilon)$. It depends on the scaling of $(c_n)_{n\in \N}$ and of available upper bounds on $\bP(\mu_{1, n}\geq \mu_1-\epsilon)$. For instance, the Chernoff method leads to an exponentially decreasing bound if $\nu_1$ admit a finite moment-generating function, and Theorem 2 of \citet{fournier_wasserstein} gives bounds decreasing as a power of $n$ if $\nu_1$ admits some finite moment. In Appendix~\ref{app::A5_heavy} we also discuss the possible replacement of the empirical mean by a robust estimator for heavy-tailed distributions.

% If $c_n$ satisfies $c_n = o(e^{-ny})$ for any $y\geq0$, it holds if $\nu_1$ is \emph{light-tailed} (i.e its moment generating function is finite in a positive neighborhood around $0$). Indeed, in that case $\bP(\mu_{1,n}\leq \mu_1-\epsilon)$ admits an exponential concentration inequality (see e.g. \citealp{large_deviation_book}). However, interestingly if $c_n$ is polynomial of order $a$ a concentration inequality in $\cO(n^{-(1+a+\eta)})$ for some $\eta>0$ is sufficient. This is the case for any distribution satisfying $\bE\left[|X|^{1+a+2\eta}\right]<+\infty$ (Corollary of Theorem 2 of \citealp{fournier_wasserstein}). 

%(A3) and (A4) are the conditions that restricts the most the choice of good candidates for $G$. (A3) seems necessary at least for distributions that belong to $\cF$ to make a sub-linear regret achievable. We allow a dependency in $n$ for $\delta_{\epsilon,n}$ for generality, but it will be used only for unbounded families of distributions. Then, (A4) ensures that the best arm has a reasonable probability to be sampled all the time, but it is not clear whether this condition is necessary or not.

We can now establish the main result of this paper, with a detailed proof in Appendix~\ref{app::proof_th2}.

%\textcolor{red}{Reprendre la discussion: why did we came up with these properties, why they look natural, and the fact that some of them can be slightly relaxed but we wrote them this way for simplicity. In appendix we can formulate the "tightest" formulation of (A1)-(A5).}

\begin{corollary}\label{th::main_result}
	Let $\cF$ be a family of distributions and $(F_1,\dots, F_K) \in \cF^K$ be an MAB. Let $\pi$ be a randomized policy satisfying Assumption~\ref{ass::sampling_prob} for a function $D_\pi$ verifying (A1)--(A5) on $\cF$ and some sequences $(a_n, c_n, C_n)_{n\in \N}$, with $a_n>0$ and $a_n=\cO(n^{-1})$. Then, for any $c > 0$ it holds that 
	\[\forall k: \Delta_k>0, \quad \bE[N_k(T)] \leq (1+c) \frac{\log(T)}{D_\pi(F_k, \mu^\star)} + o_c(\log(T)) \;.\]
%which comes from proving that $B(T,c, \epsilon)=\cO_{c, \epsilon}(1)$ in the bound of Theorem~\ref{th::first_bound}. 
Furthermore, setting $a_n=0$ is sufficient if $D_\pi$ is upper bounded, i.e. if for any $\mu \in \R$ there exists a constant $D_\mu^+\in \R$ such that for any $F\in \cP$ it holds that $D_\pi(F, \mu) \leq D_\mu^+$.
\end{corollary}

This result is particularly interesting, as it provides a general methodology to derive theoretical guarantees for a given randomized algorithm $\pi$ on a family of distributions $\cF$ by:

\begin{enumerate}
	\item Proving that $\pi$ satisfies Assumption~\ref{ass::sampling_prob} for some function $D_\pi$ and a suitable sequence $(a_n)$. 
	\item Showing that (A1)--(A5) are satisfied by $D_\pi$ on $\cF$, and concluding with Corollary~\ref{th::main_result}.
\end{enumerate}
% Furthermore, the sequence $(a_n)_{n\in \N}$ needs to be positive only when the family $\cF$ is not compact. For the families we studied, it is necessary only for SPEF and Gaussian distributions.
In the next section we apply this recipe to prove the optimality of several MED and TS algorithms.

%
%prove the strength of this result by showing that (A1)-(A5) are satisfied for all the families of distributions introduced in Section~\ref{sec::introduction} for properly chosen functions $D_\pi^\cF$. Furthermore, proving these properties for a given $D_\pi$ will directly provide the theoretical guarantees of the corresponding MED algorithm, and of the TS for which the BCP satisfies Equation~\eqref{eq::sampling_prob}.


==> results_v1.tex <==
\section{General recipe for the regret analysis of randomized algorithms -- PREVIOUS VERSION OF SECTION 3 -- REMOVE AFTER CHANGES COMPLETED}

In the previous section we introduced some examples of algorithms entering into the scope of our analysis and we now introduce the main theoretical results of this paper.
We first focus on the shared properties of the families of distributions that we introduced, next provide a regret analysis for a generic randomized algorithm, and finally instantiate this analysis to MED and \TS{} introduced in Section~\ref{sec::prelim}.

\subsection{Common properties of existing families of distributions}\label{sec::common_prop}

We start this section by answering the first question that we introduced, exhibiting the salient features shared by the families of distributions for which we know asymptotically optimal bandit algorithms.
We group these generic features in Assumption~\ref{ass::sufficient_prop}, and will prove in the next section that they are sufficient to design a theoretically sound bandit algorithm for a given family of distributions.

\rev{Before stating the assumption, we introduce an additional notation: we denote by $\cP$ the set of all possible cumulative distribution functions on $\R$: for any $F\in \cP$, it holds that $F$ is non-decreasing, $\lim_{x\to -\infty}F(x)=0$ and $\lim_{x\to +\infty} F(x)=1$.}

\begin{assumption}[Properties of the family of distributions $\cF$]\label{ass::sufficient_prop}
Let $F\in \cF$ be any distribution of mean $\mu_F$. Let us denote by $F_n$ the empirical distribution\footnote{If $\cF$ is parametric we assume that $D$ first maps $F_n$ to the distribution of $\cF$ corresponding to the MLE for its parameters.
} of $n$ i.i.d. samples drawn from $F$, and by $\mu_n$ their expectation. 

We assume that there is a function $D: \cP \times \R \mapsto \R^+$ satisfying the following properties\footnote{With a slight abuse of notation we allow $D(F_n, \mu)$ to depend on $n$.}:
\begin{itemize}
\item \textbf{Continuity and monotonicity (A1):} $D$ is continuous in its second argument, the mapping $x \mapsto D(F, x)$ is non-decreasing, and $D(F, \mu)=0$ for any $\mu\leq \mu_F$.
\item \textbf{Lower deviation (A2):} for any $\mu > \mu_F$, and $\delta>0$, \rev{there exists a constant $A_\delta>0$ such that} % small enough, 
\[\sum_{n=1}^{+\infty} \bP\left(D(F_{n}, \mu) \leq D(F, \mu)-\delta\right) \leq A_\delta %\cO_\delta(1)
\;.\]
\item \textbf{Separability of mean levels (A3):} For any $\epsilon>0$, there exists $\delta_{\epsilon, \mu_F}>0$ such that if $F_n \in \cP$, and $\mu_n \leq \mu_F-\epsilon$ it holds that
		\[D(F_n, \mu_F)-D(F_n, \mu_F-\epsilon)\geq \delta_{\epsilon, \mu_F}\;.\] 
\item \textbf{Upper deviation (A4):} \rev{There exists a constant $x_0>0$ such that, for any $x\geq x_0$, it holds that}
\[\bP(D(F_{n}, \mu_F)> x) \leq \alpha_{n}\times e^{-nx}, \] \rev{for some constant $\alpha_{n}>0$ %is non-increasing in $x$ for any fixed $n$, 
that is polynomial in $n$.} %for any fixed $x$.
%%%% I don't remember why we needed $\alpha_{n,x}$, I think it was for Gaussians but it seems we simplified the lemma now %%%
% \item \textbf{Minimal concentration speed of the mean estimator (A5):} There exists $\eta>0$ such that for any $\epsilon>0$, $\bP(\mu_n\leq \mu_F-\epsilon)= \cO(n^{-(1+\eta)})$.
\end{itemize}
\end{assumption}

These properties might look a bit heavy, but their level of generality is necessary to tackle all the settings covered in this paper, \rev{in particular the non-parametric settings}. 

\rev{\paragraph{Example: distributions supported on $[0,1]$} In many usual cases the assumption} is relatively easy to verify. For example, let us consider bounded distributions with range $[0,1]$ and choose $D(F_n, \mu)=2(\mu-\mu_n)^2\ind(\mu\geq \mu_n)$, as would be done in Maillard Sampling \citep{Maillard11, jun2022}. Then, (A1) is direct from the definition of $D$, and it follows from a simple computation that (A3) holds with $\delta_{\epsilon, \mu_F}=2\epsilon^2$. The remaining properties can then be obtained with minimal effort using Hoeffding's inequality. %(that gives (A5) directly). 
For instance, we prove (A4) (and the same can be done with (A2)) writing that
\[\bP(D(F_n, \mu_F)>x) = \bP(\mu_n < \mu-\sqrt{x/2}) \leq e^{-2 n(\sqrt{x/2})^2} = e^{-nx} \;. \]
Similarly, if we considered SPEF and defined $D$ as the KL-divergence corresponding to $\cF$ then Chernoff's inequality provides simultaneously (A2) and (A4) %and (A5) 
(see Appendix~\ref{subsec::SPEF} for details). \rev{However, in the same bounded setting, if we consider instead the divergence derived from the lower bound (Eq.~\eqref{eq::asymp_opt_def}), that is $D = \kinf^\cF$, then the constants have all the dependencies allowed by the assumption: using Lemma 13 from \citep{honda11MED} we obtain that $\delta_{\epsilon, \mu_F}=\frac{\epsilon^2}{2(\mu_F-\epsilon)(B-\mu_F)}$, and using Lemma 6 from \citep{KL_UCB} we get $\alpha_n=e(n+2)$. Note that it is not clear that this choice of $\alpha_n$ is tight, but we are not aware of an improved result.}

\rev{\paragraph{Additional intuitions} In} some sense, we can say that Assumption~\ref{ass::sufficient_prop} generalizes the properties that are usually derived from concentration inequalities on the empirical means, for simple choices of $D$ as in our example. This generalization is particularly useful for the analysis of non-parametric models, where $\kinf^\cF$ cannot be expressed only as a function of empirical means.

Indeed, intuitively the functions $D(F,\mu)$ of interest measure how ``far'' a distribution $F$ is to the class of distributions from $\cF$ with expectation larger than $\mu$.
%Indeed, intuitively the functions $D$ of interest are those for which $D(F, \mu)$ measures how ``far'' a distribution $F$ is to the sub-space of distributions from $\cF$ with expectation larger than $\mu$, according to some metric. 
In the rest of the paper we will typically consider $D$ close to $\kinf^\cF$ for the families considered, since this choice can lead to optimal algorithms, but other choices are possible (e.g. multiples of the squared gap or Bernoulli KL divergence for bounded distributions). Regarding the properties that we expect from $D$, we can first remark that \textbf{(A2)} is slightly weaker than assuming that $D$ is continuous in the first argument w.r.t. some metric and that $F_{n}$ converges ``fast enough" to some neighborhood of $F_k$. It ensures that the expected number of sample sizes for which the empirical distribution of a sub-optimal arm is ``too close to $\mu^\star$'' %(and $\mu$ is larger than the true expectation of the observations) 
is finite. On the contrary, \textbf{(A4)} relates an empirical distribution to the mean of the true distribution of its observations, requiring an exponentially decreasing bound. This ensures that, even if an empirical distribution is performing poorly (roughly, its expectation is under-estimated), it has a low probability of being very ``far'' from the true distribution.
Finally, \textbf{(A3)} ensures that $D$ allows to properly separates the different mean levels, so that it can be used to distinguish an arm of mean $\mu$ from an arm of mean $\mu-\epsilon$ for $\epsilon>0$. 

% We can finally comment on \textbf{(A5)}. Again, the statement is made general to cover all of our settings. If the distributions are \emph{light-tailed}, that is $\bE_F[\exp(\lambda |X|)]<+\infty$ for some $\lambda>0$, then an exponentially decreasing upper bound can be achieved (e.g. with Chernoff method). However, the desired polynomial bound can also be obtained if the distributions are \emph{heavy-tailed} but admit a finite moment or order strictly larger than $2$. We refer to Theorem 2 of \citet{fournier_wasserstein} for such bound. Furthermore, in Appendix~\ref{app::A5_heavy} we also discuss the possible replacement of the empirical mean by a robust estimator for heavy-tailed distributions, to obtain 
% an exponentially decreasing bound in that case, that works even if only a moment of order strictly larger than $1$ is finite.

We now show the level of generality of these properties by proving that they hold for all the families of distributions presented in Section~\ref{sec::introduction}. 
In each case, we choose a function $D$ as close as possible to the $\kinf^\cF$. %We detail the computation of these functions in Appendix~\ref{app::notation}, and postpone the proof in Appendix~\ref{app::proofs_A1_A5}, where we provide all the technical details. % and motivate the modifications made to $\kinf^\cF$ in some cases.
We postpone the proof to Appendix~\ref{app::proofs_A1_A5}, where we provide all the technical details. % and motivate the modifications made to $\kinf^\cF$ in some cases.
% \begin{theorem}[Various families of distributions satisfying Assumption~\ref{ass::sufficient_prop}]\label{lem::P15}
% Let $F$ be a distribution of mean $\mu_F$ and standard deviation $\sigma_F$, and $\mu\in\R$ be a threshold. Then, Assumption~\ref{ass::sufficient_prop} is satisfied if $\cF$ is one of the following families:  
% \begin{itemize}
% 	\item \textbf{Single Parameter Exponential Family} with $D(F, \mu) = \kinf^\cF(F, \mu)$.%, if $(a_n)_{n\in \N}$ satisfies $\forall n \in \N,\; a_n > 0$ and $1/a_n = \cO(n^\alpha)$ for some $\alpha>0$.
% 	\item \textbf{Bounded distributions} with a known upper bound $B$, with $D(F, \mu) = \kinf^\cF(F, \mu)$.
% 	\item \textbf{Gaussian distributions}\footnote{For the Gaussian case we prove slightly relaxed version of (A3) and (A4) that are sufficient to obtain the same results, and justify the tuning of the algorithms in the next section, see Section~\ref{app::gauss_P15} for more details.} with unknown means and variances, if% if $a_n > \frac{2}{n-2}$ and 
%  \[D(F, \mu) = \kinf^\cF(F, \mu)\times \ind( (\mu-\mu_F)^2\leq \sqrt{n_F}, \sigma_F^2 \leq \sqrt{n_F})\;,\] 
%  where $n_F$ is the size of the support of $F$ ($+\infty$ if $F$ is continuous).
% 	\item \textbf{$h$-moment conditions:} Let $h$ be a known positive convex function satisfying $\frac{h(|x|)}{|x|^{1+\eta}} \to + \infty$ for some $\eta>0$, and $\cF$ be defined as \begin{equation}\label{eq::uncentered_main}\cF = \left\{F \in \cP:\; \bE\left[h(|X|)\right] < B \;, \; \bE[h(|X|)^{2+\epsilon_F}]<+\infty \text{ for some } \epsilon_F>0 \right\} \;,\end{equation} 
%  then (A1)--(A4) hold with $D(F, \mu) = \kinf^\cF(F, \mu) \ind(F \in \cF)$. This is also the case if the condition is \textbf{centered}, i.e. $h(|X|)$ is replaced by $h(|X-\mu_F|)$ in \eqref{eq::uncentered_main}, under the additional assumption that the means are lower bounded by a known constant $\mu^-$.
% \end{itemize}
% \end{theorem}
\begin{theorem}[Various families of distributions satisfying Assumption~\ref{ass::sufficient_prop}]\label{lem::P15}
Let $F$ be a distribution of mean $\mu_F$ and standard deviation $\sigma_F$, and $\mu\in\R$ be a threshold. Then, Assumption~\ref{ass::sufficient_prop} is satisfied if $\cF$ is one of the following families:  
\begin{itemize}
	\item \textbf{Single Parameter Exponential Family} with \[D(F, \mu) = \kinf^\cF(F, \mu) \coloneqq \kl(\mu_F, \mu) \;, \]
 where $\kl$ is the Kullback-Leibler divergence corresponding to the parametric family, expressed as a functions of the means of the two distributions.%, if $(a_n)_{n\in \N}$ satisfies $\forall n \in \N,\; a_n > 0$ and $1/a_n = \cO(n^\alpha)$ for some $\alpha>0$.
	\item \textbf{Bounded distributions} with a known upper bound $B$, with \[D(F, \mu) = \kinf^\cF(F, \mu)\coloneqq  \max_{\lambda \in \left(0, \frac{1}{B-\mu}\right]}\bE_{F}\left[\log\left(1-\lambda(X-\mu)\right)\right]\;. \]
 \item \textbf{Gaussian distributions}\footnote{For the Gaussian case (A3) holds with $\delta_{\epsilon, \mu_F}$ that depends on $n_F$. In addition, we prove a slightly weaker version of Assumption~\ref{ass::sufficient_prop} instead of Assumption~\ref{ass::sufficient_prop} itself. Both of them are not a problem in the subsequent analysis, see Appendix~\ref{app::gauss_p15} for more details.} with unknown means and variances, if% if $a_n > \frac{2}{n-2}$ and 
 \begin{align}
 D(F, \mu) = \kinf^\cF(F, \mu)\times \ind( (\mu-\mu_F)^2\leq \sqrt{n_F}, \sigma_F^2 \leq \sqrt{n_F})\;,
 \label{check_gaussian}
 \end{align}
 where $n_F$ is the size of the support of $F$ ($+\infty$ if $F$ is continuous). Furthermore, 
 \[\kinf^\cF(F, \mu) \coloneqq \frac{1}{2}\log\left(1+\frac{(\mu-\mu_F)^2}{\sigma_F^2}\right)\times \ind(\mu\geq \mu_F) \;. \]
	\item \textbf{$h$-moment conditions (uncentered):} Let $h$ be a known positive convex function satisfying $\frac{h(|x|)}{|x|^{1+\eta}} \to + \infty$ for some $\eta>0$, and $\cF$ be defined as follows, 
\begin{equation}\label{eq::uncentered_main}\cF = \left\{F \in \cP:\; \bE_F\left[h(|X|)\right] < B \;, \; \bE_F[h(|X|)^{2+\epsilon_F}]<+\infty \text{ for some } \epsilon_F>0 \right\} \;.\end{equation} 
 Then, (A1)--(A4) hold with $D(F, \mu) = \kinf^\cF(F, \mu) \ind(F \in \cF)$. Furthermore, 
 \[\kinf^\cF(F, \mu) =  \max_{(\lambda_1, \lambda_2) \in \cR_2}\bE_{F}\left[\log\left(1-\lambda_1(X-\mu)-\lambda_2 (B-h(|X|))\right)\right]\;, \]
 where $\cR_2= \{(\lambda_1,\lambda_2) \in (\R^+)^2 \;:\; \forall x \in \R \;, 1-\lambda_1 (x-\mu) - \lambda_2 (B-h(|x|)) \geq 0 \}$ is the set for which the logarithm is defined.
 
\item \textbf{Centered $h$-moment conditions:} 
Let $h$ be a known positive convex function satisfying $\frac{h(|x|)}{|x|^{1+\eta}} \to + \infty$ for some $\eta>0$, and $\cF$ be defined as \begin{equation}\label{eq::uncentered_main}\cF = \left\{F \in \cP:\; \bE_F\left[h(|X-\mu_F|)\right] < B \;, \; \bE_F[h(|X|)^{2+\epsilon_F}]<+\infty \text{ for some } \epsilon_F>0, \mu_F\geq \mu^- \right\} \;,\end{equation}
for a known constant $\mu^-$. Then, (A1)--(A4) hold with $D(F, \mu) = \kinf^\cF(F, \mu) \ind(F \in \cF)$. Furthermore, %we prove in Appendix~\ref{app::cent_h_P15} that
 \begin{equation}\label{eq::kinf_centered}
     \kinf^\cF(F, \mu) =  \max_{(\lambda_1, \lambda_2) \in \cR_2}\bE_{F}\left[\log\left(1-\lambda_1(X-\mu)-\lambda_2 (B-h(|X-\mu|))\right)\right]\;,
 \end{equation} where $\cR_2= \{(\lambda_1,\lambda_2) \in (\R^+)^2 \;:\; \forall x \in \R \;, 1-\lambda_1 (x-\mu) - \lambda_2 (B-h(|x-\mu|)) \geq 0 \}$.
\end{itemize}
\end{theorem}

Theorem~\ref{lem::P15} answers the first question raised in Section~\ref{sec::introduction}: there is indeed a set of fundamental properties shared by all the main families of distributions that have been studied in the bandit literature, which may explain why the same algorithm principles work for all of them. Furthermore, we proved that these assumptions are valid for $\kinf^\cF$ or a function that matches $\kinf^\cF$ once the empirical distribution of a sub-optimal arm is ``close" to its true distribution. %As far as we know, this paper is the first to provide theoretical guarantees for settings with centered $h$-moment condition, that we believe to be an interesting result.

To prove this theorem, we use several results from the literature, but also prove novel results of independent interest. For instance, Lemma~\ref{lem::conc_gaussian} in Appendix~\ref{app::gauss_p15} is (as far as we know) a novel concentration inequality for the $\kinf$ of Gaussian distributions with unknown variances. %We now show the application of these results for the MED and TS algorithms introduced in Section~\ref{sec::prelim}.
Still on Gaussian distributions, a check on the squared gap and variance is added if $F$ is an empirical distribution as shown in \eqref{check_gaussian}.
This is necessary to prove (A3), since $\kinf(F,\mu)-\kinf(F, \mu-\epsilon)$ could be made arbitrarily small otherwise in some (low probability) scenarios. %$\delta_{\epsilon, \mu_F}$ actually depends on $n$ in this setting, which is not a problem in the proof (see details in Appendix~\ref{app::gauss_p15}). We did not introduce $n$ in the notation for clarity, since this dependency holds only in this example.
Finally, the expression of $\kinf$ for the centered $h$-moment conditions in \eqref{eq::kinf_centered} is similar to its counterpart in the uncentered case. However, it is a novel result that we prove in Appendix~\ref{app::cent_h_P15}.

We now motivate the changes in the definition of $\cF$ for $h$-moment conditions, compared to the initial definition from \cite{agrawal2020optimal}. We recall that they consider families of distributions satisfying \[\cF = \left\{F \in \cP:\; \bE\left[h(|X|)\right] \leq  B \right\} \text{ for a convex function } h \text{ satisfying } \frac{h(|x|)}{x} \to +\infty \;. \]

In our case, the motivation for the strict inequality $\bE[h(|X|)]<B$ and for requesting $\bE[h^{2+\epsilon_F}]<+\infty$ is that these conditions ensures with large enough probability that the empirical distributions belong to $\cF$ so that the regret is not harmed by checking that $\{F_n \in \cF\}$. %This is crucial for our analysis, and allows us to provide results for the centered case, which is novel. 
We refer to Appendix~\ref{app::h_P15} for details.

\subsection{Generic analysis of randomized bandit algorithms}\label{sec::generic_analysis}

While the previous section focused on the shared properties of several usual families of distributions, we now introduce our main assumption on the bandit algorithm to propose a unified analysis.

\begin{assumption}[Upper and lower bound on $p_k^\pi(t)$] \label{ass::sampling_prob}
$\pi$ is a randomized bandit algorithm, and there exists a function $D_\pi: \cP \times \R \mapsto \R$, \textbf{positive} sequences $(c_n)_{n \in \N}, (C_n)_{n \in \N}$ and a \textbf{non-negative} sequence $(a_n)_{n \in \N}$% satisfying $a_n=\cO(n^{-1})$
such that for any $k$ in $[K]$ $\pi$ satisfies
\begin{equation}\label{eq::sampling_prob} p_k^\pi(t) \exp\left(N_k(t) \frac{D_\pi(F_k(t),\mu^\star(t))}{1+a_{N_k(t)}}\right) \in [c_{N_k(t)}^{-1}, C_{N_k(t)}] \;.
\end{equation}
Furthermore, $\log(C_n)=\cO(n^\alpha)$ for some $\alpha<1$ and $c_n = o(e^{n \beta})$ for any $\beta>0$.
%The bandit algorithm $\pi$ admits a function $D_\pi: \cP \times \R \mapsto \R$ and some \textbf{positive} sequences $(a_n)_{n \in \N}, (c_n)_{n \in \N}, (C_n)_{n \in \N}$ such that for any $F_k(t), \mu_k(t)$ it holds that
%\begin{equation}\label{eq::sampling_prob} p_k^\pi(t) \exp\left(N_k(t) \frac{D_\pi(F_k(t),\mu^\star(t))}{1+a_{N_k(t)}}\right) \in [c_{N_k(t)}^{-1}, C_{N_k(t)}] \;,
%\end{equation}
%for some function $D_\pi$.
\end{assumption}

This assumption is the very core of the general recipe that we propose to analyze randomized policies, but it will be the only assumption directly made on a given policy. We actually prove the result that we are going to present under the more general Assumption~\ref{ass::relaxed_sp} (presented in Appendix) on the sampling probabilities, but we chose to present Assumption~\ref{ass::sampling_prob} in the main paper for the clarity of the presentation. %Intuitively, a good choice of $D_\pi$ would be as close as possible to $\kinf^\cF$ to obtain an optimal algorithm. 
Equation~\eqref{eq::sampling_prob} recalls the form \eqref{eq::MED} of the general MED presented in Section~\ref{sec::prelim}, and we explained that \TS{} may also satisfy it under some conditions on its BCP. The requirements for $(c_n, C_n)$ give some flexibility to this definition, but we will show that in most of the cases considered in this paper they are at most polynomial. We discuss these questions in the next section,
% We can directly verify that Assumption~\ref{ass::sampling_prob} holds with $c_n = K$ and $C_n=1$ for any $n\in \N$, as under (A1) we have that $D_\pi(F_k(t), \mu^\star)\geq 0$ with equality if $\mu_k(t)=\mu^\star(t)$.
and now establish the main result of this paper.

\begin{theorem}\label{th::main_result}
Let $\cF$ be a family of distributions and $(F_1,\dots, F_K) \in \cF^K$ be an MAB, and assume w.l.o.g. that $\mu_1=\max \mu_k$. Let $\pi$ be a randomized policy satisfying Assumption~\ref{ass::sampling_prob} or Assumption~\ref{ass::relaxed_sp} for a function $D_\pi$ and sequences $(a_n, c_n, C_n)_{n\in \N}$ that make Assumption~\ref{ass::sufficient_prop} 
with $D:=D_{\pi}$
hold on $\cF$.

Further assume that $\sum_{n=1}^{+\infty} c_n \bP(\mu_{1,n}\leq \mu_1-\epsilon)=\cO_{\epsilon}(1)$ for any $\epsilon>0$. Then, for any $c > \displaystyle \lim_{n\to \infty} a_n$, if $a_n^{-1}$ is polynomial it holds that 
	\[\forall k: \Delta_k>0, \quad \bE[N_k(T)] \leq (1+c) \frac{\log(T)}{D_\pi(F_k, \mu^\star)} + o_c(\log(T)) \;.\]
%which comes from proving that $B(T,c, \epsilon)=\cO_{c, \epsilon}(1)$ in the bound of Theorem~\ref{th::first_bound}. 
Furthermore, setting $a_n=0$ is sufficient if $D_\pi$ is upper bounded as follows: for any $\mu \in \R$ there exists a constant $D_\mu^+\in \R$ such that for any $F\in \cP$ it holds that $D_\pi(F, \mu) \leq D_\mu^+$. %Finally, the constant $o_c(1)$ scales polynomially in $c^{-1}$. 
\end{theorem}

We can comment on the assumptions required to obtain this result: we use Assumption~\ref{ass::sufficient_prop} on the family of distribution, and Assumption~\ref{ass::sampling_prob} (or \ref{ass::relaxed_sp}) on the randomized bandit algorithm, that we already introduced and for which we provided some intuitions. We also need a last assumption that $\sum c_n \bP(\mu_{1, n}\leq \mu_1-\epsilon)$ converges. It depends both on the algorithm (via $c_n$) and on the distributions, but is a mild assumption in most settings: the deviation probability is exponentially decreasing if the distribution is \emph{light-tailed} (that is $\bE_F[\exp(\lambda |X|)]<+\infty$ for some $\lambda>0$), which is enough for the convergence due to the assumption that $(c_n)_{n\in \N}$ is polynomial in $n$. Hence, only heavy-tailed distributions may be problematic. In that case, the empirical means can be replaced by any robust estimator, as discussed in Appendix~\ref{app::A5_heavy}.
% Again, the assumption is made general to cover all of the settings considered in this paper. If the distributions are \emph{light-tailed}, that is $\bE_F[\exp(\lambda |X|)]<+\infty$ for some $\lambda>0$, then an exponentially decreasing upper bound can be achieved for $\bP(\mu_{1,n}\leq \mu_1-\epsilon)$ (e.g. with Chernoff method). In that case the assumption hold thanks to our upper bound on $c_n$. In Appendix~\ref{app::A5_heavy} we also discuss the possible replacement of the empirical mean by a robust estimator, allowing the same result to hold for \emph{heavy-tailed} distributions. Finally, in some cases where $c_n$ is constant or polynomial the assumption can still hold for some heavy-tailed distributions. We refer to Theorem 2 of \citet{fournier_wasserstein} for polynomially decreasing concentration inequalities for the empirical mean of heavy-tailed distributions.

Theorem~\ref{th::main_result} provides a general methodology to derive new theoretically sound bandit algorithms for a given family $\cF$, by first finding a suitable function $D_\pi$ that makes Assumption~\ref{ass::sufficient_prop} hold with $D\coloneqq D_\pi$, and then designing a randomized algorithm $\pi$ satisfying Assumption~\ref{ass::sampling_prob} with this same function. Conversely, an existing randomized bandit algorithm can be analyzed by computing a range on its sampling probabilities in the form of Assumption~\ref{ass::sampling_prob}, and then verify that the function $D_\pi$ that was identified makes Assumption~\ref{ass::sufficient_prop} hold for the family of distributions.

\paragraph{Elements of proof} The proof of Theorem~\ref{th::main_result} can be decomposed into two parts. We first prove an upper bound of the expected number of pulls of each sub-optimal arm $k$ for any randomized policy satisfying Assumptions~\ref{ass::sampling_prob} and property (A1) of Assumption~\ref{ass::sufficient_prop} only.

\begin{lemma}\label{th::first_bound}
Let $\pi$ be a policy satisfying Assumption~\ref{ass::relaxed_sp} or \ref{ass::sampling_prob} for a function $D_\pi$ satisfying (A1) of Assumption~\ref{ass::sufficient_prop}. Then, for any $c > \displaystyle \limsup_{n\to \infty} a_n$ and for any $\epsilon>0$, it holds for any sub-optimal arm $k$ that 
\begin{equation}\label{eq::th_2}\bE[N_k(T)] \leq  (1+c) \frac{\log(T)}{D_\pi(F_k, \mu_1)} + B(c, \epsilon) + o(\log(T))\;,\end{equation}
with \begin{align*}
	B(c, \epsilon) = &\sum_{n=1}^{+\infty} \bP\left(D_\pi(F_{k,n}, \mu_1-\epsilon)\frac{1+c}{1+a_n} \leq D_\pi(F_k, \mu_1)\right) \\ 
	+ &\sum_{n=1}^{+\infty} c_n \bE\left[e^{n \frac{D_\pi(F_{1,n}, \mu_1-\epsilon)}{1+a_n}}-1\right] +   \sum_{n=1}^{+\infty} (c_n-1) \bP\left(\mu_{1,n} \leq \mu_1-\epsilon \right) \;. 
\end{align*}
\end{lemma}
The proof of this result is inspired by the analysis of Maillard Sampling \citep{jun2022}, and we detail it in Appendix~\ref{app::proof_th1}. The additional $o(\log(T))$ term in \eqref{eq::th_2} is explicitly upper bounded in the proof: its scaling in $T$ only depends on $(C_n)$, and is for instance in $\cO\left(\log(\log(T))\right)$ if $(C_n)$ is polynomial, and constant if it is bounded.

Then, the term $B(c, \epsilon)$ encapsulates the elements in the upper bound that require to carefully analyze the properties of $D_\pi$ on the family of distributions $\cF$, and hence motivated the design of properties (A2)--(A4) in Assumption~\ref{ass::sufficient_prop}, and the additional assumption $\sum c_n \bP(\mu_{1, n}\leq \mu_1-\epsilon)=\cO_{\epsilon}(1)$. \rev{When $c_n$ is independent of $n$ and $\mu_{1,n}$ admits a sub-Gaussian tail bound this term is typically of order $\epsilon^{-2}$.} The rest of the proof of Theorem~\ref{th::main_result} consists in upper bounding $B(c, \epsilon)$ by a constant. We can upper bound its first component with (A2), using the continuity of $D_\pi$ in its second argument and choosing $\epsilon$ small enough. Then, using (A3) and (A4) we can upper bound its second term by explicitly computing the expectation. Finally, the remaining term justifies the last assumption presented in Theorem~\ref{th::main_result}. As previously discussed, this assumption is mild. %For example, if $c_n=\cO(1)$ then (A5) is sufficient to make it hold.
